Vinci2: Providing Proactive Assistance in Continuous Egocentric Videos

When should an intelligent assistant speak up without being asked? Continuous egocentric video offers rich, evolving context that enables a new form of assistance: one that is proactive rather than merely reactive. Yet existing approaches either wait passively for user queries or treat every detected event as requiring a response, without considering the user's history, current activity, or whether assistance would actually be welcome. We reframe proactive assistance as a context-dependent decision problem: the agent must not only perceive what is happening, but reason over accumulated temporal context to determine when and whether to intervene. To this end, we present Vinci2, a proactive egocentric assistance system that advances the on-device assistant Vinci from reactive response toward proactivity. On the evaluation side, we present EgoServe, the first large-scale benchmark for proactive assistance in continuous egocentric video. EgoServe comprises over 3,000 service instances organized along 4 temporal memory horizons, ranging from immediate safety alerts to long-term habit coaching, across 10 service categories. On the modeling side, we propose EgoMemo, a training-free, memory-augmented agent that maintains three complementary memory representations: multi-scale temporal summaries, a semantic knowledge graph, and visual embedding archives. At each timestep, EgoMemo performs retrieval-augmented reasoning to determine whether assistance is warranted and, if so, produces contextually grounded responses. Experiments demonstrate that EgoMemo establishes strong baselines on EgoServe while remaining competitive on existing egocentric benchmarks. Our benchmark and code are publicly available at \href{https://sitonggong.github.io/EgoServe-page/}{Vinci2}.

==> Tables/annotation_prompt.tex <==
% \section{EgoServe Annotation Prompts}
% \label{sec:supp_annotation_prompts}

% We provide the complete prompt templates used in the EgoServe annotation pipeline to construct service-event annotations and dialogues for each dataset. These prompts are reproduced \textbf{verbatim} from the codebase. The annotation pipeline operates per service category: each prompt defines the role, service taxonomy (for mutual-exclusion awareness), detection criteria, temporal scope, dialogue generation requirements, and structured output schema.

% \subsection{EgoLife Annotation Prompts}
% \label{sec:supp_egolife_annotation}

% The EgoLife subset uses 11 separate prompts, one per service sub-type. Each prompt is sent to Gemini along with the human-annotated interaction records for a batch of $\leq$10-minute egocentric segments. The model extracts service events from the annotations and generates multi-turn dialogues. All 11 prompts share a common input format (structured JSON of interaction records with time windows) and output schema, but differ in their service definition, detection criteria, mutual exclusion rules, and dialogue style.

\begin{promptbox}[EgoLife — Instant · Safety]
\#\#\# Task Context

You are analyzing MULTIPLE egocentric annotation files (each less than 10 minutes) from the EgoLife dataset for one contiguous batch of time (less than 2.5 hours).

Your job in this stage is signal mining and dialogue generation for a special Instant Proactive Service subtype:

Instant Safety Proactive Service  
(short: Instant Safety)

This service focuses on acute physical hazards within a very short time window (≈0-10 seconds), where:
- The user is currently performing an action or is in a configuration that can immediately cause bodily harm (cut, burn, slip, collision, electric shock, etc.).
- The danger is present right now or in the next few seconds (no more than 10 seconds), not a long-term ergonomic or lifestyle issue.
- A short, timely warning from the assistant could realistically help the user avoid injury in this moment.

Typical examples:
    - The user's fingers are very close to a knife blade while cutting.
    - The user reaches over a boiling pot or an open flame with bare hands or loose clothing.
    - There is spilled liquid on the floor right where the user is stepping.
    - The user touches or approaches exposed electrical wiring or a wet powered device.
    - The user stands or walks very near a moving vehicle, trolley, or heavy object.

*You must:*
1. Scan the current batch to detect instant safety hazards grounded in the annotations.
2. For each hazard, select the current moment where:
   - the hazard is already present or about to occur within a few seconds, and
   - a warning would still be timely and helpful.
3. For each such moment, generate a short multi-turn dialogue where the assistant:
   - issues a clear, concise safety warning, and
   - offers concrete, practical suggestions to reduce the immediate risk.

There is no historical memory JSON for this service:
- You treat each batch independently.
- You do not track cross-day or long-horizon safety state.
- You only output dialogues for this batch, each grounded in one current hazardous episode.

You must NOT guess new hazards, invent timestamps, or hallucinate behaviors not supported by the annotations.

⸻

\#\#\# Authoritative Timestamps \& Fine-Grained Evidence Priority

Each fine-grained annotation entry has a time\_window aligned to the original video, for example:
    - i\_do\_steps[].time\_window
    - interactions\_with\_objects[].time\_window
    - interactions\_with\_people[].time\_window
    - speakers\_say[].time\_window

All time\_window strings already have the format:

\textgreater{} DAY\# HH:MM:SS-HH:MM:SS
  
When you output current\_time\_window, you MUST copy it only from i\_do\_steps[].time\_window or speakers\_say[].time\_window.
You must NOT use interactions\_with\_objects, interactions\_with\_people, or interaction\_records as the source of current\_time\_window.
Do NOT interpolate, merge, extend, shrink, or invent new time ranges.

Fine-grained evidence priority

When detecting Instant Safety opportunities, you must prioritize fine-grained entries:

- Primary sources to consider as candidate hazardous episodes:
  - i\_do\_steps
  - interactions\_with\_objects
  - interactions\_with\_people
  - speakers\_say

Treat each fine-grained entry as a potential Instant Safety episode only if its content clearly matches the safety definition (immediate physical hazard within a few seconds).

This priority applies both to:

- which content you treat as hazardous episodes, and  
- which time\_window you copy for those episodes.

⸻

\#\#\# Input Human Annotations

You are given MULTIPLE JSON objects, each representing a \textless{}= 10-minute egocentric segment:
\{
  "segment\_id": "\textless{}identifier for this \textasciitilde{}10-minute segment\textgreater{}",
  "description": "... high-level summary of what I do in this segment ...",
  "interaction\_records": [
    \{
      "time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "description": "... micro-episode summary ...",

      "i\_do\_steps": [ ... ],
      "speakers\_say": [ ... ],
      "interactions\_with\_objects": [ ... ],
      "interactions\_with\_people": [ ... ],
      "environment\_state": [ ... ],
      "task\_transition": [ ... ],
      "confidence": 0.0-1.0
    \}
  ]
\}

These interaction\_records and their subfields are your only evidence.

The coverage of this batch is defined by the minimum and maximum timestamps appearing in these JSONs.  
You can assume this coverage is at most about 2.5 hours.

⸻

\#\#\# Service Category

- service\_main\_type: "Instant Proactive Service"
- service\_sub\_type: "Safety Proactive Service"

Note: this service operates on instant, short-horizon physical hazards (≈0-10 seconds) and is distinct from:

- Episodic Memory Recall (short-horizon episodic memory across ≤ 2.5 hours),
- Episodic Task Reminder (unfinished tasks inside one episode),
- Habit-Coaching or Long-Term Safety Habits (chronic risk, posture, lifestyle),
- Long-Horizon Memory-Link (cross-day or ≥2h links).

⸻

\#\#\# What counts as an Instant Safety signal?

An Instant Safety opportunity is defined by one current hazardous episode, characterized by:

1. Concrete hazardous condition

   The annotations indicate that the user is interacting with, or very near to, a hazard such as:

   - open flame, very hot cookware, boiling liquids,
   - knife edges or sharp tools near hands/body,
   - spilled liquids on the floor, loose cables that could cause tripping,
   - exposed wires, wet or damaged electrical equipment,
   - unstable heavy objects that might fall,
   - nearby moving vehicles, bikes, trolleys, or machines.

2. Immediate risk window

   The risk is:

   - present now or in the next few seconds,
   - not yet mitigated (no evidence of moving away, switching off, etc.),
   - clearly more than a mild ergonomic or comfort issue.

The core question:  
\textgreater{} “If a careful assistant were watching this exact moment, would they reasonably say:  
\textgreater{}  *'Be careful right now, you might get hurt in the next few seconds.'*?”

If yes, it is a strong candidate for Instant Safety.

⸻

\#\#\# Mutual Exclusion \& Priority vs. Other Services

Use these rules to distinguish Safety from other proactive services:

1. Safety vs. Tool Use
   - Safety: the main concern is immediate injury risk (cut, burn, shock, collision) that could happen in the next few seconds.  
     Even if the user is also using a tool in a suboptimal way, label it Safety when physical danger is high and imminent.
   - Tool Use: the issue is mainly about how the user operates a tool (grip, angle, stability, posture), not about an acute bodily hazard.  
     Typical Tool Use cases are: holding a knife in an unstable way, using a screwdriver at an awkward angle, or standing too far/close for good leverage, but no clear risk of being cut/burned/shocked in the next few seconds.  
     A Tool Use message sounds like “hold the knife like this for better control” or “adjust your stance so the drill is more stable,” rather than “watch out, you might get hurt right now.”

2. Safety vs. Error-Recovery
   - Error-Recovery: the user chooses the wrong object/step/target/configuration in a multi-step workflow, and the main problem is that they must roll back to an earlier step and redo correctly, not that they are in immediate physical danger.  
     For example, the user does step 1 and step 2 of a procedure, realizes step 2 was wrong, and needs to go back to the state after step 1 and repeat step 2; or they pour a reagent into the wrong container but there is no acute hazard.
   - If the same workflow error also creates an acute physical danger (e.g., placing a flammable liquid beside an open flame, mis-wiring something that can shock them), then for this service it should be treated as Safety, not pure Error-Recovery.

3. Safety vs. Resource Reminder
   - Resource Reminder: the user is about to leave non-closed states (stove still on, door unlocked, device not shut down) but there is no immediate serious hazard at this exact moment (e.g., low heat with a stable pot and no overflow yet).
   - If the leftover state is already causing immediate serious danger (e.g., an unattended pot already boiling over, gas flame under an almost dry pan), treat it as Safety here.

4. Safety vs. Habit-Coaching / Long-Term
   - Posture, screen distance, repetitive strain, or lifestyle risk without a specific acute moment of injury belong to Habit-Coaching or Long-Term services, not Instant Safety.

⸻

\#\#\# Time-Window Rules (strict)

For every Instant Safety dialogue you output, you must define a single:

- current\_time\_window representing the hazardous episode and the moment when the assistant speaks.

\#\#\#\# Rules:

1. Current time window (current\_time\_window)
   - Prefer to copy from one fine-grained entry's time\_window:
     - i\_do\_steps[].time\_window, or
     - interactions\_with\_objects[].time\_window, or
     - interactions\_with\_people[].time\_window, or
     - speakers\_say[].time\_window.
   - Do NOT merge or fabricate new ranges.

2. Instant horizon
   - current\_time\_window should correspond to the short segment (≈0-10 seconds) where:
     - the hazardous configuration arises, and
     - a warning would still be in time to prevent harm.

The assistant's first proactive utterance is interpreted as happening during or immediately after this current\_time\_window.

⸻

\#\#\# Instant Safety Detection Objective

For the current batch (no external history):

1. Scan all segments and interaction\_records to find candidate hazardous episodes where:
   - fine-grained annotations describe risky objects, body positions, or environmental states, and
   - the risk could cause physical injury within the next few seconds.

2. For each candidate, verify:
   - There is a specific hazard (e.g., knife near fingers, boiling water near hands).
   - The risk is immediate (not vague or long-term, no more than 10 seconds).
   - There is no evidence that the user has already moved away or fully mitigated the risk.

3. For each valid hazardous episode:
   - Choose the most fine-grained time\_window that best captures the critical 0-10 second window, and this time\_window MUST come from i\_do\_steps[].time\_window or speakers\_say[].time\_window in the annotations.
   - Record the local scene context and a short explanation of why this is dangerous now.

4. For each such episode, generate:
   - One structured Instant Safety entry with:
     - current\_segment\_id, current\_time\_window, supporting\_source,
     - a neutral scene description,
     - hazard\_key, hazard\_summary, risk\_type, potential\_consequence,
     - occurrence\_confidence.
   - One multi-turn dialogue where the assistant issues a timely safety warning.

You may output multiple safety events in one batch, but:

- Do not duplicate events for trivially overlapping time\_windows describing the same hazard.
- If multiple fine-grained annotations describe the same continuous hazard, you may choose one representative time\_window.

⸻

\#\#\# Dialogue Generation Objective

For each Instant Safety episode, you must generate a short multi-turn dialogue that:

    1. Grounds in the specific hazard

    - The assistant should explicitly or implicitly mention:
        - the risky object or surface,
        - the relevant body part or position,
        - the immediate nature of the risk.
    - Examples:
        - “Watch your fingers; the knife blade is very close.”
        - “Be careful, the pot on your left is boiling and might splash.”
        - “There's liquid on the floor right where you're walking.”

    - Do not mention “video”, “annotations”, “models”, or internal logging.

    2. Keeps focus on the present moment

    - Make it clear that the warning is about what is happening right now, e.g.:
        - “As you reach across the stove…”
        - “Right in front of your feet there's a wet spot.”
        - “While you're plugging this in, the socket looks exposed.”

    3. Offers concrete, practical suggestions

    - Suggest one or two simple actions to reduce risk, such as:
        - adjusting grip or hand position,
        - stepping around a spill,
        - turning down the heat,
        - moving flammable items away,
        - unplugging or avoiding a damaged cable.

    4. Tone and emotional value

    - Calm, supportive, non-panicking.
    - Emphasize care and prevention, not blame:
        - “just so you don't get hurt,”
        - “to stay safe while you're doing this.”
    - Avoid scolding language (“you're being careless”); instead:
        - “If you slow down a bit and move your hand back…”
        - “You might want to wipe that up before you walk through.”

    5. Dialogue structure

    Each proactive\_dialogue should contain at least 2 turns, preferably 3-4:

        1. Assistant (Turn 1)  
        - Proactively issues a safety warning,
        - names or hints at the hazard,
        - and suggests a simple mitigating action.

        2. User (Turn 2)  
        - Natural reply (≥ 12 English words).
        - May:
            - acknowledge and adjust,
            - explain they already noticed,
            - ask for a specific suggestion,
            - or briefly decline (“I'm okay, but thanks for the reminder”).

        3. Assistant (optional Turn 3)  
        - Acknowledge the user's response,
        - offer a refined suggestion or reassurance,
        - or back off politely while keeping safety in mind.

        4. User (optional Turn 4)  
        - Short acknowledgement or final confirmation.

        Diversity
        Across different safety dialogues in the same output:
            - Vary how you phrase the warning:
            - “Be careful…”
            - “Watch out…”
            - “Just a heads-up…”
            - Vary the help framing:
            - “Maybe move your hand a little further back.”
            - “You could step around that spill.”
            - “It might be safer to turn the heat down a bit.”

Not every user must respond enthusiastically; some may give a brief answer or lightly downplay the risk.

⸻

\#\#\# Output Format

Your output MUST be ONE JSON object:

\{
  "service\_main\_type": "Instant Proactive Service",
  "service\_sub\_type": "Safety Proactive Service",

  "safety\_events": [
    \{
      "event\_id": "safety\_001",

      "current\_segment\_id": "\textless{}segment id where the assistant speaks\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "supporting\_source": "i\_do\_steps \textbar{} speakers\_say",

      "scene\_description": "\textless{}short neutral description of what the user is doing around this moment\textgreater{}",
      "trigger\_reason": "\textless{}why this moment is an Instant Safety opportunity, grounded in the annotations\textgreater{}",

      "hazard\_key": "\textless{}abstract description of the hazard, e.g., 'knife near fingers', 'spilled liquid underfoot'\textgreater{}",
      "hazard\_summary": "\textless{}short explanation of what is dangerous and why now\textgreater{}",
      "risk\_type": "cut \textbar{} burn \textbar{} slip \textbar{} collision \textbar{} electric\_shock \textbar{} other",
      "risk\_immediacy": "immediate",
      "potential\_consequence": "\textless{}optional: what could happen (scald, cut, fall, etc.)\textgreater{}",

      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}assistant issues an instant safety warning, grounded in the hazard and context\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}likely user reply (\textgreater{}= 12 English words)\textgreater{}"
        \}
        // optionally 1-2 more turns, alternating assistant ↔ user
      ]
    \}
  ]
\}

Notes:
- safety\_events may contain 0, 1, or multiple entries depending on how many Instant Safety opportunities exist in this batch.
- You may approximate the severity in potential\_consequence, but it must remain consistent with the annotations.

⸻

\#\#\# Failure Case Format

If you find no Instant Safety opportunities in the current batch:

\{
  "service\_main\_type": "Instant Proactive Service",
  "service\_sub\_type": "Safety Proactive Service",
  "safety\_events": [],
  "note": "No Instant Safety Proactive Service opportunities were detected in the current batch, given the current annotations."
\}
\end{promptbox}

\begin{promptbox}[EgoLife — Instant · Tool Use]
\#\#\# Task Context

You are analyzing MULTIPLE egocentric human annotation files (each less than 10 minutes) from the EgoLife dataset for one contiguous short-horizon batch (less than 2.5 hours).

Your job in this stage is signal mining and multi-turn dialogue generation for:

Instant Proactive Service
Subtype: Tool Use Proactive Service (“Tool Use”)

This service focuses on detecting suboptimal tool-use technique that:
	•	occurs during ongoing execution of a concrete task,
	•	does not create immediate physical danger (otherwise → Safety),
	•	can be corrected by small micro-action adjustments (grip / angle / force / motion), and
	•	benefits from a short, supportive assistant suggestion.

Tool Use is strictly about how to do a tool-related action — not about:
	•	whether the workflow step is correct (Error-Recovery),
	•	whether the state is dangerous (Safety),
	•	whether the user should move on to the next step (Next-Step Guidance), or
	•	whether the user forgot to close something (Resource Reminder).

⸻

\#\#\# Purpose of Tool Use

A Tool Use Proactive Service event is triggered when:
	•	The user is currently performing a correct step involving a specific physical tool, and
	•	Their grip / angle / stability / force / contact position / micro-motion is suboptimal, and
	•	The issue does not cause immediate serious injury risk (if yes → Safety), and
	•	The user's goal and workflow direction are correct (if wrong → Error-Recovery), and
	•	Fixing it requires only minor micro-action adjustments, not rollback or undo of previous steps.

This service should provide gentle, real-time technique optimization, similar to how an experienced coworker might say:
	•	“Hold it a little closer to the base—that'll be more stable.”
	•	“Your brush angle is quite flat; tilting it a bit will give better coverage.”
	•	“Your screwdriver grip looks a bit unsteady; try keeping your wrist straighter.”

⸻

\#\#\# Authoritative Timestamps \& Fine-Grained Evidence Priority

Each fine-grained annotation entry has a time\_window aligned to the original video, such as:
	•	i\_do\_steps[].time\_window
	•	speakers\_say[].time\_window

All time\_window strings already have the format:

DAY\# HH:MM:SS-HH:MM:SS

When you output current\_time\_window, you MUST:
	•	copy it only from:
	•	i\_do\_steps[].time\_window, or
	•	speakers\_say[].time\_window.

You must NOT use:
	•	interactions\_with\_objects[].time\_window,
	•	interactions\_with\_people[].time\_window,
	•	interaction\_records[].time\_window

as the source of current\_time\_window (although they can still provide contextual evidence that a tool is being used, and how).

You must NOT:
	•	fabricate new timestamps,
	•	merge multiple ranges,
	•	extend or shrink an existing range.

Fine-grained evidence priority

When detecting Tool Use technique issues, you must prioritize fine-grained entries:
	•	Primary sources for discovering tool-use technique episodes:
	•	i\_do\_steps
	•	interactions\_with\_objects
	•	interactions\_with\_people
	•	speakers\_say (if describing tool manipulation or technique)

You must tie each Tool Use event to one concrete fine-grained entry that clearly shows suboptimal technique. Do not infer from vague or long summaries alone.

⸻

\#\#\# Input Human Annotations

You are given MULTIPLE JSON objects, each representing a \textless{}10-minute egocentric segment:
\{
  "segment\_id": "\textless{}identifier for this \textasciitilde{}10-minute segment\textgreater{}",
  "description": "... high-level summary of what I do in this segment ...",
  "interaction\_records": [
    \{
      "time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "description": "... micro-episode summary ...",

      "i\_do\_steps": [ ... ],
      "speakers\_say": [ ... ],
      "interactions\_with\_objects": [ ... ],
      "interactions\_with\_people": [ ... ],
      "environment\_state": [ ... ],
      "task\_transition": [ ... ],
      "confidence": 0.0-1.0
    \}
  ]
\}
These interaction\_records and their subfields are your only evidence.

The coverage of this batch is defined by the minimum and maximum timestamps appearing in these JSONs.
You can assume this coverage is at most about 2.5 hours.

⸻

Service Category
	•	service\_main\_type: "Instant Proactive Service"
	•	service\_sub\_type: "Tool Use Proactive Service"

This service is distinct from:
	•	Error-Recovery (wrong object / step / configuration → requires rollback),
	•	Instant Safety (acute physical danger, e.g., cut / burn / shock / collision),
	•	Next-Step Guidance (what to do next in a workflow),
	•	Short-Term Resource Reminder (forgot to close / turn off / secure),
	•	Habit-Coaching / Long-Term (posture, long-term strain, lifestyle).

⸻

\#\#\# What counts as a Tool Use signal?

A Tool Use signal is valid when all of the following hold:

1. A specific physical tool is involved
Examples:
	•	knife, spatula, ladle, tongs, peeler,
	•	screwdriver, wrench, drill, scissors,
	•	brush, sponge, mop, squeegee,
	•	cleaning tools, small handheld devices, etc.

2. The action itself is correct
	•	The user is performing the right task and right step in the workflow.
	•	The chosen tool is appropriate for the task (not obviously wrong tool type).
	•	The current workflow state remains valid even if technique is not ideal.

3. The micro-technique is suboptimal
Look for concrete issues such as:
	•	grip is too far from the active end, reducing stability,
	•	tool angle is too shallow / too steep relative to the surface,
	•	wrist seems unstable or twisted,
	•	two-handed stabilization would clearly help but user uses one hand only,
	•	too little or too much force is applied,
	•	contact surface is uneven or only partially engaged,
	•	motion path is inefficient (e.g., large arm swings instead of small controlled motions).

4. The issue is fixable by micro-adjustments
	•	No rollback, undo, or step reset is required.
	•	Adjusting grip, angle, stance, or motion within the current step is enough to improve the outcome.

5. No acute physical hazard (otherwise → Safety)
If the same technique pattern also creates immediate bodily danger (cut, burn, shock, severe slip, collision within the next ≈0-10 seconds), then for this service it must be handled as Instant Safety, not Tool Use.

⸻

\#\#\# Distinction From Other Service Types

1. Tool Use vs. Error-Recovery (MOST IMPORTANT)
Error-Recovery occurs when:
	•	The user has made a workflow-level mistake:
	•	wrong object / wrong tool,
	•	wrong slot / wrong orientation,
	•	wrong step order or invalid configuration.
	•	The system is now in a wrong or invalid state.
	•	Fixing it requires rollback (undo/redo), not just better technique.
	•	Even perfect technique cannot fix the state.

Therefore, Tool Use MUST NOT be used when:
	•	The user selected the wrong item.
	•	The user inserted something into the wrong slot/orientation.
	•	A step must be undone before proceeding.
	•	The state is invalid even if technique becomes perfect.

Diagnostic question:

“If the user's technique becomes perfect from this moment on, will the underlying problem disappear?”

	•	Yes → Tool Use is possible (as long as state is valid).
	•	No → This is Error-Recovery, not Tool Use.

Examples of Error-Recovery (NOT Tool Use):
	•	Upside-down battery inserted into a device (must remove \& reinsert correctly).
	•	Wrong container used for a chemical step.
	•	Clearly wrong tool selected for the target (e.g., flat screwdriver in a Phillips screw).
	•	A component fully misaligned in a way that cannot be fixed by grip/angle alone.

⸻

2. Tool Use vs. Safety
Safety applies when:
	•	The technique issue causes immediate physical danger (cut, burn, slip, shock, collision) within the next ≈0-10 seconds.

If danger exists, then → ALWAYS Safety, NEVER Tool Use.

Examples that become Safety:
	•	Knife held close enough to cut the user's finger within a small motion.
	•	Hot pot / boiling liquid extremely close to bare skin.
	•	User touching or approaching exposed live wires.
	•	Heavy object visibly unstable and about to fall on or near the user.

⸻

3. Tool Use vs. Next-Step Guidance
If the user:
	•	is doing the correct step, but
	•	mainly needs help with what to do next in the sequence,

→ this is Next-Step Guidance, not Tool Use.

Tool Use = how to do the current tool action better.
Next-Step Guidance = what to do after this step.

⸻

4. Tool Use vs. Short-Term Resource Reminder
If the main issue is:
	•	forgetting to turn off a stove or power switch,
	•	leaving water running,
	•	leaving a tool powered on or a lid open,

→ this is Short-Term Resource Reminder, not Tool Use.

⸻

5. Tool Use vs. Habit-Coaching / Ergonomics
Long-term ergonomic concerns (e.g., posture at a desk, long-term strain, monitor distance) without a specific tool-use micro-technique in a concrete step → Habit-Coaching / Long-Term, not Tool Use.

Tool Use only addresses immediate technique optimization during an ongoing tool operation.

⸻

\#\#\# Short-Horizon Technique Window

Tool Use operates strictly within an instant, ultra-short-horizon window, reflecting local technique within an ongoing step.

The model must follow these temporal constraints:
	•	Immediate technique window (≈0-10 seconds)
	•	A Tool Use opportunity arises when the user is currently manipulating a tool,
	•	and the suboptimal technique is visible now or within the next few seconds.
	•	The assistant's suggestion is assumed to be delivered during the same short action phase, not minutes later.
	•	No long-horizon technique memory
	•	Do not reason over tool-use patterns older than \textasciitilde{}10 seconds as evidence for a Tool Use event.
	•	Do not chain across multiple distant clips or sessions.
	•	Tool Use must rely on local, immediate evidence within one short micro-episode.

⸻

\#\#\# Time-Window Rules

For every Tool Use event, you must define a single:
	•	current\_time\_window representing the short interval where the suboptimal technique occurs and where the assistant speaks up.

Rules:
	1.	Source of current\_time\_window
        •	You MUST copy current\_time\_window from exactly one of:
        •	i\_do\_steps[].time\_window, or
        •	speakers\_say[].time\_window.
        •	You must NOT use:
        •	interactions\_with\_objects[].time\_window,
        •	interactions\_with\_people[].time\_window,
        •	interaction\_records[].time\_window
    as the timestamp source for current\_time\_window.
	2.	Single moment only
        •	You must copy one existing time\_window string exactly.
        •	You must NOT:
        •	invent new time ranges,
        •	merge two ranges,
        •	extend or shorten an existing range.

The assistant's first proactive utterance is interpreted as happening during or immediately after this current\_time\_window.

⸻

\#\#\# Tool Use Detection Objective

For the given batch:
	1.	Scan all fine-grained entries (i\_do\_steps, interactions\_with\_objects, interactions\_with\_people, speakers\_say) to identify episodes where the user is clearly manipulating a tool.
	2.	For each candidate episode, check whether:
        •	The task and step are correct (no wrong-object / wrong-slot / wrong-order error).
        •	There is no acute physical hazard (otherwise → Safety).
        •	The main issue is a technique inefficiency (grip, angle, stability, force, motion, contact).
        •	Technique issues can be fixed by local micro-adjustments, with no rollback.
	3.	Filter out episodes where a different service is dominant:
        •	Safety (immediate bodily danger),
        •	Error-Recovery (invalid workflow state requiring undo),
        •	Short-Term Resource Reminder (forgotten closure),
        •	Next-Step Guidance (sequencing),
        •	Habit-Coaching / Long-Term (posture, lifestyle).
	4.	For each valid Tool Use episode:
        •	Select the most fine-grained i\_do\_steps or speakers\_say entry that best captures the problematic technique moment.
        •	Copy its time\_window as current\_time\_window.
        •	Record what tool is used, what the user is trying to do, and what technique issue appears.

⸻

\#\#\# Dialogue Generation Objective

For each Tool Use event, you must generate a short, natural multi-turn dialogue.

Assistant (Turn 1)
	•	Speaks first.
	•	Mentions or clearly implies the specific tool.
	•	Points out the technique issue in a neutral, descriptive way.
	•	Offers 1-2 concrete micro-adjustments (e.g., grip, angle, force, motion).

Examples:
	•	“If you hold the knife a bit closer to the handle base, it will feel more stable while you slice.”
	•	“Your wrist is quite bent while using the screwdriver; straightening it a little can give you better control.”
	•	“Right now the brush is almost flat; tilting it slightly will help the bristles reach the surface more evenly.”

Do not mention “video”, “annotations”, “dataset”, or internal processing.

⸻

User (Turn 2)
	•	Provides a natural reply (≥ 12 English words).
	•	May:
	•	acknowledge the suggestion and adjust,
	•	ask for clarification,
	•	say they prefer their current style,
	•	briefly explain what they're trying to achieve.

⸻

Assistant (optional Turn 3)
	•	Acknowledges the user's reaction.
	•	Either:
	•	refines the suggestion (more concrete), or
	•	supports the user's choice and gently closes the guidance.

⸻

User (optional Turn 4)
	•	Short acknowledgment or confirmation (e.g., “Got it, I'll try that grip now.”).

Tone:
	•	Helpful, calm, non-judgmental.
	•	Emphasize making the task easier or more stable, not blaming.
	•	Avoid scolding (“you are doing it wrong”); prefer supportive phrasing:
	•	“You might find it easier if…”
	•	“It may feel more stable when…”

⸻

\#\#\# Output Format

Your output MUST be exactly one JSON object:
\{
  "service\_main\_type": "Instant Proactive Service",
  "service\_sub\_type": "Tool Use Proactive Service",

  "tool\_use\_events": [
    \{
      "event\_id": "tooluse\_001",

      "current\_segment\_id": "\textless{}segment id\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "supporting\_source": "i\_do\_steps \textbar{} speakers\_say",

      "scene\_description": "\textless{}neutral description of what the user is doing with the tool\textgreater{}",
      "trigger\_reason": "\textless{}why this moment is a Tool Use technique issue (not Safety / not Error-Recovery)\textgreater{}",

      "tool\_name": "\textless{}knife / screwdriver / brush / sponge / etc.\textgreater{}",
      "technique\_issue": "\textless{}specific suboptimal technique (e.g., unstable wrist, angle too flat)\textgreater{}",
      "why\_suboptimal": "\textless{}why this technique reduces stability, efficiency, or quality\textgreater{}",
      "risk\_level": "low",
      "requires\_rollback": false,
      "is\_safe": true,

      "occurrence\_confidence": 0.0,

      "dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}concise, supportive technique advice\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}\textgreater{}=12-word natural reply\textgreater{}"
        \}
        // optional extra turns (assistant ↔ user)
      ]
    \}
  ]
\}

Notes:
	•	tool\_use\_events may contain 0, 1, or multiple entries depending on how many Tool Use opportunities are detected.
	•	supporting\_source MUST be "i\_do\_steps" or "speakers\_say", consistent with the allowed sources for current\_time\_window.

⸻

\#\#\#\# Failure Case Format

If no Tool Use opportunity exists in the current batch:
\{
  "service\_main\_type": "Instant Proactive Service",
  "service\_sub\_type": "Tool Use Proactive Service",
  "tool\_use\_events": [],
  "note": "No Tool Use technique issues were detected in the current batch, given the current annotations."
\}
\end{promptbox}

\begin{promptbox}[EgoLife — Short-Horizon · Error-Recovery]
\#\#\# Task Context

You are analyzing MULTIPLE egocentric annotation files (each less than 10 minutes) from the EgoLife dataset for one contiguous batch of time (the actual span is determined by the timestamps in the input, typically ≤ 2.5 hours).

Your job in this stage is signal mining and dialogue generation for a special Short-term Proactive Service subtype:

Short-term Error-Recovery Proactive Service
(short: Short-term Error-Recovery)

This service focuses on workflow-level mistakes inside ongoing tasks with short-term window (10s-10min), where:
	•	The user is performing a multi-step task or configuration workflow.
	•	The annotations show that they have entered a wrong state, used the wrong object/target, or executed the wrong step.
	•	Correcting the situation requires the user to roll back to an earlier valid state (undo or revert) and then redo the step correctly, not just adjust technique.
	•	A timely assistant reminder can help the user fix the mistake before it propagates (wasted effort, invalid results, broken setup, etc.).

Typical examples:
	•	The user inserts a battery in the wrong orientation and needs to remove it and reinsert it correctly.
	•	The user pours a liquid into the wrong container and must pour it back or restart in the correct container.
	•	The user selects the wrong menu option or mode in a multi-step configuration flow and must undo and re-select the correct one.
	•	The user plugs a cable into the wrong port or attaches the wrong adapter and must detach it and reconnect to the intended interface.
	•	The user performs “step 3” of a procedure without having done “step 2”, and must roll back to the correct step order.

You must:
	1.	Scan the current batch to detect short-term error-recovery opportunities grounded in the annotations.
	2.	For each error, select the current moment where:
		•	the wrong state is already present,
		•	continuing from this state would propagate or lock in the mistake, and
		•	a rollback reminder would still be timely and helpful.
	3.	For each such moment, generate a short multi-turn dialogue where the assistant:
		•	points out the workflow error,
		•	suggests how to undo or roll back,
		•	and offers concrete steps to redo the action correctly.

There is no historical memory JSON for this service:
	•	You treat each batch independently.
	•	You do not track cross-day or long-horizon workflows.
	•	You only output dialogues for this batch, each grounded in one current error-recovery episode.

You must NOT guess new errors, invent timestamps, or hallucinate behaviors not supported by the annotations.

⸻

\#\#\# Authoritative Timestamps \& Fine-Grained Evidence Priority

Each fine-grained annotation entry has a time\_window aligned to the original video, for example:
	•	i\_do\_steps[].time\_window
	•	interactions\_with\_objects[].time\_window
	•	interactions\_with\_people[].time\_window
	•	speakers\_say[].time\_window

All time\_window strings already have the format:

DAY\# HH:MM:SS-HH:MM:SS

When you output current\_time\_window, you MUST copy it only from i\_do\_steps[].time\_window or speakers\_say[].time\_window.
You must NOT use interactions\_with\_objects, interactions\_with\_people, or interaction\_records as the source of current\_time\_window.
Do NOT interpolate, merge, extend, shrink, or invent new time ranges.

\#\#\#\# Fine-grained evidence priority

When detecting Short-term Error-Recovery opportunities, you must prioritize fine-grained entries:
	•	i\_do\_steps
	•	interactions\_with\_objects
	•	interactions\_with\_people
	•	speakers\_say

Treat a fine-grained entry as a potential Error-Recovery episode only if its content clearly indicates a wrong step, wrong object, wrong target, wrong configuration, or invalid workflow state.

This priority applies both to:
	•	which content you treat as the error episode, and
	•	which time\_window you copy for that episode.

⸻

\#\#\# Input Human Annotations

You are given MULTIPLE JSON objects, each representing a \textless{}10-minute egocentric segment:
\{
  "segment\_id": "\textless{}identifier for this \textasciitilde{}10-minute segment\textgreater{}",
  "description": "... high-level summary of what I do in this segment ...",
  "interaction\_records": [
    \{
      "time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "description": "... micro-episode summary ...",

      "i\_do\_steps": [ ... ],
      "speakers\_say": [ ... ],
      "interactions\_with\_objects": [ ... ],
      "interactions\_with\_people": [ ... ],
      "environment\_state": [ ... ],
      "task\_transition": [ ... ],
      "confidence": 0.0-1.0
    \}
  ]
\}

These interaction\_records and their subfields are your only evidence.

The coverage of this batch is defined by the minimum and maximum timestamps appearing in these JSONs.
You can assume this coverage is at most about 2.5 hours.

⸻

Service Category
	•	service\_main\_type: “Short-term Proactive Service”
	•	service\_sub\_type: “Error-Recovery Proactive Service”

Note: this service operates on short-term, local workflow mistakes that require rollback + redo, and is distinct from:
	•	Instant Safety (immediate physical injury risk),
	•	Tool Use (suboptimal technique when the workflow state is still valid),
	•	Episodic Task Reminder (unfinished tasks inside one episode),
	•	Episodic Memory Recall (short-horizon episodic memory across ≤2 hours),
	•	Habit-Coaching or Long-Term services (chronic posture or lifestyle issues),
	•	Long-Horizon Memory-Link (cross-day or ≥2h memory links).

⸻

\#\#\# What counts as an Short-term Error-Recovery signal?

An Short-term Error-Recovery opportunity is defined by one current error episode, characterized by:

1. A concrete workflow error
The annotations indicate that the user has:
	•	chosen the wrong object or resource (wrong container, wrong tool, wrong component),
	•	executed a wrong step of a procedure,
	•	applied a wrong configuration (incorrect setting, mode, or parameter),
	•	inserted or attached something in an invalid way (wrong orientation, wrong port),
	•	or otherwise put the system into an invalid or undesired state that does not match the intended workflow.

2. Recovery requires rollback, not just technique adjustment
To proceed correctly, the user must:
	•	undo or reverse an action (e.g., remove the battery, detach the connector),
	•	move something back to an earlier valid resource (e.g., pour liquid back, move items back),
	•	revert a setting (e.g., switch mode back, uncheck a wrong option),
	•	or go back to a previous step and repeat correctly.

If the situation can be fully fixed by small technique adjustments (changing grip, angle, speed) while staying in the same workflow state, it is not Error-Recovery; it belongs to Tool Use.

3. No acute physical hazard (otherwise → Safety)
If the same wrong step also creates immediate physical risk (cut, burn, shock, collision within a few seconds), then it should be treated as Instant Safety, not Error-Recovery.

4. Not a purely missing step (otherwise → Episodic Task Reminder)
If the issue is that the user never performed a required step and is now moving away (unfinished task), but they are not in an invalid state that requires rollback, this belongs to Episodic Task Reminder, not Error-Recovery.

5. Not a long-horizon or habit issue
Long-term posture, repeated strain, or lifestyle risk without an explicit wrong step in a multi-step workflow belongs to other services (Habit-Coaching, Long-Term), not Error-Recovery.

⸻

\#\#\# Mutual Exclusion \& Priority vs. Other Services

Use these rules to distinguish Error-Recovery from other proactive services:

1. Error-Recovery vs. Tool Use  (critical distinction)
This is the most important boundary and must be enforced strictly.
	•	Tool Use:
		•	The user is performing the correct task and correct step, but with suboptimal technique.
		•	Examples: unstable grip on a screwdriver, holding a knife awkwardly, standing in a position that makes leverage poor.
		•	The workflow state is valid; the result might be less efficient or less precise, but does not require undoing previous steps.
		•	The assistant message sounds like:
			•	“Hold it this way for better control.”
			•	“If you adjust your angle, it will be easier.”
	•	Error-Recovery:
		•	The user has performed a wrong step or wrong choice, or created an invalid system state.
		•	Technique changes alone cannot fix it; the user must roll back (undo or revert) and redo correctly.
		•	The assistant message sounds like:
			•	“You might have placed this in the wrong slot; you may want to remove it and connect it to the other one.”
			•	“This liquid went into the wrong container; you could pour it back and use the labeled cup instead.”

A useful test:  If perfect technique from this point on would still leave the system in the wrong state, it is Error-Recovery, not Tool Use.

2. Error-Recovery vs. Instant Safety
	•	Instant Safety: main concern is immediate physical injury (cut, burn, slip, collision, electric shock) in the next few seconds.
	•	Error-Recovery: main concern is task correctness and valid workflow state; consequences are incorrect results, wasted effort, or broken setup, not immediate bodily harm.

If a wrong step also causes acute danger (e.g., mis-wiring near exposed live contacts), classify as Safety for this Short-term Proactive Service.

3. Error-Recovery vs. Episodic Task Reminder
	•	Episodic Task Reminder: the user has not yet completed a task or planned step within the episode and is switching away, but the current state is not necessarily invalid. A reminder is about finishing a missing step.
	•	Error-Recovery: the user has already performed a wrong step or wrong choice that must be undone; the reminder is about rolling back and correcting the workflow.

4. Error-Recovery vs. Next-Step Guidance
	•	Next-Step Guidance: the user is in a valid state and simply needs help deciding or remembering what the next correct step should be.
	•	Error-Recovery: the user is in an invalid state and must go backwards before any next step makes sense.

5. Error-Recovery vs. Habit-Coaching / Long-Term
	•	Long-term patterns (working posture, screen distance, frequency of breaks) without a specific wrong step in a concrete workflow should not be labeled Error-Recovery.

⸻


\#\#\# Time-Window Rules

For every Short-term Error-Recovery dialogue you output, you must define a single:
	•	current\_time\_window representing the error episode and the moment when the assistant speaks.

Rollback Memory Horizon (critical)
When determining whether a rollback is needed and which earlier step/state it depends on, you must follow these temporal limits:
	•	The relevant earlier step or valid state must end within 10 seconds to 5 minutes before the current\_time\_window.
	•	In all cases, you must never use evidence older than 10 minutes when establishing the rollback chain.
	•	If the only correct reference state is older than this horizon, you must not classify the situation as Short-term Error-Recovery (it belongs to long-horizon services instead).

Rules:
	1.	Current time window (current\_time\_window)
		•	Prefer to copy from one fine-grained entry’s time\_window:
		•	i\_do\_steps[].time\_window, or
		•	speakers\_say[].time\_window.
		•	Do NOT merge or fabricate new ranges.
	2.	Instant horizon
		•	current\_time\_window should correspond to the short segment where:
			•	the incorrect state is present and visible in the annotations, and
			•	a rollback reminder would still be in time to prevent the error from propagating.

The assistant’s first proactive utterance is interpreted as happening during or immediately after this current\_time\_window.

⸻

\#\#\# Short-term Error-Recovery Detection Objective

For the current batch (no external history):
	1.	Scan all segments and interaction\_records to find candidate error episodes where:
		•	fine-grained annotations describe a wrong object, wrong step, wrong configuration, invalid connection, or invalid state.
	2.	For each candidate, verify that:
		•	There is a specific workflow error (wrong resource, wrong step, wrong orientation, wrong target).
		•	Technique adjustments alone cannot fully fix it; rollback is required.
		•	There is no immediate physical danger (otherwise → Safety).
		•	The situation is not purely a missing step where the user is walking away (otherwise → Episodic Task Reminder).
	3.	For each valid error episode:
		•	Choose the most fine-grained time\_window capturing the error moment.
		•	Record the local scene context and a short explanation of what is wrong and what must be undone.
	4.	For each such episode, generate:
		•	One structured Short-term Error-Recovery entry with:
		•	current\_segment\_id, current\_time\_window, supporting\_source,
		•	a neutral scene description,
		•	error\_key, error\_summary, rollback\_required, rollback\_reason,
		•	occurrence\_confidence.
		•	One multi-turn dialogue where the assistant suggests rolling back and redoing correctly.

You may output multiple error\_recovery\_events in one batch, but:
	•	Do not duplicate events for trivially overlapping time\_windows describing the same error.
	•	If multiple fine-grained annotations describe the same continuous error, you may choose one representative time\_window.

⸻

\#\#\# Dialogue Generation Objective

For each Short-term Error-Recovery episode, you must generate a short multi-turn dialogue that:
	1.	Grounds in the specific workflow error
		•	The assistant should explicitly or implicitly mention:
		•	what was done incorrectly (wrong object/step/setting/orientation),
		•	why this state is invalid for the task,
		•	and that going back one step will help.
		•	Examples:
		•	“It looks like this cable is connected to the other port; you might want to move it to the port labeled X instead.”
		•	“You poured this into the unlabeled cup; the instructions refer to the marked measuring cup. You could pour it back and use that one.”
		•	“This battery seems reversed; you may want to remove it and reinsert it with the plus side aligned to the mark.”
		•	Do not mention “video”, “annotations”, “models”, or internal logging.
	2.	Keeps focus on the current moment
		•	Make it clear that the guidance is about the error as it exists now, e.g.:
		•	“Before you continue with the next step…”
		•	“Right now, this setting doesn’t match the intended mode.”
		•	“As it’s currently connected, this won’t work as expected.”
	3.	Offers concrete rollback actions
		•	Suggest one or two simple steps to revert and redo:
		•	remove / detach / undo,
		•	move back / revert to previous container or location,
		•	change setting back to default and reselect,
		•	go back to the missing or correct step.
	4.	Tone and emotional value
		•	Calm, non-judgmental, supportive.
		•	Emphasize helping the user avoid wasted effort or confusion:
		•	“so you don’t have to redo everything later,”
		•	“to keep this setup consistent with the instructions.”
		•	Avoid scolding language (“you did it wrong again”); instead:
		•	“If you’d like, you can undo this step and try it this way…”
		•	“You might want to adjust this before moving on.”
	5.	Dialogue structure

		Each proactive\_dialogue should contain at least 2 turns, preferably 3-4:
		1.	Assistant (Turn 1)
			•	Proactively identifies the error,
			•	explains that rollback will help,
			•	and suggests specific recovery actions.
		2.	User (Turn 2)
			•	Natural reply (≥ 12 English words).
			•	May:
			•	accept and undo the step,
			•	partially accept (e.g., ask for details),
			•	decline (“I intended to do it this way”),
			•	or clarify the goal.
		3.	Assistant (optional Turn 3)
			•	Acknowledge the user’s choice,
			•	provide more precise guidance, or
			•	gracefully back off if the user declines.
		4.	User (optional Turn 4)
			•	Short acknowledgment or final confirmation.

	Diversity

	Across different error-recovery dialogues in the same output:
		•	Vary how you introduce the rollback:
		•	“You might want to undo this step…”
		•	“Before you go on, it could help to reverse that…”
		•	“It may work better if you go back one step and adjust this.”
		•	Vary how you describe the benefit:
		•	“to match the intended setup,”
		•	“so the result follows the instructions,”
		•	“so you don’t need to redo more work later.”

	Not every user must comply; some may choose to proceed intentionally.

⸻

\#\#\# Output Format

Your output MUST be ONE JSON object:
\{
  "service\_main\_type": "Short-term Proactive Service",
  "service\_sub\_type": "Error-Recovery Proactive Service",

  "error\_recovery\_events": [
    \{
      "event\_id": "erecovery\_001",

      "current\_segment\_id": "\textless{}segment id where the assistant speaks\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "supporting\_source": "i\_do\_steps \textbar{} speakers\_say",

      "scene\_description": "\textless{}short neutral description of what the user is doing around this moment\textgreater{}",
      "trigger\_reason": "\textless{}why this moment is an Error-Recovery opportunity, grounded in the annotations\textgreater{}",

      "error\_key": "\textless{}abstract description of the workflow error, e.g., 'wrong container', 'incorrect orientation', 'wrong port', 'invalid step order'\textgreater{}",
      "error\_summary": "\textless{}short explanation of what is wrong and why rollback is needed\textgreater{}",
      "rollback\_required": true,
      "rollback\_reason": "\textless{}why the user needs to undo and redo the step instead of only adjusting technique\textgreater{}",
      "risk\_type": "workflow\_error",
      "risk\_immediacy": "immediate",
      "potential\_downstream\_issue": "\textless{}optional: what could happen if the user continues without fixing it (invalid result, wasted effort, etc.)\textgreater{}",

      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}assistant issues rollback guidance, grounded in the error and context\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}likely user reply (\textgreater{}= 12 English words)\textgreater{}"
        \}
        // optionally 1-2 more turns, alternating assistant ↔ user
      ]
    \}
  ]
\}

Notes:
	•	error\_recovery\_events may contain 0, 1, or multiple entries depending on how many Short-term Error-Recovery opportunities exist in this batch.
	•	potential\_downstream\_issue is optional and should stay consistent with the annotations (e.g., “measurement result may be invalid”, “mixture may not follow the intended recipe”).

⸻

\#\#\#\# Failure Case Format

If you find no Short-term Error-Recovery opportunities in the current batch:
\{
  "service\_main\_type": "Short-term Proactive Service",
  "service\_sub\_type": "Error-Recovery Proactive Service",
  "error\_recovery\_events": [],
  "note": "No Short-term Error-Recovery Proactive Service opportunities were detected in the current batch, given the current annotations."
\}
\end{promptbox}

\begin{promptbox}[EgoLife — Short-Horizon · Next-Step Guidance]
\#\#\# Task Context

You are analyzing MULTIPLE egocentric annotation files (each less than 10 minutes) from the EgoLife dataset for one contiguous batch of time (typically ≤ 2.5 hours).

Your job in this stage is signal mining and dialogue generation for a special Short-term Proactive Service subtype:

Next-Step Guidance Proactive Service
(short: Next-Step Guidance)

This service is triggered after the user completes a correct step, in a workflow where the next step is:
	•	logically required,
	•	sequential,
	•	and immediately actionable within a short-horizon window (≈10 seconds-10 minutes).

The assistant gives the user the next logical step to continue the multistep workflow smoothly.

Typical examples:
	•	The user finishes chopping vegetables → assistant suggests “you can heat the pan now.”
	•	The user completes reagent preparation → assistant suggests the next experiment step.
	•	The user finishes assembling a part → assistant reminds them of the next continuation step.

This service is not about correcting mistakes, preventing danger, or adjusting technique.
It is simply about what comes next, assuming the current step is correct and valid.

⸻

\#\#\# Authoritative Timestamps \& Fine-Grained Evidence Priority

Each fine-grained annotation entry has a time\_window aligned to the original video, e.g.:
	•	i\_do\_steps[].time\_window
	•	speakers\_say[].time\_window
	•	interactions\_with\_objects[].time\_window
	•	interactions\_with\_people[].time\_window

All time\_window strings already have the format:

DAY\# HH:MM:SS-HH:MM:SS

When you output current\_time\_window, you MUST:
	•	copy it only from:
	•	i\_do\_steps[].time\_window, or
	•	speakers\_say[].time\_window.

You must NOT use interactions\_with\_objects, interactions\_with\_people, or interaction\_records as the source of current\_time\_window (though they can still be used as content evidence for detecting steps and workflows).

Do NOT interpolate, merge, extend, shrink, or invent new time ranges.

Fine-grained evidence priority

When detecting Next-Step Guidance opportunities, you must prioritize fine-grained entries:
	•	Primary sources for detecting steps and workflow structure:
	•	i\_do\_steps
	•	interactions\_with\_objects
	•	interactions\_with\_people
	•	speakers\_say

Treat a fine-grained entry (or short sequence of entries) as a potential Next-Step episode only if its content clearly indicates:
	•	a correctly completed step in a multi-step workflow, and
	•	a natural “what’s next?” moment (pause, idle, or transition).

This priority applies both to:
	•	which content you treat as the completed-step episode, and
	•	which time\_window you copy (from i\_do\_steps or speakers\_say) for that episode as current\_time\_window.

⸻

\#\#\# Input Human Annotations

You are given MULTIPLE JSON objects, each representing a \textless{}10-minute egocentric segment:
\{
  "segment\_id": "\textless{}identifier for this \textasciitilde{}10-minute segment\textgreater{}",
  "description": "... high-level summary of what I do in this segment ...",
  "interaction\_records": [
    \{
      "time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "description": "... micro-episode summary ...",

      "i\_do\_steps": [ ... ],
      "speakers\_say": [ ... ],
      "interactions\_with\_objects": [ ... ],
      "interactions\_with\_people": [ ... ],
      "environment\_state": [ ... ],
      "task\_transition": [ ... ],
      "confidence": 0.0-1.0
    \}
  ]
\}

These interaction\_records and their subfields are your only evidence.

The coverage of this batch is defined by the minimum and maximum timestamps appearing in these JSONs.
You can assume this coverage is at most about 2.5 hours.

⸻

Service Category
	•	service\_main\_type: "Short-term Proactive Service"
	•	service\_sub\_type: "Next-Step Guidance Proactive Service"

This service is distinct from:
	•	Error-Recovery (wrong step → rollback),
	•	Tool Use (correct step but poor technique),
	•	Instant Safety (physical hazard),
	•	Episodic Task Reminder (unfinished tasks across an episode),
	•	Habit-Coaching / Long-Term,
	•	Long-Horizon Memory-Link (≥ 2h or cross-day).

⸻

\#\#\# What counts as a Next-Step Guidance signal?

A Next-Step Guidance opportunity must satisfy all of the following:

⸻

1. The user has just completed a correct step
Evidence from fine-grained annotations shows:
	•	correct object usage,
	•	correct manipulation,
	•	correct preparation step,
	•	correct mode selection,
	•	correct assembly action.

The step is valid, successful, and brings the workflow forward.

⸻

2. The task is clearly a multistep sequential workflow
Examples:
	•	cooking / preparation sequences,
	•	DIY / assembly processes,
	•	experiment procedures,
	•	device setup flows,
	•	multi-step maintenance tasks.

The workflow must have forward continuity: a natural “what’s next?” moment.

⸻

3. The user is in a state that suggests readiness for the next step
For example:
	•	the user pauses after a correct step,
	•	looks around for what to do next,
	•	the workflow obviously continues but the user is idle,
	•	or the last step’s objective is clearly achieved (e.g., lid tightened, item cleaned, button pressed).

This service triggers when user intent likely requires continuation, not rollback or abandonment.

⸻

\#\#\# What does NOT count as Next-Step Guidance?

1. Wrong step was performed → Error-Recovery
If the user:
	•	picked the wrong object,
	•	performed the wrong step,
	•	created an invalid configuration,

then the assistant must instruct rollback (Error-Recovery), not next step.

⸻

2. Technique is poor → Tool Use
If the user:
	•	holds a tool at a poor angle,
	•	performs a valid step but inefficiently,

this is Instant Tool Use, not Next-Step Guidance.

⸻

3. Immediate danger appears → Instant Safety
If a risky configuration arises (burn, cut, slip, shock risk):

→ classify as Instant Safety, not Next-Step Guidance.

⸻

4. User is abandoning an unfinished task → Episodic Task Reminder
Next-Step Guidance is used only when:
	•	the user is still within the workflow,
	•	and should proceed forward.

If the user walks away with an unfinished step → Episodic Task Reminder, not Next-Step Guidance.

⸻

\#\#\# Mutual Exclusion \& Priority

This section explains how to distinguish Next-Step Guidance from adjacent types.

Next-Step vs. Error-Recovery
	•	Next-Step:
        •	previous step is correct,
        •	workflow state is valid,
        •	next action naturally follows,
        •	no rollback required.
	•	Error-Recovery:
        •	previous step is incorrect OR created an invalid state,
        •	workflow requires rollback to repair,
        •	next logical step would fail if executed now.

Test:

“If the user proceeds without undoing anything, will the workflow still be valid?”
If NO → Error-Recovery.

⸻

Next-Step vs. Tool Use
	•	Tool Use:
        •	correct step is in progress,
        •	technique is suboptimal,
        •	assistant says “how to do”.
	•	Next-Step:
        •	step is complete,
        •	next step is “what to do next”.

⸻

Next-Step vs. Instant Safety
	•	If danger in the next 0-10 seconds → Safety.
	•	If safe and user is waiting/transitioning → Next-Step Guidance.

⸻

\#\#\# Time-Window Rules

For every Next-Step Guidance dialogue you output, you must define a single:
	•	current\_time\_window representing the short interval where the user has just completed a correct step and is ready for the next one, and the moment when the assistant speaks.

Rules:
	1.	Source of current\_time\_window
        •	You MUST copy current\_time\_window only from:
            •	i\_do\_steps[].time\_window, or
            •	speakers\_say[].time\_window.
        •	You must NOT use:
            •	interactions\_with\_objects[].time\_window,
            •	interactions\_with\_people[].time\_window,
            •	interaction\_records[].time\_window
        as the source for current\_time\_window (though they may still inform your understanding of the workflow).
        •	Never merge, fabricate, extend, or shrink time ranges.
	2.	Short-term next-step micro-interval
        •	A Next-Step moment corresponds to the short interval (≈0-10 seconds) immediately after the user finishes a correct step and is paused, waiting, or naturally transitioning.
        •	Choose the time\_window that best captures when the step is completed and the assistant’s suggestion would be timely.

⸻

\#\#\# Short-Horizon Memory Window

Next-Step Guidance operates strictly within a short-horizon memory range, reflecting short-term reasoning inside one continuous local workflow. The model must follow these temporal constraints:
	•	Immediate window (≈10 seconds)
If the user finishes a correct step and within ≈10 seconds pauses or appears to look for what to do next, treat this as a strong Next-Step Guidance opportunity.
	•	Typical short-horizon span (≈10 seconds - 5 minutes)
You may link the earlier step completion to the current pause/transition only if both belong to the same continuous workflow and fall within this short span (≤ 5 minutes).
	•	Maximum allowed memory span: 10 minutes
	•	You must not use any step completion older than 10 minutes as evidence for Next-Step Guidance.
	•	If the relevant earlier step happened more than ≈10 minutes ago or in a previous episode, it is not eligible for this service.
	•	No long-horizon or cross-episode reasoning
Do not retrieve step information from previous activities, earlier times of day, or different sessions.
Next-Step Guidance must rely exclusively on short-horizon evidence within the current local episode.

⸻

\#\#\# Next-Step Guidance Detection Objective

For the current batch:
	1.	Scan all fine-grained annotations for completed correct steps in clearly sequential workflows.
	2.	For each candidate, verify that:
        •	The step was correctly executed (no error requiring rollback).
        •	The workflow is multistep and sequential.
        •	The user is in a pause / wait / transition state suggesting readiness for the next step.
        •	There is no concurrent safety risk dominating the situation.
        •	There is no incorrect step that must be fixed first (no Error-Recovery).
        •	No tool-usage problem dominates (i.e., technique is not the main issue).
        •	The earlier step completion and the current pause/transition lie within the 10 seconds-10 minutes short-horizon window (ideally 10s-5min).
	3.	Choose the best fine-grained time\_window (from i\_do\_steps or speakers\_say) for the moment just after step completion as current\_time\_window.
	4.	For each valid Next-Step episode, construct:
        •	scene\_description (neutral description of what step the user just completed),
        •	trigger\_reason (why this moment qualifies as Next-Step Guidance),
        •	next\_step\_key,
        •	next\_step\_summary,
        •	occurrence\_confidence.
	5.	Generate a short multi-turn dialogue grounded in this context.

        \#\#\# Dialogue Generation Objective

        Each Next-Step Guidance episode requires a short dialogue:

        Assistant (Turn 1)
            •	Proactively proposes the next logical step,
            •	connects it explicitly to the step just completed,
            •	gives simple, practical guidance.

        Examples:
            •	“Since you’ve just finished chopping the vegetables, you can start heating the pan now.”
            •	“You’ve prepared the reagent; next you can pour it into the labeled tube.”
            •	“You finished attaching that part; now the next screw goes into the top-right hole.”

        Avoid mentioning videos, annotations, or datasets.

        ⸻

        User (Turn 2)

        A natural response (≥ 12 English words), such as:
            •	acknowledging the suggestion,
            •	asking how to proceed in more detail,
            •	confirming intention,
            •	or briefly explaining their plan.

        ⸻

        Assistant (optional Turn 3)

        Provides additional clarification, step-by-step instruction, or encouragement, or gracefully backs off if the user declines.

        ⸻

        User (optional Turn 4)

        Final acknowledgment or confirmation.

        Tone should be:
            •	calm,
            •	supportive,
            •	non-overbearing,
            •	focused on smooth task continuation.

⸻

\#\#\# Output Format

Your output MUST be exactly one JSON object:

\{
  "service\_main\_type": "Short-term Proactive Service",
  "service\_sub\_type": "Next-Step Guidance Proactive Service",

  "next\_step\_events": [
    \{
      "event\_id": "nextstep\_001",

      "current\_segment\_id": "\textless{}segment id\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "supporting\_source": "i\_do\_steps \textbar{} speakers\_say",

      "scene\_description": "\textless{}neutral description of what step the user just completed\textgreater{}",
      "trigger\_reason": "\textless{}why this moment qualifies as Next-Step Guidance\textgreater{}",

      "next\_step\_key": "\textless{}short tag: 'heat\_pan', 'tighten\_next\_screw', 'select\_mode', etc.\textgreater{}",
      "next\_step\_summary": "\textless{}the next action the user can take\textgreater{}",
      "workflow\_continuity": "sequential",
      "risk\_immediacy": "none",
      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}assistant gives next step\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}user reply (\textgreater{}= 12 words)\textgreater{}"
        \}
        // optional further turns
      ]
    \}
  ]
\}

Notes:
	•	next\_step\_events may contain 0, 1, or multiple entries depending on how many Next-Step Guidance opportunities exist in this batch.
	•	supporting\_source MUST be either "i\_do\_steps" or "speakers\_say", consistent with the allowed sources for current\_time\_window.

⸻

\#\#\#\# Failure Case Output

If no Next-Step Guidance opportunities are detected:
\{
  "service\_main\_type": "Short-term Proactive Service",
  "service\_sub\_type": "Next-Step Guidance Proactive Service",
  "next\_step\_events": [],
  "note": "No Next-Step Guidance opportunities were detected in this batch, given the current annotations."
\}
\end{promptbox}

\begin{promptbox}[EgoLife — Short-Horizon · Resource Reminder]
\#\#\# Task Context

You are analyzing MULTIPLE egocentric annotation files (each less than 10 minutes) from the EgoLife dataset for one contiguous batch of time (the batch span is determined by timestamps in the input, typically ≤ 2.5 hours).

Your job in this stage is signal mining and proactive dialogue generation for:

Short-Term Resource Reminder Proactive Service
(short: Resource Reminder)

This service focuses on short-horizon (≈10 seconds-10 minutes) mismanaged resources or incomplete closure tasks within the current episode (≤2.5 hours), where:
	•	The user has likely forgotten to close, shut off, secure, lock, or finalize a resource or state.
	•	The risk is not immediately physically dangerous (otherwise it belongs to Safety).
	•	The reminder helps the user avoid loss, damage, or unnecessary rework within the same short episode.
	•	The model must identify “closure failures” that the user is about to leave behind, based only on short-horizon evidence.

Typical examples:
	•	Forgetting to turn off a stove burner (low flame, no overflow → not yet Safety).
	•	Forgetting to turn off electrical power or water source.
	•	Leaving a document unsaved before walking away from a computer.
	•	Leaving a door not fully closed.
	•	Leaving a bottle cap loosely attached.
	•	Throwing trash away but forgetting to close the trash-can lid.

You must:
	1.	Scan the current batch to detect resource mismanagement or incomplete closure tasks grounded in the annotations.
	2.	For each case, identify the current moment where:
        •	the resource/state is left unresolved, and
        •	the user is transitioning away or about to shift context (within the short-horizon window).
	3.	Generate a short multi-turn dialogue where the assistant:
        •	proactively reminds the user of the unresolved task,
        •	explains why it matters right now,
        •	encourages a quick fix that avoids loss/damage/rework.

There is no long-term memory JSON for this service:
	•	You treat each batch independently.
	•	You do not consider cross-day or long-horizon tasks.
	•	You only output reminders for this batch, each tied to one current unresolved resource state.

The assistant must NOT hallucinate new states, objects, hazards, timestamps, or intentions.

⸻

\#\#\# Authoritative Timestamps \& Fine-Grained Evidence Priority

Each fine-grained annotation entry has a time\_window aligned to the original video, for example:
	•	i\_do\_steps[].time\_window
	•	interactions\_with\_objects[].time\_window
	•	interactions\_with\_people[].time\_window
	•	speakers\_say[].time\_window

All time\_window strings already have the format:

DAY\# HH:MM:SS-HH:MM:SS

When you output current\_time\_window, you MUST copy it only from i\_do\_steps[].time\_window or speakers\_say[].time\_window.
You must NOT use interactions\_with\_objects, interactions\_with\_people, or interaction\_records as the source of current\_time\_window.
Do NOT interpolate, merge, extend, shrink, or invent new time ranges.

Fine-grained evidence priority
	•	Use fine-grained subfields (i\_do\_steps, interactions\_with\_objects, interactions\_with\_people, speakers\_say) as the primary sources to detect potential short-term resource issues and to select current\_time\_window.
	•	Only fall back to interaction\_records.description and interaction\_records.time\_window when necessary (no fine-grained entry clearly reflects the unresolved resource or transition-away moment).

⸻

\#\#\# Input Human Annotations

You are given multiple JSON annotation files:
\{
  "segment\_id": "\textless{}segment id\textgreater{}",
  "description": "... high-level summary ...",
  "interaction\_records": [
    \{
      "time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "description": "... micro-episode summary ...",

      "i\_do\_steps": [ ... ],
      "speakers\_say": [ ... ],
      "interactions\_with\_objects": [ ... ],
      "interactions\_with\_people": [ ... ],
      "environment\_state": [ ... ],
      "task\_transition": [ ... ],
      "confidence": 0.0-1.0
    \}
  ]
\}

These are your only evidence sources for detection.

The coverage of this batch is defined by the minimum and maximum timestamps appearing in these JSONs.
You can assume this coverage is at most about 2.5 hours.

⸻

Service Category
	•	service\_main\_type: "Short-term Proactive Service"
	•	service\_sub\_type: "Short-Term Resource Reminder Proactive Service"

This service is distinct from:
	•	Next-Step Guidance (which helps continue a workflow),
	•	Error-Recovery (rollback to previous step),
	•	Tool Use (micro-action correction),
	•	Safety (immediate bodily danger),
	•	Long-Term Habit Coaching (chronic patterns),
	•	Long-Horizon Memory-Link (≥2 hours or cross-day).

⸻

\#\#\# What counts as a Short-Term Resource Reminder signal?

A resource reminder opportunity arises when ALL of the following hold:
	1.	There exists an unresolved resource / closure state
        Examples:
            •	A stove burner is still on.
            •	Water faucet left running or dripping.
            •	Computer document unsaved while user moves away.
            •	Trash-can lid open after throwing trash.
            •	Bottle cap loose after a sealing attempt.
            •	Power switch left on after using a tool.
            •	A door left ajar.

	2.	User is transitioning away
        Signals include:
            •	User moves to another room.
            •	User starts a different task.
            •	User stops interacting with the resource.
            •	User’s attention shifts to another device, person, or object.

	3.	The situation does not meet Safety criteria

        •	Flame is low and stable (not boiling over).
        •	Wet floor is not involved.
        •	Electrical equipment is off or not in a hazardous state.
        •	No imminent physical harm expected in the next few seconds.

        If a serious hazard is imminent → classify as Safety, not Resource Reminder.
	4.	Reminder is still useful now

        •	User has not walked too far away yet.
        •	The resource can still be quickly fixed.
        •	The relevant earlier interaction with the resource and the current transition-away moment both fall within the short-horizon memory window (see below).

The assistant’s proactive intervention must feel timely and grounded.

⸻

\#\#\# Mutual Exclusion vs. Other Services

Use these distinctions carefully:

Resource Reminder vs. Safety
	•	Resource Reminder: open/unfinished resource state, not dangerous yet.
	•	Safety: the leftover state is already causing immediate bodily danger.

Resource Reminder vs. Next-Step Guidance
	•	Next-Step Guidance: user finished a correct step and needs the next logical action.
	•	Resource Reminder: user forgot a closure step after finishing a workflow or interaction with a resource.

Resource Reminder vs. Error-Recovery
	•	Error-Recovery: user must rollback due to a wrong step (invalid state).
	•	Resource Reminder: workflow is complete or valid; user just forgot to close or finalize something.

Resource Reminder vs. Tool Use
	•	Tool Use: correcting grip/angle/stability for efficiency.
	•	Resource Reminder: ensuring resource closure, not usage mechanics.

⸻

\#\#\# Time-Window Rules (strict)

Each event MUST have:
	•	current\_time\_window = the timestamp of the fine-grained entry that best captures the moment the user leaves the resource unresolved and starts to transition away, within the allowed short-horizon memory window.

Rules:
	1.	Source of current\_time\_window
        •	Prefer timestamps from:
            •	i\_do\_steps[].time\_window
            •	speakers\_say[].time\_window
        •	Do NOT merge or fabricate new ranges.
	2.	Short-Horizon Memory Window (critical)
        Short-Term Resource Reminder operates strictly within a short-horizon memory range, reflecting short-term forgetfulness inside one continuous local episode. The model must follow these temporal constraints:
            •	Immediate window (≈10 seconds)
                If the user finishes interacting with a resource (e.g., stove, faucet, power switch, bottle cap, door latch) and within ≈10 seconds begins to leave or shift tasks, treat this as a strong Resource Reminder opportunity.
            •	Typical short-horizon span (≈10 seconds - 5 minutes)
                The model may link an earlier resource-related action to the user’s current transition-away behavior only if both belong to the same continuous episode and fall within this short window (≤ 5 minutes).
            •	Maximum allowed memory span: 10 minutes
            •	You must never use any resource-related behavior older than 10 minutes as evidence for this service.
            •	If the unresolved resource state originates beyond ≈10 minutes or from a previous episode, it is not eligible for Short-Term Resource Reminder (ignore it for this service).
            •	No long-horizon or cross-episode reasoning
        Do NOT retrieve information from previous activities, previous rooms, earlier times of day, or different sessions.
        The reminder must rely exclusively on short-horizon evidence within the current local episode.

    The assistant’s first utterance is interpreted as occurring during or immediately after this current\_time\_window.

⸻

\#\#\# Resource Reminder Detection Objective

For each batch:
	1.	Scan all segments and interaction\_records to find candidate unresolved resources or closure tasks, where fine-grained annotations indicate that a resource was used/changed but not properly closed, turned off, or secured.
	2.	For each candidate, verify that:
        •	The closure step is missing (e.g., burner not turned off, file not saved, door not fully closed).
        •	The user begins transitioning away or shifting attention to something else.
        •	The state is non-hazardous (else → Safety).
        •	The earlier interaction with the resource and the transition-away moment are within the allowed 10 seconds-10 minutes short-horizon window (ideally 10s-5min, never \textgreater{}10min).
	3.	Select the most fine-grained time\_window indicating when the user abandoned or left behind the closure task as current\_time\_window.
	4.	For each valid case, prepare:
        •	scene\_description (what the user was doing around that moment),
        •	trigger\_reason (why this is a short-term resource reminder),
        •	resource\_key \& resource\_summary,
        •	potential\_consequence,
        •	occurrence\_confidence.

You may output multiple reminders, but avoid duplicates describing the same unresolved resource within overlapping time\_windows.

⸻

\#\#\# Dialogue Generation Objective

For each event, generate a short, natural multi-turn dialogue:

Assistant (Turn 1)
	•	Proactively reminds the user of the unresolved resource.
	•	References the specific resource (stove, faucet, file, door, etc.).
	•	Sounds timely and supportive, grounded in the current short-horizon situation.

Examples:
	•	“Just a reminder — the stove burner is still on.”
	•	“Looks like the trash-can lid is still open.”
	•	“I noticed your document isn’t saved yet.”

User (Turn 2, ≥ 12 English words)
	•	Acknowledges or explains.
	•	May return to close the resource or briefly justify their choice.

Optional Turn 3-4
	•	Assistant gives brief reassurance or a simple suggestion (“You can turn it off now to avoid wasting gas.”).
	•	User confirms closing the resource or clarifies their decision.

Tone
	•	Calm, friendly, non-judgmental.
	•	No scolding or blaming.
	•	Emphasize prevention and convenience (e.g., “so you don’t lose your work,” “to avoid wasting water”).

Do not mention “video”, “annotations”, “models”, or any internal logging.

⸻

\#\#\# Output Format

Your output MUST be exactly one JSON object:
\{
  "service\_main\_type": "Short-term Proactive Service",
  "service\_sub\_type": "Short-Term Resource Reminder Proactive Service",

  "resource\_events": [
    \{
      "event\_id": "resource\_001",

      "current\_segment\_id": "\textless{}segment id\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "supporting\_source": "i\_do\_steps \textbar{} speakers\_say",

      "scene\_description": "\textless{}what the user was doing before or while walking away\textgreater{}",
      "trigger\_reason": "\textless{}why this is a short-term resource reminder\textgreater{}",

      "resource\_key": "\textless{}e.g., stove\_left\_on, water\_running, file\_unsaved, door\_ajar\textgreater{}",
      "resource\_summary": "\textless{}short explanation of what closure step was missed\textgreater{}",
      "potential\_consequence": "\textless{}waste, mess, data loss, inconvenience\textgreater{}",

      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}assistant proactive reminder\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}\textgreater{}=12-word natural reply\textgreater{}"
        \}
        // optional turns 3-4
      ]
    \}
  ]
\}

Notes:
	•	resource\_events may contain 0, 1, or multiple entries depending on how many Short-Term Resource Reminder opportunities exist in this batch.
	•	potential\_consequence is optional but should stay consistent with the annotations (e.g., “wasting gas,” “water may overflow,” “risk of losing unsaved work”).

⸻

\#\#\#\# Failure Case

If no Resource Reminder opportunities appear:
\{
  "service\_main\_type": "Short-term Proactive Service",
  "service\_sub\_type": "Short-Term Resource Reminder Proactive Service",
  "resource\_events": [],
  "note": "No Short-Term Resource Reminder opportunities were detected in this batch."
\}
\end{promptbox}

\begin{promptbox}[EgoLife — Episodic · Task Reminder]
\#\#\# Task Context

You are analyzing MULTIPLE egocentric annotation files (each less than 10 minutes) from the EgoLife dataset for one contiguous batch of time (the actual span is determined by the timestamps in the input, typically within ≤ 2.5 hours).

Your job in this stage is signal mining and dialogue generation for a special Episodic Proactive Service subtype:

Episodic Task Reminder Proactive Service  
(short: Episodic Task Reminder)

This service focuses on pending steps / tasks inside the same episodic window (same local activity or short continuous session), where:

- The user has started or committed to a concrete task or step earlier in the SAME episodic context.
- There is no clear evidence of completion for that task/step.
- The user's behavior now shows they are transitioning away to another activity or state, so the task is likely to be left unfinished right now.
- The assistant should remind the user at the moment of this transition, before the task is silently dropped.

Typical examples:

- The user is doing a multi-step procedure (step 1, step 2…) and skips step 3, then starts packing up or leaving the lab.
- The user says "I'll submit this result once I finish checking it," then later closes the document and opens a different app without submitting.
- The user starts a short form, fills in most fields, then switches to another unrelated task while some required fields are still empty.

*You must:*
1. Scan the current batch to detect within-episode tasks that have pending steps.
2. For each such task, watch later moments in the same episodic window where the user appears to move on without completing it.
3. For each strong case, choose one current moment as the reminder trigger and generate a short multi-turn dialogue where the assistant:
   - points out the unfinished step or task, and
   - offers concrete, helpful options (finish now vs. schedule/ignore).

There is no historical memory JSON for this service:

- You treat each batch independently.
- You do not maintain cross-day or long-horizon memory.
- You only output dialogues for this batch, each grounded in:
  - one pending task/step episode (past), and
  - one transition-away episode (current).

You must NOT guess new events, invent timestamps, or hallucinate behaviors not supported by the annotations.

⸻

\#\#\# Authoritative Timestamps \& Fine-Grained Evidence Priority

Each fine-grained annotation entry has a time\_window aligned to the original video, for example:

- i\_do\_steps[].time\_window
- interactions\_with\_objects[].time\_window
- interactions\_with\_people[].time\_window
- speakers\_say[].time\_window

All time\_window strings already have the format:

\textgreater{} DAY\# HH:MM:SS-HH:MM:SS

You MUST only copy these existing time\_window values.  
Do NOT interpolate, merge, extend, shrink, or invent new time ranges.

Fine-grained evidence priority

When detecting episodic task reminders, you must prioritize fine-grained entries:

- Primary sources to consider as candidate episodes:
  - i\_do\_steps
  - interactions\_with\_objects
  - interactions\_with\_people
  - speakers\_say

Each pending-task episode and each transition-away episode must correspond to at least one fine-grained entry whose content supports that interpretation.

⸻

\#\#\# Input Human Annotations

You are given MULTIPLE JSON objects, each representing a \textless{}10-minute egocentric segment:

\{
  "segment\_id": "\textless{}identifier for this \textasciitilde{}10-minute segment\textgreater{}",
  "description": "... high-level summary of what I do in this segment ...",
  "interaction\_records": [
    \{
      "time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "description": "... micro-episode summary ...",

      "i\_do\_steps": [ ... ],
      "speakers\_say": [ ... ],
      "interactions\_with\_objects": [ ... ],
      "interactions\_with\_people": [ ... ],
      "environment\_state": [ ... ],
      "task\_transition": [ ... ],
      "confidence": 0.0-1.0
    \}
  ]
\}

These interaction\_records and their subfields are your only evidence.

The coverage of this batch is defined by the minimum and maximum timestamps appearing in these JSONs.  
You can assume this coverage is at most about 2.5 hours and usually contains several episodic windows (short continuous activities).

⸻

\#\#\# Service Category

- service\_main\_type: "Long-Term Proactive Service"
- service\_sub\_type: "Episodic Task Reminder Proactive Service"

Note: this service operates on short-horizon, same-episode pending tasks; it is different from Episodic Memory Recall, which focuses on recalling earlier helpful episodes across a longer short-horizon (≤ 2h) even when the current activity is different.

⸻

\#\#\# What counts as an Episodic Task Reminder signal?

An Episodic Task Reminder opportunity is defined by one task thread inside the same episodic window, with two roles:

1. A pending-task episode (earlier in this episode):
   - The user starts, mentions, or is in the middle of a clearly defined task or step, such as:
     - following a numbered or ordered procedure ("step 1 / step 2 / …"),
     - stating an intention to finish something within this episode ("before I leave I'll do X"),
     - performing most of a recognizable task (washing dishes, exporting a result, submitting a form).
   - There is no subsequent evidence in this batch that the critical step or finalization is completed.

2. A transition-away episode (later in the same episodic window):
   - The user switches away from that task thread, e.g.:
     - leaving the current location,
     - starting a different, unrelated activity,
     - closing the relevant app/document,
     - putting away tools or changing context.
   - At this transition moment, the earlier task/step is still pending.

The core question:  
\textgreater{} "Is there something the user clearly intended or needed to do in this episode, which now looks left unfinished as they move on?"

We distinguish three common reminder types:

1. Skipped step in a multi-step procedure (skipped\_step)  
   - Past: annotations show a structured process (explicit "step 1 / step 2 / …" or implicit ordered actions) where a key step is never executed, e.g.:
     - user does step 1 and step 3 but there is no evidence of step 2,
     - user prepares a sample but never logs the result, etc.
   - Current: user transitions into another task or leaves the station (new task\_transition, new context, or clear "packing up").
   - Reminder: "There's still step X you haven't done in this procedure."

2. Unfinished task in this episode (unfinished\_task)  
   - Past: the user starts or states a task with a clear completion condition:
     - "I'll submit this result after checking it,"
     - opening a submission page, filling most fields,
     - beginning to clean an area or pack a box.
   - Current: there is no evidence that the completion event happened (no "submit", no final cleaning step, etc.), and the user is now:
     - idle in a different app,
     - walking away,
     - or starting a new unrelated task.
   - Reminder: "You haven't actually finished / submitted / wrapped up X yet."

3. Pending check or confirmation within this episode (pending\_check)  
   - Past: the user sets up a short verification step inside this episode:
     - "After this run I need to verify the result,"
     - enabling a setting but intending to test it,
     - preparing an experiment whose outcome should be checked before leaving.
   - Current: the user:
     - finishes the main run and starts to move on,
     - or changes context without doing the check.
   - Reminder: "You planned to check Y before moving on; do you want to confirm it now?"

Time \& context constraints (critical):

- The pending-task episode and the transition-away episode must:
  - be within the same episodic window (same local activity context),
  - occur within a short horizon (typically minutes, always ≤ 2 hours),
  - belong to the same task thread (same object/result/form/area/procedure).
- Very short gaps (a few seconds) that represent micro-steps or natural pauses inside the same continuous action should not trigger a reminder; treat these as normal task execution, not as "moving on".

Simple test:

- If the main value is "you're about to walk away / switch tasks while something here is still unfinished" → candidate for Episodic Task Reminder.
- If the main value is "remember something from earlier in this session even though the current activity is different" → Episodic Memory Recall.
- If the main value is "build a habit / routine / long-term progress" → other services (Habit-Coaching, Routine Optimization, Personal Progress Feedback, Long-Horizon Memory-Link).

⸻

\#\#\# Time-Window Rules (strict)

For every Episodic Task Reminder dialogue you output, you must define:

- A past\_time\_window representing the pending-task episode.
- A current\_time\_window representing the moment when the assistant speaks up (transition-away).

Rules:

1. Past time window (past\_time\_window)

   - MUST be copied exactly from one fine-grained entry's time\_window:
     - i\_do\_steps[].time\_window, or
     - interactions\_with\_objects[].time\_window, or
     - interactions\_with\_people[].time\_window, or
     - speakers\_say[].time\_window.
   - Do NOT use interaction\_record.time\_window.
   - Do NOT merge or fabricate new ranges.

2. Current time window (current\_time\_window)

   - MUST be copied exactly from one:
     - i\_do\_steps[].time\_window, or
     - speakers\_say[].time\_window.
   - You MUST NOT use interactions\_with\_objects or interactions\_with\_people as the source for current\_time\_window, even if they describe related context.
   - Choose the earliest time\_window where:
     - the user's behavior first clearly shows they are leaving or switching away from the task thread, and
     - a reminder about the pending step would still be timely and helpful.

3. Temporal order \& horizon

   - past\_time\_window MUST be strictly earlier than current\_time\_window.
   - The gap between them should be:
     - more than a few seconds (so it's not the same micro-action), and
     - at most \textasciitilde{}2 hours, usually within the same short session.

The assistant's first proactive utterance is interpreted as happening immediately after this current\_time\_window.

⸻

\#\#\# Task Reminder Detection Objective

For the current batch (no external history):

1. Scan all segments and interaction\_records to find candidate task threads:
   - Sequences of i\_do\_steps / interactions / speech that:
     - share the same object, document, device, or area, and/or
     - are described as parts of one procedure or goal.

2. For each task thread, identify critical steps or completion conditions, such as:
   - explicit numbered steps,
   - explicit "I'll do X after Y" statements,
   - implicit but clear "finalization" events (submit, save, clean up, switch off, confirm).

3. For each critical step or completion condition:
   - Check whether there is evidence of completion later in the episode.
   - If no completion is detected, treat this as a pending-task episode, with:
     - its segment\_id, past\_time\_window, past\_observation.

4. For each pending-task episode, search later in the same episodic window for a transition-away episode where:
   - the user starts a different task or leaves the relevant context,
   - AND this happens before any completion evidence appears.

5. For each strong pair (pending-task episode, transition-away episode):
   - Ensure both episodes are supported by specific fine-grained annotations.
   - Ensure they belong to the same task thread and the gap fits the short-horizon nature.
   - Select one transition-away episode as the trigger point.

6. For each such pair, generate:
   - One structured reminder entry (with both past and current timestamps).
   - One multi-turn dialogue where the assistant gently reminds the user of the pending task.

You may output multiple task\_reminders in one batch, but:

- Never duplicate the same (past, current) pair.
- Do not trigger multiple times for trivially overlapping transitions referring to the same pending task.

⸻

\#\#\# Dialogue Generation Objective

For each activated episodic task reminder pair, you must generate a short multi-turn dialogue that:

1. Grounds in the specific pending task

   - The assistant should implicitly or explicitly reference the unfinished step or task, in a natural way, e.g.:
     - "You haven't done step 2 of this procedure yet."
     - "You haven't submitted this result you were working on."
     - "You planned to double-check this setting before leaving."
   - Do not mention "video", "annotations", "models", or internal logging.

2. Connects to the transition-away behavior

   - Make it clear that the reminder comes because the user is moving on, e.g.:
     - "Since you're putting things away now…"
     - "Now that you're switching to something else…"
     - "Before you leave the lab area…"

3. Offers concrete, practical choices

   - For skipped\_step:
     - Suggest doing the missing step now, or explicitly skipping it with awareness.
   - For unfinished\_task:
     - Suggest finishing now, or scheduling a reminder / marking it as deferred.
   - For pending\_check:
     - Suggest doing the quick check now, or confirming that it can be safely delayed.

4. Tone and emotional value

   - Gentle, non-judgmental, supportive.
   - Emphasize reducing cognitive load:
     - "so it doesn't slip your mind,"
     - "just in case you still want to finish it now."
   - Avoid scolding language ("you forgot again"); instead:
     - "If you'd like, we can…"
     - "Do you want to quickly handle it before moving on?"

5. Dialogue structure

  Each proactive\_dialogue should contain at least 2 turns, preferably 3-4:

  1. Assistant (Turn 1)  
    - Proactively mentions the pending task/step,
    - links it to the fact that the user is leaving / switching,
    - and offers one or two clear options.

  2. User (Turn 2)  
    - Natural reply (≥ 12 English words).
    - May:
      - accept and finish now,
      - partially accept (e.g., "remind me later"),
      - decline ("it's intentional, I'm done with it"),
      - or modify the reminder rule.

  3. Assistant (optional Turn 3)  
    - Acknowledge the user's choice and either:
      - confirm taking action now (e.g., guiding through the step),
      - confirm a follow-up reminder rule,
      - or gracefully back off if the user declines.

  4. User (optional Turn 4)  
    - Short acknowledgement or final confirmation.

  Diversity

  Across different reminders in the same output:

  - Vary how you phrase the transition:
    - "since you're leaving this desk…"
    - "as you switch to another task…"
    - "now that you're done here for the moment…"
  - Vary the help framing:
    - "Want to quickly finish X before you go?"
    - "Should we tick off that last step now?"
    - "I can set a reminder for later if you prefer."

Not every user must comply; some may say "not now," "I intentionally left it," or "remind me this evening."

⸻

\#\#\# Output Format

Your output MUST be ONE JSON object:

\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Episodic Task Reminder Proactive Service",

  "task\_reminders": [
    \{
      "reminder\_id": "etask\_001",
      "reminder\_type": "skipped\_step \textbar{} unfinished\_task \textbar{} pending\_check",

      "task\_thread\_summary": "\textless{}short abstract description of the task this reminder belongs to\textgreater{}",

      "current\_segment\_id": "\textless{}segment id where the assistant speaks\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "current\_supporting\_source": "i\_do\_steps \textbar{} speakers\_say",
      "current\_observation": "\textless{}what is happening now that shows the user is moving away\textgreater{}",
      "current\_local\_context": "\textless{}short description of current scene / situation\textgreater{}",

      "past\_segment\_id": "\textless{}segment id of the pending-task episode\textgreater{}",
      "past\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "past\_supporting\_source": "i\_do\_steps \textbar{} speakers\_say",
      "past\_observation": "\textless{}what happened earlier that defines the unfinished task or step\textgreater{}",

      "time\_gap\_seconds": 0.0,
      "transition\_reason": "\textless{}why this looks like a switch away from the task\textgreater{}",
      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}assistant proactive reminder, linking pending step to current transition\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}likely user reply (\textgreater{}= 12 words)\textgreater{}"
        \}
        // optionally 1-2 more turns, alternating assistant ↔ user
      ]
    \}
  ]
\}

Notes:

- time\_gap\_seconds can be approximate; it only needs to reflect that this is a short within-episode gap (e.g., 120 for 2 minutes, 900 for 15 minutes).
- task\_reminders may contain 0, 1, or multiple entries depending on how many good within-episode pending-task opportunities exist in this batch.

⸻

\#\#\# Failure Case Format

If you find no good episodic task reminder opportunities in the current batch (no clear "unfinished task + user moving on" cases), output:

\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Episodic Task Reminder Proactive Service",
  "task\_reminders": [],
  "note": "No within-episode pending tasks with clear transition-away behavior were detected in this batch, given the current annotations."
\}
\end{promptbox}

\begin{promptbox}[EgoLife — Episodic · Memory Recall]
\#\#\# Task Context

You are analyzing MULTIPLE egocentric annotation files (each less than 10 minutes) from the EgoLife dataset for one contiguous batch of time (the actual span is determined by the timestamps in the input, typically within ≤ 2.5 hours).

Your job in this stage is signal mining and dialogue generation for a special Episodic Proactive Service subtype:

Episodic Memory Recall Proactive Service
(short: Episodic Recall Service)

This service focuses on short-horizon episodic memory within the same day and within \textasciitilde{}2 hours, where:
	•	Something the user did/said/placed earlier in this batch (the past episode)
	•	Becomes relevant and helpful now (the current episode),
	•	And the assistant can proactively remind or resurface that past episode at the right moment.

Examples:
	•	The user put their notebook on a side table 30 minutes ago; now they are leaving the room without it.
	•	The user said "I'll send that email after finishing this call" 40 minutes ago; now they are idling at the laptop after the call.
	•	The user prepared ingredients or tools a while ago; now they are about to start the related task.

*You must:*
	1.	Scan the current batch to detect episodic links within ≤ 2 hours (no cross-day and no external history).
	2.	For each strong link, select one current moment where a reminder would be useful.
	3.	For each such moment, generate one short multi-turn dialogue where the assistant recalls the past episode and offers concrete, helpful action.

There is no historical memory JSON in this service:
	•	You treat each batch independently.
	•	You do not need to output or update any persistent memory state.
	•	You only output dialogues for the current batch, each grounded in one current episode and one past episode.

You must NOT guess new events, invent timestamps, or hallucinate behaviors not supported by the annotations.

⸻

\#\#\# Authoritative Timestamps \& Fine-Grained Evidence Priority

Each fine-grained annotation entry has a time\_window aligned to the original video, for example:
	•	i\_do\_steps[].time\_window
	•	interactions\_with\_objects[].time\_window
	•	interactions\_with\_people[].time\_window
	•	speakers\_say[].time\_window

All time\_window strings already have the format:

DAY\# HH:MM:SS-HH:MM:SS

You MUST only copy these existing time\_window values.
Do NOT interpolate, merge, extend, shrink, or invent new time ranges.

\#\#\# Fine-grained evidence priority
When detecting episodic memory links, you must prioritize fine-grained entries:
	•	i\_do\_steps
	•	interactions\_with\_objects
	•	interactions\_with\_people
	•	speakers\_say

Each past episode and current episode in a recall link must correspond to at least one fine-grained entry whose content supports that interpretation.

⸻

\#\#\# Input Human Annotations

You are given MULTIPLE JSON objects, each representing a \textless{}10-minute egocentric segment:
\{
  "segment\_id": "\textless{}identifier for this \textasciitilde{}10-minute segment\textgreater{}",
  "description": "... high-level summary of what I do in this segment ...",
  "interaction\_records": [
    \{
      "time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "description": "... micro-episode summary ...",

      "i\_do\_steps": [ ... ],
      "speakers\_say": [ ... ],
      "interactions\_with\_objects": [ ... ],
      "interactions\_with\_people": [ ... ],
      "environment\_state": [ ... ],
      "task\_transition": [ ... ],
      "confidence": 0.0-1.0
    \}
  ]
\}

These interaction\_records and their subfields are your only evidence.

The coverage of this batch is defined by the minimum and maximum timestamps appearing in these JSONs.
You can assume this coverage is at most about 2.5 hours.

⸻

Service Category
	•	service\_main\_type: "Episodic Proactive Service"
	•	service\_sub\_type: "Episodic Memory Recall Proactive Service"

But note: this service operates on short-horizon episodic memory (≤ 2 hours) and does not maintain long-horizon or cross-day memory state.

⸻

\#\#\# What counts as an Episodic Memory Recall signal?

An Episodic Recall opportunity is defined by a pair of episodes within the same batch:
	1.	A past episode (earlier in time in this batch) where the user does/says/places something that can be useful later.
	2.	A current episode (later in time, within ≤ 2 hours of the past one) where recalling that past episode would clearly help the user.

We distinguish three common recall types:
	1.	Forgotten / mis-placed item (forgotten\_item)
        •	Past: the user puts or leaves an item somewhere (bag, table, shelf, other room).
        •	Current: the user:
            •	is about to leave the place without it, or
            •	is looking for / mentioning the item, or
            •	starts a task where that item is obviously needed.
        •	The reminder: "That thing you used/put earlier is over there."
	2.	Unfinished or deferred plan (unfinished\_plan)
        •	Past: the user expresses an intention or plan to do something later within this session, e.g.:
            •	"After this I'll send the email / check the results / tidy up here."
            •	"I'll come back to finish labeling these boxes."
        •	Current: the user:
            •	reaches a natural moment where that plan could be executed (idle at computer, done with prior task), or
            •	mentions or starts a related task in a way that suggests they might have forgotten the earlier plan.
        •	The reminder: "You said you wanted to do X after Y, do you want to handle it now or schedule it?"
  3. Contextual cue, status check, or inspired use (context\_cue / check\_status / inspired\_use)
        Past: The user previously started a short process, left a cue, or heard/said a tip that may soon matter (e.g., starting a download, putting food in the oven, charging a device, hearing a useful instruction or trick).
        Current: The user returns to the relevant context (oven, desk, charging spot, device) or begins a task where that earlier process/tip becomes directly helpful.
        Reminder:
            •	check\_status: "You started X earlier — do you want to check its status or use it now?"
            •	context\_cue: "You left/mentioned Y earlier — it might be relevant here."
            •	inspired\_use: "Someone/you mentioned Z earlier — do you want to try that approach now?"

Time constraint (critical):
	•	The past episode and the current episode must be within the same batch and within a short horizon ≤ 2 hours.
	•	Anything that spans \textgreater{} 2 hours or different days belongs to Long-term Memory-Link service, not this one.
	•	Very short gaps (a few seconds) that only reflect micro-steps of the same immediate action should be treated as local task structure, not Episodic Recall.

Simple test:
	•	If the main value is "remember what just happened earlier in this session (≤ 2h) to avoid forgetting or to complete a plan" → candidate for Episodic Recall.
	•	If the main value is:
        •	"build a habit" → Habit-Coaching Proactive Service.
        •	"optimize a routine or default config" → Routine Optimization Proactive Service.
        •	"track long-term progress / skill improvement" → Personal Progress Feedback Proactive Service.
        •	"link events across days or long gaps (≥ 2h)" → Long-Horizon Memory-Link Proactive Service.

⸻

\#\#\#\# Exclusions

Do NOT classify as Episodic Recall:
	•	One-off random actions with no clear short-horizon future relevance.
	•	Generic tidying/arranging without any obvious near-future scenario tied to it.
	•	Pure routine optimization ("you always do this sequence, let me bundle it") without a specific past episode within this batch.
	•	Long-term health/productivity habits (hydration / posture / breaks).
	•	External safety issues (hot surfaces, tripping, etc.) → Safety Proactive Service.
	•	Long-horizon links (≥ 2h or cross-day) → Memory-Link Contextual Proactive Service.

⸻

\#\#\# Time-Window Rules (strict)

You must define for every Episodic Recall dialogue:
	•	A past\_time\_window representing the earlier episode.
	•	A current\_time\_window representing the moment when the assistant speaks up.
    •	Each past\_time\_window MUST correspond to exactly one specific earlier event that is directly used in the current\_time\_window episode; the past and current events must form a clear one-to-one correspondence for the recall link.

Rules:
	1.	Past time window (past\_time\_window)
        •	MUST be copied exactly from one fine-grained entry's time\_window:
            •	i\_do\_steps[].time\_window, or
            •	interactions\_with\_objects[].time\_window, or
            •	interactions\_with\_people[].time\_window, or
            •	speakers\_say[].time\_window.
        •	Do NOT use interaction\_record.time\_window.
        •	Do NOT merge or fabricate new ranges.
	2.	Current time window (current\_time\_window)
        •	MUST be copied exactly from one:
            •	i\_do\_steps[].time\_window, or
            •	speakers\_say[].time\_window.
        •	You MUST NOT use interactions\_with\_objects or interactions\_with\_people as the source for current\_time\_window, even if they describe related context.
        •	Choose the earliest time\_window where:
            •	the current behavior first shows that the past episode is relevant (e.g., starting to leave, starting to sit at the desk, opening the app), and
            •	a reminder would still be timely and helpful.
	3.	Temporal order
        •	past\_time\_window MUST be strictly earlier than current\_time\_window.
        •	The gap between them should be more than a few seconds (so it's not the same micro-action) and at most \textasciitilde{}2 hours.

The assistant's first proactive utterance is interpreted as happening immediately after this current\_time\_window.

⸻

\#\#\# Episodic Link Detection Objective

For the current batch (no external history):
	1.	Scan all segments and interaction\_records to find candidate past episodes that:
	    •	create a resource, place an object, express a near-future plan, says something, or start a short-horizon process whose status will matter soon.
	2.	For each candidate past episode, look later in the batch (within ≤ 2.5 hours) for current episodes where:
        •	the same object/plan/process becomes relevant, or
        •	the user's current behavior suggests they might forget/need that earlier episode.
	3.	For each strong pair (past episode, current episode):
        •	Confirm that both episodes are supported by specific fine-grained annotations.
        •	Confirm that the gap is within ≤ 2 hours and fits the short-horizon nature.
        •	Select one current episode as the trigger point.
	4.	For each such pair, generate:
        •	One structured recall entry with:
        •	past\_segment\_id, past\_time\_window, past\_observation,
        •	current\_segment\_id, current\_time\_window, current\_observation,
        •	a natural-language link\_reason.
        •	One multi-turn dialogue where the assistant uses this episodic memory to help now.

You may output multiple recall dialogues in one batch, but:
	•	Never duplicate the same (past, current) pair.
	•	Do not trigger multiple times for trivially overlapping current episodes referring to the same past event.

⸻

\#\#\# Dialogue Generation Objective

For each activated episodic recall pair, you must generate a short multi-turn dialogue that:
	1.	Grounds in the specific past episode
        •	The assistant should implicitly or explicitly reference the earlier action or statement, in a natural way, e.g.:
        •	"You left your notebook on the side table earlier."
        •	"A bit earlier you said you wanted to send that email after this call."
        •	"You started charging this device earlier this afternoon."
        •	But: do not mention "video", "annotations", "models", or internal logging.
	2.	Connects the past to the current situation
        •	Show that the reminder is context-aware, e.g.:
            •	User is leaving room: remind about item left behind.
            •	User is idle at laptop: remind about earlier plan to send email.
            •	User returns to kitchen: remind about food in oven or short process started earlier.
	3.	Offers concrete, practical help
        •	For forgotten\_item:
        •	Point out the location, offer to mark it or remind again later if needed.
        •	For unfinished\_plan:
        •	Suggest doing it now or scheduling it later, possibly summarizing the plan.
        •	For context\_cue / check\_status:
        •	Suggest checking status, verifying results, or moving to the next step.
	4.	Tone and emotional value
        •	Gentle, non-judgmental, slightly caring.
        •	Emphasize reducing mental load ("so you don't have to keep it in your head").
        •	Avoid scolding ("you forgot again"), instead:
        •	"If you'd like, I can remind you…"
        •	"Do you want to take a moment to…"
	5.	Dialogue structure
        Each proactive\_dialogue must contain at least 2 turns, preferably 3-4:
        1.	Assistant (Turn 1)
            •	Proactively recalls the past episode, links it to the current situation, and offers one or two clear options.
        2.	User (Turn 2)
            •	Natural reply (≥ 12 English words).
            •	May accept, partially accept, decline, postpone, or ask for a different behavior.
        3.	Assistant (optional Turn 3)
            •	Acknowledge the choice and either:
            •	confirm the action (e.g. "Let's quickly do it now"), or
            •	confirm the rescheduling/reminder rule, or
            •	gracefully back off.
        4.	User (optional Turn 4)
            •	Short acknowledgment or final confirmation.
        5.	Diversity
        Across different recall dialogues in the same output:
            •	Vary how you phrase the episodic connection:
                •	"A bit earlier you…"
                •	"Just a while ago you…"
                •	"Earlier in this session you…"
            •	Vary the help framing:
                •	"Do you want to grab it before you go?"
                •	"Would now be a good time to finish that?"
                •	"I can remind you again later if you prefer."

Not every user must comply; some may say "not now", "remind me in a bit", etc.

⸻

\#\#\# Output Format

Your output MUST be ONE JSON object:
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Episodic Memory Recall Proactive Service",

  "recall\_dialogues": [
    \{
      "recall\_id": "erecall\_001",
      "recall\_type": "forgotten\_item \textbar{} unfinished\_plan \textbar{} context\_cue \textbar{} check\_status",

      "current\_segment\_id": "\textless{}segment id where the assistant speaks\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "current\_supporting\_source": "i\_do\_steps \textbar{} speakers\_say",
      "current\_observation": "\textless{}what is happening now that makes the past episode relevant\textgreater{}",
      "current\_local\_context": "\textless{}short description of current scene / situation\textgreater{}",

      "past\_segment\_id": "\textless{}segment id of the past episode\textgreater{}",
      "past\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "past\_supporting\_source": "i\_do\_steps \textbar{} speakers\_say",
      "past\_observation": "\textless{}what happened earlier that is now useful\textgreater{}",

      "time\_gap\_seconds": 0.0,
      "link\_reason": "\textless{}why this past episode is helpful to recall now within \textasciitilde{}2 hours\textgreater{}",
      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}assistant proactive reminder, explicitly or implicitly recalling the past episode\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}likely user reply (\textgreater{}= 12 English words)\textgreater{}"
        \}
        // optionally 1-2 more turns, alternating assistant ↔ user
      ]
    \}
  ]
\}

Notes:
	•	time\_gap\_seconds can be approximate; it is only used to reflect the short-horizon nature (e.g., 600 for 10 minutes).
	•	recall\_dialogues may contain 0, 1, or multiple entries depending on how many good episodic recall opportunities exist in this batch.

⸻

\#\#\#\# Failure Case Format

If you find no episodic recall opportunities in the current batch (no clear past-current pairs within ≤ 2 hours that would benefit from reminder):
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Episodic Memory Recall Proactive Service",
  "recall\_dialogues": [],
  "note": "No short-horizon episodic memory recall opportunities were detected in this batch, given the current annotations."
\}
\end{promptbox}

\begin{promptbox}[EgoLife — Long-Term · Habit-Coaching]
\#\#\# Task Context

You are analyzing MULTIPLE egocentric annotation files (each less than 10 minutes) from the EgoLife dataset for one contiguous batch of time (up to \textasciitilde{}2.5 hours).

Your job in this stage is habit-signal mining and dialog generation for:

•	service\_main\_type: "Long-Term Proactive Service"
•	service\_sub\_type: "Habit-Coaching Proactive Service"

In this stage, your task is to mine unhealthy behavior signals within the current batch and, for each event that satisfies the activation rules, generate a short Habit-Coaching proactive dialogue.

The assistant here behaves like a health / productivity tracker:
	•	For some behaviors (e.g., prolonged sitting, continuous screen use, not drinking/eating),
    it should trigger within the same day once unhealthy accumulation exceeds a threshold.
	•	For other behaviors (e.g., frequently working very late at night),
    it should trigger based on a cross-day lifestyle pattern.

Therefore, you must distinguish two types of unhealthy behavior:
	1.	Type A - Intra-day accumulation events
    Unhealthy exposure within the same day that should trigger a coaching reminder once a threshold is reached.
    Examples:
        •	Sitting or desk-bound work continuously for ≥ 40-60 minutes without meaningful standing/walking.
        •	Long continuous or cumulatively excessive screen usage (phone / laptop / tablet) without sufficient breaks.
        •	No drinking or no meals for a long stretch while engaged in work/activities.
	2.	Type B - Cross-day lifestyle patterns
    Habits that only become clearly problematic when observed across days.
    Examples:
        •	Repeatedly working or using screens very late at night (e.g., past midnight) over multiple days.
        • Consistently eating lunch around noon on prior days, but on the current day still skipping lunch well past the usual time (e.g., after 1 PM).
        •	Other long-term patterns (if specified) that require next-day or cross-day coaching, e.g.:
        "If the user worked very late last night, remind them the next evening to go to bed earlier."

You will receive two inputs each time:
	1.	Current batch annotations (required) - multiple segment-level human annotations for this ≤2.5hours window.
	2.	Historical habit summary JSON (optional) - previously mined habit events and triggered habit-coaching dialogues across earlier hours/days.

You must NOT guess new events, invent timestamps, or hallucinate behaviors not supported by the annotations.

⸻

\#\#\# Authoritative Timestamps

Every annotation entry has a time\_window aligned to the original video, for example:
	•	i\_do\_steps[].time\_window
  •	speakers\_say[].time\_window
	•	interactions\_with\_objects[].time\_window
	•	interactions\_with\_people[].time\_window

All time\_window strings use the format:

DAY\# HH:MM:SS-HH:MM:SS

You MUST only copy these existing time\_window values.
Do NOT interpolate or invent new time ranges.

⸻

\#\#\# Input Human Annotations

1. Current batch: segment-level episodic annotations

You are given MULTIPLE JSON objects, each representing a \textless{}=10-minute egocentric segment:
\{
  "segment\_id": "\textless{}identifier for this \textasciitilde{}10-minute segment\textgreater{}",
  "description": "... high-level summary of what I do in this segment ...",
  "interaction\_records": [
    \{
      "time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "description": "... micro-episode summary ...",

      "i\_do\_steps": [ ... ],
      "speakers\_say": [ ... ],
      "interactions\_with\_objects": [ ... ],
      "interactions\_with\_people": [ ... ],
      "environment\_state": [ ... ],
      "task\_transition": [ ... ],
      "confidence": 0.0-1.0
    \}
  ]
\}

These interaction\_records and their subfields are your primary evidence.
The coverage of this batch is defined by the min/max timestamps in these JSONs.

⸻

2. Historical habit summary JSON (optional memory)

You may receive ONE historical JSON summarizing previously mined habit-related events and triggered habit-coaching dialogues:
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Habit-Coaching Proactive Service",
  "habit\_events": [
    \{
      "habit\_id": "habit\_001",
      "habit\_key": "\textless{}abstract description of one unhealthy habit pattern\textgreater{}",
      "habit\_type": "intra\_day\_health \textbar{} cross\_day\_lifestyle \textbar{} mixed",
      "threshold\_description": "\textless{}what threshold defines 'unhealthy'\textgreater{}",
      "habit\_summary": "\textless{}how this habit has appeared over previous hours/days\textgreater{}",

      "occurrences": [
        \{
          "segment\_id": "\textless{}old segment id\textgreater{}",
          "day\_id": 1,
          "time\_window": "DAY1 HH:MM:SS-HH:MM:SS",
          "supporting\_source": "i\_do\_steps \textbar{} interactions\_with\_objects \textbar{} interactions\_with\_people \textbar{} speakers\_say",

          "observation": "\textless{}what happened\textgreater{}",
          "local\_context": "\textless{}local scene / surroundings\textgreater{}",
          "metrics": \{
            "sitting\_minutes": 45.0,
            "screen\_minutes": 60.0
          \},
          "historical\_context": "\textless{}how it related to earlier ones\textgreater{}",
          "inferred\_role": "sub\_threshold \textbar{} near\_threshold \textbar{} threshold\_cross \textbar{} followup\_check",
          "workflow\_position": "start \textbar{} middle \textbar{} end \textbar{} standalone",
          "social\_dynamics": "self-initiated \textbar{} reacting\_to\_others \textbar{} jointly\_decided",
          "occurrence\_confidence": 0.0
        \}
      ]
    \}
  ],
  "historical\_habit\_triggers": [
    \{
      "trigger\_id": "htrig\_001",
      "habit\_id": "habit\_001",
      "habit\_key": "\textless{}copied from habit\_state\_updates\textgreater{}",
      "trigger\_type": "intra\_day\_threshold \textbar{} cross\_day\_pattern",

      "current\_segment\_id": "\textless{}segment id where reminder is triggered\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "supporting\_source": "i\_do\_steps \textbar{} speakers\_say ",

      "current\_observation": "\textless{}what just happened that makes this a good coaching moment\textgreater{}",
      "current\_local\_context": "\textless{}short description of current scene\textgreater{}",
      "trigger\_reason": "\textless{}why threshold is considered exceeded or cross-day pattern confirmed\textgreater{}",
      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}assistant coaching reminder, like a health band: e.g., you've been sitting for a long time, want to stand or stretch?\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}likely user reply (\textgreater{}= 10-12 words), may accept/decline/adjust\textgreater{}"
        \},
        \{
          "role": "assistant",
          "utterance": "\textless{}follow-up: confirm reminder, suggest simple action, or gently back off\textgreater{}"
        \}
      ]
    \}
  ]
\}

Notes:
    •  habit\_key must describe ONE concrete unhealthy pattern and its intended coaching meaning.
    •  habit\_id is a stable identifier bound to one habit\_key.  
        - All occurrences of the same unhealthy habit pattern MUST reuse the same habit\_id and habit\_key.  
        - habit\_id MUST follow a simple global increasing scheme: `"habit\_001"`, `"habit\_002"`, `"habit\_003"`, …  
        - When you need to create a NEW habit\_key (a new kind of unhealthy habit), you MUST look at all existing habit\_id in the historical JSON, find the largest index, and assign the next number (e.g., history has `habit\_001` and `habit\_002` → next new habit\_id MUST be `habit\_003`).  
        - You MUST NOT rename or renumber any existing habit\_id.
    •	habit\_type:
        •	intra\_day\_health: same-day accumulation events like prolonged sitting / screen / no drinking/ no meals.
        •	cross\_day\_lifestyle: cross-day patterns related to irregular daily routines, such as frequently working very late.
    •	mixed: when both views are relevant.
    •	day\_id is derived from time\_window's DAY\#.

If no historical summary JSON is provided or habit\_events is empty, treat this as no prior habit memory.

⸻

Service Category
	•	service\_main\_type: Long-Term Proactive Service
	•	service\_sub\_type: Habit-Coaching Proactive Service

⸻

\#\#\# What counts as a Habit-Coaching signal?

You focus ONLY on health / productivity habits, not on preferences or safety emergencies.

We distinguish:

Type A - Intra-day accumulation
Behaviors where continuous or cumulative exposure in the same day becomes unhealthy and should trigger a coaching reminder, similar to a smartwatch alert.

    Typical patterns (examples, not exhaustive):
        1.	Prolonged sitting / lack of movement
            •	Multiple i\_do\_steps / speakers\_say entries showing:
            •	sitting at desk / working on laptop / watching TV,
            •	with no standing/walking / posture change over a long stretch.
            •	Threshold examples:
                •	sitting\_minutes ≥ 40min without a break.
        2.	Continuous screen usage
            •	speakers\_say or i\_do\_steps indicating "scrolling phone", "working on laptop", "watching videos" with no interruption.
            •	Threshold examples:
                •	screen\_minutes ≥ 45min without substantial off-screen activity.
                •	accumulated screen\_time ≥ 5h one day
                •	Very frequent screen checking in a short time window (e.g. picking up phone every few minutes).
        3.	No hydration / no meals for a long stretch
            •	Long block of work / study / moving around with no drinking/eating events.
            •	Threshold examples:
                •	no\_drink\_minutes ≥ 120min while awake and active.
                •	no\_meal\_hours ≥ 5h since last meal, with continuous activities.

    *These are always judged within the current day.*
    We do not sum "30min sitting today + 30min tomorrow" to trigger Habit-Coaching.

Type B - Cross-day lifestyle patterns
Behaviors where the risk comes from repeated late-night / irregular rest patterns across days.

    Typical patterns (examples, not exhaustive):
        1.	Repeated late-night work / screen use
            •	On DAY N: annotations show active computer/phone use or work well past midnight or very late night.
            •	On DAY N+1: user still follows similar schedule (e.g., again working late, or clearly tired).
            •	Habit-Coaching should:
                •	On the following evening, remind the user to rest earlier because of last night's late session.
                •	Or, if late-night behavior persists across multiple days, strengthen the coaching.
            •   On DAY N: user usually eats lunch around 12:00 (e.g., ordering food at noon).
            •   On DAY N+1: it is already past 13:00 and the user still has not eaten lunch.
            •   Habit-Coaching should:
                •   During DAY N+1 early afternoon (e.g., 13:00-13:30), remind the user to eat lunch on time based on their usual pattern.
        2.	Other cross-day health patterns (if specified)
            •	e.g., consistently waking up very early after very late nights.
            •   e.g., persistently irregular meal schedules across days (e.g., lunch or dinner consistently much later than usual).
            (You should only handle what is clearly supported by historical JSON; do not invent new categories.)

⸻

\#\#\# Fine-Grained Evidence Priority (critical)

When detecting candidate habit occurrences, prioritize fine-grained entries:
	•	i\_do\_steps
  •	speakers\_say
	•	interactions\_with\_objects
	•	interactions\_with\_people
	
→ Use these to infer:
	•	whether the user is sitting / using screen / moving / drinking / eating / resting,
	•	how long they keep doing so in this batch.

This priority applies to:
	•	which content you use to measure accumulation or late-night behavior, and
	•	which time\_window you copy for each occurrence.

⸻

\#\#\# Authoritative Time Rules for Triggers

For habit\_triggers (where you will generate dialogues):
    •	current\_time\_window MUST be copied from: i\_do\_steps[].time\_window or speakers\_say[].time\_window
    •	current\_time\_window must correspond to:
        • For Type A (intra-day):
                - the first interval in THIS DAY where the unhealthy threshold is crossed
                (e.g., the moment continuous sitting reaches 40+ minutes, or no-drink
                duration reaches \textasciitilde{}2 hours), while the user is still in that pattern.
        • For Type B (cross-day lifestyle):
            - a representative interval in the CURRENT BATCH on the new day where the
                SAME unhealthy pattern clearly continues again, such as:
                ▫ the first "working on laptop / using screen" interval tonight after a
                    previous very late-night work session, or
                ▫ the first main-meal interval that again happens very late in the day
                    after a history of late dinners.
            - In other words, pick the earliest fine-grained i\_do\_steps / speakers\_say
                time\_window in this batch where the cross-day lifestyle habit is
                obviously active again on this DAY\#, and use it as current\_time\_window.

You MUST NOT:
	•	invent new or merged time ranges,
	•	extend or shorten existing time\_window strings.

⸻

\#\#\# Habit Key Granularity Rules

Each habit\_key should describe one concrete unhealthy habit + its coaching goal, e.g.:
	•	"Sits at desk for \textgreater{}40 minutes without standing or walking."
	•	"Uses phone or laptop screens continuously for long stretches without eye breaks."
	•	"Often works on laptop past midnight on consecutive days."

Template you should be able to fill:

"When I [do X in this situation] for [too long / too often],
the assistant should coach me to [take Y healthier action]."

Bad examples (too vague):
	•	"Health issues"
	•	"Bad time management"
	•	"Screen usage" (without threshold / context)

Good examples:
	•	"Prolonged desk sitting (\textgreater{}40min) without standing during study/work time"
	•	"Late-night laptop work after midnight on multiple days"

If you cannot express all occurrences under one habit\_key with a single, concrete unhealthy pattern and threshold, you must split into multiple habit\_keys.

⸻

\#\#\# Historical Integration Rules
	1.	Reusing an existing habit\_key
    Given a new occurrence and an existing habit\_key in history, reuse it if:
        1.	Same target behavior
            •	Same kind of activity: sitting vs screen vs no drinking vs late-night work.
        2.	Same health framing and threshold scale
            •	e.g., both are "sitting continuously for \textasciitilde{}40+ minutes", not one for 10min and another for 4h.
        3.	Same habit type
            •	Both are intra\_day\_health events about breaks,
            •	or both are cross\_day\_lifestyle events about late-night work.

    If all align:
        •	Reuse the same habit\_id and habit\_key.
        •	Add a new occurrence with appropriate metrics (sitting\_minutes, screen\_minutes, etc.).
        •	Update habit\_summary to reflect how this batch extends or reinforces the habit.

	2.	Creating a new habit\_key
    Create a new habit\_id / habit\_key when:
        •	The behavior is clearly different (e.g., "no drinking" vs "prolonged sitting").
        •	The time scale and coaching strategy differ (intra-day vs cross-day).
        •	The existing keys would become too vague if forced to include this pattern.
    When you create a new habit\_id, you MUST:  
        • Use the global `"habit\_XXX"` format (e.g., `habit\_001`, `habit\_002`, …).  
        • Scan all existing habit\_id in the historical JSON, find the maximum numeric index, and assign the next integer (zero-padded to 3 digits).  
        • Example: if existing IDs are `habit\_001` and `habit\_002`, the next new habit\_id MUST be `habit\_003`.
⸻

\#\#\# Objective

For the current batch of segments (≤2.5 hours), with optional historical habits, you must:
	  1.	Update habit\_state (habit\_state\_updates)
        •   Scan all segments and interaction\_records to find:
            •   new evidence for cross-day lifestyle patterns (Type B), such as when the user actually goes to sleep, when they have lunch/dinner, or when late-night work extends well past midnight.
            •   optionally, you may record intra-day accumulation events (Type A) only when they are needed as context for later cross-day reasoning; Type A is not required to be fully logged here.
        •   When deciding whether to reuse an existing habit\_key or create a new one, you MUST follow the Habit Key Granularity Rules strictly, so that each habit\_key consistently represents one coherent habit or lifestyle pattern.
        •   When integrating new occurrences into historical habit\_state, you MUST follow the Historical Integration Rules strictly, including:
            •   reusing habit\_id / habit\_key only when the semantics and temporal pattern match the existing habit definition, and
            •   creating a new habit\_id / habit\_key when the behavior differs in goal, context, or time-of-day pattern.
        •	  Integrate with habit\_events from history by reusing or creating habit\_keys accordingly.
        •	  For each habit\_id, append new occurrences capturing:
            •	segment\_id, day\_id, time\_window, supporting\_source,
            •	observation, local\_context, metrics (e.g., sitting\_minutes),
            •	inferred\_role (sub\_threshold / threshold\_cross / followup\_check),
            •	occurrence\_confidence.

    2. Decide current-batch habit triggers (habit\_triggers covering both types)
        •	For Type A (intra-day short-horizon habits, gap between triggers \textgreater{}= 2 hours each type):
            •	Within the current annotation batch, *scan all segments and interaction\_records*, track the cumulative exposure to each habit\_key (e.g., continuous sitting, continuous screen use, time since last drink, etc.).
            •	When the accumulation for a given habit\_key crosses the unhealthy threshold inside this batch, select the earliest suitable interval as a trigger point where:
                •	the user is still in that pattern (still sitting, still using screen, still not drinking, etc.), and
                •	a gentle coaching reminder would still be timely and helpful.
            •	Trigger frequency constraint:
                • You may trigger more than once per day for different habit\_keys (e.g., one prolonged-sitting reminder + one hydration reminder).
                •	But for the same habit\_key, you MUST trigger at most once within any ≤2.5h batch (no more than one strong reminder per 2-hour window for that pattern).
        •	For Type B (cross-day lifestyle habits):
            •	Use the "habit\_events" in historical JSON to detect cross-day lifestyle patterns, such as:
                •	sleep\_too\_late (e.g., still working / using screen past 01:00),
                •	eat\_too\_late (e.g., main meal consistently after a very late time),
                •	or other explicitly defined cross\_day\_lifestyle habit\_keys.
            •	For each such habit\_key:
                •	First, confirm from history that the user has repeatedly shown this pattern on previous days (e.g., multiple late nights, multiple late dinners).
                • In today's relevant batch (e.g., the evening work batch for sleep\_too\_late, or the dinner-time batch for eat\_too\_late), treat the first segment that matches the risky context as a trigger opportunity and use its fine-grained time\_window as the current\_time\_window.
            •	Daily trigger constraint:
                •	For each cross\_day\_lifestyle habit\_key (e.g., sleep\_too\_late, eat\_too\_late), you MUST trigger at most one coaching reminder per DAY\#.
                • Different habit\_keys may each trigger once on the same day (e.g., the user may receive one “sleeping too late” reminder and one “eating too late” reminder on the same day, but each habit\_key triggers at most once).
        •	For every trigger (Type A or Type B), prepare:
            •	a structured habit\_trigger record, and
            •	a short multi-turn coaching dialogue grounded in that current\_time\_window and the corresponding habit\_key.
        •	*The "historical\_habit\_triggers" field in the Historical Habit Summary JSON is used to help determine whether the activation frequency for the same habit type complies with the above trigger rules (especially for type A, the gap between triggers \textgreater{}= 2 hours each type).*

⸻

\#\#\# Dialogue Generation Objective (per activated trigger)

For every activated habit trigger (Type A or Type B), you must generate a short, natural, multi-turn proactive coaching dialogue grounded strictly in the chosen current\_time\_window. The dialogue should behave like a gentle health/productivity assistant, similar to a smartwatch or wellbeing coach.

Assistant - Turn 1 (required)
The assistant should:
	•	Refer to the specific unhealthy habit pattern reflected by habit\_key (e.g., prolonged sitting, long continuous screen use, late-night work, late meal).
	•	Mention why this moment is appropriate for a gentle reminder (threshold crossed, or cross-day pattern continuing).
	•	Offer one simple, actionable suggestion (stand/stretch, rest eyes, drink water, take a short break, eat on time, wind down earlier).
	•	Be supportive and non-judgmental.

User - Turn 2 (required, ≥ 12 English words)
The user replies naturally, often acknowledging, explaining context, or tentatively agreeing.
Example behaviors:
	•	"Yes, I didn't notice how long I've been sitting."
	•	"I'm almost done, but I can take a short break."

Assistant - Turn 3 (optional but recommended)
A brief follow-up that:
	•	Acknowledges the user's response,
	•	Offers a small encouragement or adjustment,
	•	Or gently confirms the coaching suggestion.

Tone requirements
	•	Calm, friendly, supportive.
	•	No scolding, no medical claims, no pressure.
	•	Avoid absolute statements ("you must…"). Prefer soft phrasing ("you could…", "might help to…").
	•	Do not mention sensors, annotations, thresholds, or dataset internals.

Content constraints
	•	All details must come from the habit\_key, current\_observation, and time\_window.
	•	No hallucinated behaviors, tools, or locations.
	•	The dialogue must stay strictly tied to the unhealthy habit detected in this trigger.

⸻

\#\#\# Output Format (two sections)

Your output must be ONE JSON object:
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Habit-Coaching Proactive Service",

  "habit\_state\_updates": [
    \{
      "habit\_id": "habit\_001",
      "habit\_key": "\textless{}one unhealthy habit pattern\textgreater{}",
      "habit\_type": "intra\_day\_health \textbar{} cross\_day\_lifestyle \textbar{} mixed",
      "threshold\_description": "\textless{}natural-language threshold\textgreater{}",
      "habit\_summary": "\textless{}how this habit looks so far including this batch\textgreater{}",
      "batch\_consistency\_level": "high \textbar{} medium \textbar{} low",
      "batch\_confidence": 0.0,

      "occurrences": [
        \{
          "segment\_id": "\textless{}source segment id\textgreater{}",
          "day\_id": 2,
          "time\_window": "DAY2 HH:MM:SS-HH:MM:SS",
          "supporting\_source": "i\_do\_steps \textbar{} speakers\_say",

          "observation": "\textless{}specific evidence of this habit in this batch\textgreater{}",
          "local\_context": "\textless{}what the user is doing / environment\textgreater{}",
          "metrics": \{
            "sitting\_minutes": 45.0,
            "screen\_minutes": 0.0,
            "no\_drink\_minutes": 120.0
          \},
          "historical\_context": "\textless{}how this occurrence relates to earlier ones under this habit\_id\textgreater{}",
          "inferred\_role": "sub\_threshold \textbar{} threshold\_cross \textbar{} followup\_check",
          "workflow\_position": "start \textbar{} middle \textbar{} end \textbar{} standalone",
          "social\_dynamics": "self-initiated \textbar{} reacting\_to\_others \textbar{} jointly\_decided",
          "occurrence\_confidence": 0.0
        \}
      ]
    \}
  ],

  "habit\_triggers": [
    \{
      "trigger\_id": "htrig\_001",
      "habit\_id": "habit\_001",
      "habit\_key": "\textless{}copied from habit\_state\_updates\textgreater{}",
      "trigger\_type": "intra\_day\_threshold \textbar{} cross\_day\_pattern",

      "current\_segment\_id": "\textless{}segment id where reminder is triggered\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "supporting\_source": "i\_do\_steps \textbar{} speakers\_say ",

      "current\_observation": "\textless{}what just happened that makes this a good coaching moment\textgreater{}",
      "current\_local\_context": "\textless{}short description of current scene\textgreater{}",
      "trigger\_reason": "\textless{}why threshold is considered exceeded or cross-day pattern confirmed\textgreater{}",
      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}assistant coaching reminder, like a health band: e.g., you've been sitting for a long time, want to stand or stretch?\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}likely user reply (\textgreater{}= 10-12 words), may accept/decline/adjust\textgreater{}"
        \},
        \{
          "role": "assistant",
          "utterance": "\textless{}follow-up: confirm reminder, suggest simple action, or gently back off\textgreater{}"
        \}
      ]
    \}
  ]
\}

\#\#\#\# Notes \& Constraints
	•	habit\_state\_updates:
    •   In practice, habit\_state\_updates is mainly used for Type B cross\_day\_lifestyle patterns (e.g., sleep time, late-night work end time, main meal times). You do not need to exhaustively log every Type A intra\_day event.
	•	Only needs to include new or updated habits/occurrences from this batch (not all history).
	•	For the very first batch with no history:
    •	habit\_summary: "initial hypothesis of an unhealthy habit pattern in this batch."
    •	historical\_context: "no prior records; first detected in this batch."
    •	habit\_triggers: Each entry corresponds to one concrete coaching moment in this batch.
    •	trigger\_type:
      •   intra\_day\_threshold: same-day accumulation (e.g., prolonged sitting, no drinking, long uninterrupted screen use).
      •   cross\_day\_pattern: e.g., reminding the user in the evening, “You went to bed very late yesterday — try to rest earlier tonight.”
	•	You must NOT invent time\_window; copy from existing fine-grained entries as defined above.
	•	*Do not repeatedly activate the same event or generate identical dialogue content.*

⸻

\#\#\#\# Failure Case Format
If you find no unhealthy habit accumulations and no cross-day lifestyle patterns that justify a coaching reminder:
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Habit-Coaching Proactive Service",
  "habit\_state\_updates": [],
  "habit\_triggers": [],
  "note": "No unhealthy accumulation or cross-day lifestyle habit requiring coaching was detected in this batch, given the current annotations and historical summary."
\}
\end{promptbox}

\begin{promptbox}[EgoLife — Long-Term · Memory-Link]
\#\#\# Task Context

You are analyzing MULTIPLE egocentric annotation files (each less than 10 minutes) from the EgoLife dataset for one contiguous batch of time (less than 2.5 hours).

Your job in this stage is signal mining for a special Long-Term Proactive Service subtype:

•	service\_main\_type: "Long-Term Proactive Service"
•	service\_sub\_type: "Memory-Link Contextual Proactive Service"
(short: Memory-Link Service)

This service is about long-horizon memory across days or long gaps within a day (typically ≥ 2 hours).
This includes:
	•	cross-day links (DAY1 → DAY2/3/…)
	•	same-day links with a substantial temporal gap (typically ≥ 2 hours) between the earlier event and the current one.

In this stage, you must perform two related but distinct subtasks:
	1.	Type A - Future-impact memory hooks (to be stored as memory for later)
    Find events in the current batch that should be remembered because they are likely to matter later or create a potential link to future behavior.
    In other words:
    "If the system remembers this now, it can help with something that happens later."

    Typical examples:
        •	"I put the spare key behind this plant (so I can find it in an emergency)."
        •	"I promised to review this document tomorrow."
        •	"I left the box under the bed for later reuse."
        •	"I created a detailed engineering plan that will need to be executed step by step later."
    All such hooks from the current batch must be output under new\_memory\_candidates, and will be reused as historical memory in future batches.
	
  2.	Type B - Realized memory links (use past memory now + generate dialogue)
    Using the current batch together with the historical memory JSON (past Type A hooks and their follow-ups), find current events that reuse, depend on, or are made easier by some earlier event or piece of information.
    In other words:
    "This current action works better because I remember / rely on something that happened before."

    Typical examples:
        •	retrieving the spare key from behind the plant where it was hidden yesterday
        •	using the box that was intentionally stored under the bed the day before
        •	following up on a promise or prior instruction ("I'll now review the slides I promised you yesterday.")
        •	recalling something someone said earlier that now helps solve a problem
        •	e.g., "Yesterday they mentioned this trick with the router; I'll try it now to fix the connection."
    For each such realized link, you must output a realized\_memory\_links entry and generate a short multi-turn dialogue where the assistant proactively leverages the remembered past event to help in the current situation.

You will receive two types of input:
	1.	Current batch annotations (required): multiple segment-level human annotations for this contiguous time window.
	2.	Historical memory summary JSON (optional): all previously mined Memory-Link candidates that might matter for future (Type A) or already had some follow-ups (Type B).

Important:
	•	If the historical JSON is missing or empty, treat this as the first mining pass and assume there are no past events.
	•	In that case, you MUST set "realized\_memory\_links": [] in the output, because there is no earlier memory that can be linked; you only mine new Type A hooks.

You must NOT guess new events, invent timestamps, or hallucinate behaviors not supported by the annotations.

⸻

\#\#\# Authoritative Timestamps

Every annotation entry has a time\_window aligned to the original video, for example:
	•	i\_do\_steps[].time\_window
	•	interactions\_with\_objects[].time\_window
	•	interactions\_with\_people[].time\_window
	•	speakers\_say[].time\_window

All time\_window strings already have the format:

DAY\# HH:MM:SS-HH:MM:SS

You MUST only copy these existing time\_window values.
Do NOT interpolate or invent new time ranges.

⸻

\#\#\# Input Human Annotations

1. Current batch: segment-level episodic annotations
You are given MULTIPLE JSON objects, each representing a \textless{}10-minute egocentric segment:
\{
  "segment\_id": "\textless{}identifier for this \textasciitilde{}10-minute segment\textgreater{}",
  "description": "... high-level summary of what I do in this segment ...",
  "interaction\_records": [
    \{
      "time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "description": "... micro-episode summary ...",

      "i\_do\_steps": [ ... ],
      "speakers\_say": [ ... ],
      "interactions\_with\_objects": [ ... ],
      "interactions\_with\_people": [ ... ],
      "environment\_state": [ ... ],
      "task\_transition": [ ... ],
      "confidence": 0.0-1.0
    \}
  ]
\}
These interaction\_records and their subfields are your primary evidence.

The coverage of this batch is defined by the minimum and maximum timestamps appearing in these JSONs.

⸻

2. Historical memory summary JSON (optional memory)

This historical JSON has the same schema as the new\_memory\_candidates you will output in this stage.
In later runs, the system will feed your previous new\_memory\_candidates as memory\_events in this historical JSON.
Therefore, new\_memory\_candidates should only contain Type A - future-impact memory hooks that are worth remembering for future batches.

You may also receive ONE historical JSON summarizing previously mined memory-relevant events (Future-impact memory hooks) and triggered realized memory links, with the following structure:
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Memory Link Contextual Proactive Service",
  "memory\_events": [
    \{
      "event\_id": "mem\_001",
      "memory\_key": "\textless{}abstract description of this memory-relevant pattern\textgreater{}",
      "memory\_type": "future\_hook \textbar{} realized\_link \textbar{} mixed",
      "memory\_summary": "\textless{}how this memory pattern unfolded over previous hours/days\textgreater{}",

      "occurrences": [
        \{
          "segment\_id": "\textless{}old segment id\textgreater{}",
          "time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
          "supporting\_source": "i\_do\_steps \textbar{} interactions\_with\_objects \textbar{} interactions\_with\_people \textbar{} speakers\_say",

          "observation": "\textless{}what happened\textgreater{}",
          "local\_context": "\textless{}local scene / surroundings\textgreater{}",
          "historical\_context": "\textless{}how it related to earlier ones\textgreater{}",
          "inferred\_link\_role": "initial\_hook \textbar{} followup\_use \textbar{} reminder \textbar{} unresolved\_plan \textbar{} other",
          "link\_target\_ids": ["mem\_000", "mem\_005"],

          "workflow\_position": "start \textbar{} middle \textbar{} end \textbar{} standalone",
          "social\_dynamics": "self-initiated \textbar{} reacting\_to\_others \textbar{} jointly\_decided",
          "occurrence\_confidence": 0.0
        \}
      ]
    \}
  ],
  
  "historical\_realized\_memory\_links": [
    \{
      "link\_id": "mlink\_00Y",

      "current\_segment\_id": "\textless{}current segment id\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "supporting\_source": "i\_do\_steps \textbar{} speakers\_say",

      "current\_observation": "\textless{}what happens now that uses/depends on a past event\textgreater{}",
      "current\_local\_context": "\textless{}current scene / situation\textgreater{}",
      "inferred\_link\_role": "followup\_use \textbar{} reminder \textbar{} check\_status \textbar{} other",

      "linked\_past\_events": [
        \{
          "event\_id": "mem\_00A",
          "memory\_key": "\textless{}copied from history\textgreater{}",
          "past\_segment\_id": "\textless{}segment\_id of the past occurrence\textgreater{}",
          "past\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
          "link\_reason": "\textless{}why this current event is a follow-up to that past event\textgreater{}"
        \}
      ],

      "workflow\_position": "start \textbar{} middle \textbar{} end \textbar{} standalone",
      "social\_dynamics": "self-initiated \textbar{} reacting\_to\_others \textbar{} jointly\_decided",
      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}first turn: assistant proactively referencing the remembered past event and offering help now\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}likely user response\textgreater{}"
        \},
        \{
          "role": "assistant",
          "utterance": "\textless{}second assistant turn, refining help based on user response\textgreater{}"
        \}
      ]
    \}
  ]
\}
This historical JSON is read-only memory and is a global aggregation over all previous time ranges.
	•	Each memory\_key should describe one type of "remember this to help later" pattern, not a vague category.
	•	It should roughly answer:
        "What did I do / say / place earlier that could matter later, and in what situation will it matter?"

Examples of good memory\_key:
	•	"Put spare apartment key behind the big plant near the door for emergencies"
	•	"Told labmate I will review their slides the next morning"
	•	"Store the cardboard boxes under the bed for future packing"
	•	"Write Wi-Fi password on a note next to the router for visitors"

The occurrences under that memory\_key are concrete historical events:
	•	sometimes the initial memory hook (e.g., "I put the key behind the plant"),
	•	sometimes a follow-up use (e.g., "I later take the key from behind the plant").

If the historical JSON is not provided or contains an empty list, treat this as no prior memory.

⸻

\#\#\#\# Service Category
	•	service\_main\_type: Long-Term Proactive Service
	•	service\_sub\_type: Long-Horizon Memory-Link Contextual Proactive Service

You must:
	1.	In the current batch, find:
        •	Events that should be remembered because they may help in the future (future hooks).
        •	Events that reuse or depend on earlier memory hooks (realized links).
	2.	Integrate with historical memory events when possible:
        •	Reuse existing memory\_key where appropriate.
        •	Link new follow-ups to earlier event\_ids, and explicitly copy the timestamps of the linked past events into the output.
        •   For each realized memory link, generate a short multi-turn dialogue between the assistant and the user grounded in these linked events.

⸻

\#\#\# Fine-Grained Evidence Priority (critical)

When detecting candidate occurrences, you must prioritize fine-grained entries before falling back to coarse summaries:

\#\#\#\# Primary sources for discovering memory-relevant events  
   • i\_do\_steps  
   • interactions\_with\_objects  
   • interactions\_with\_people  
   • speakers\_say  

→ Treat each fine-grained entry as a potential memory hook or realized link if its content matches the Memory-Link definition.  
→ You must copy the `time\_window` directly from these fine-grained entries only.

This priority applies to both:  
   • which content you consider as occurrences, and  
   • which `time\_window` you copy for those occurrences.

Strict constraints on timestamps:  
   • You must never use `interaction\_record.time\_window`.  
   • You must never merge, split, expand, or shorten any existing `time\_window`.  
   • You must never create a new or "combined" `time\_window` (e.g., by joining two ranges or inventing a midpoint).  
   • For every occurrence, you must copy one existing `time\_window` string exactly as it appears in the fine-grained annotations.

⸻

\#\#\# What counts as a Memory-Link signal?

We distinguish two roles:
	•	Type A - Future-impact memory hook:
    Something is done/said/placed now so that it can be leveraged later.
    (Current batch → future.)
	•	Type B - Realized memory link:
    A current action clearly refers back to, or makes use of, an earlier event.
    (Past → current batch.)

Only Type A - future-impact memory hooks are written into new\_memory\_candidates and will be carried forward as long-horizon memory for future batches.
Type B - realized memory links are reported only in realized\_memory\_links for this batch and are not stored as new memory hooks.

A single occurrence is enough to record a candidate, as long as it clearly fits one of these roles.

\#\#\#\# A. Future-impact memory hooks (in the current batch)
You are looking for events where the user creates a future resource, landmark, or commitment that only becomes useful later if remembered.

Typical patterns:
	1.	Place or configure something for later use
        •	Hiding or storing important items in specific places for later retrieval:
            •	putting a spare key behind a plant or under a mat
            •	placing a package in a specific corner "for later pickup"
            •	storing boxes under the bed for future packing
        •	Preparing tools/materials clearly intended for future tasks:
            •	pre-labeling boxes or cables for future organization
            •	pre-charging multiple devices for tomorrow's recording
	2.	Verbal commitments, instructions, or future-facing notes
        •	Making promises or plans that require remembering later:
            •	"I'll review your slides tomorrow morning."
            •	"Let's continue this discussion after lunch."
        •	Leaving instructions or explanations meant for future self/others:
            •	explaining where something is stored or how to operate something later
            •	saying "I'm putting the spare key here so I don't forget."
    3.	Creating explicit future reference points
        •	Writing down info in a place that will be used later:
            •	writing Wi-Fi password on a note near the router
            •	labeling shelves/boxes so others can find items later
        •	Setting up long-running processes that will need attention:
            •	starting an overnight download and saying when to check it
            •	starting a slow-cooking process that must be checked later

If such an event appears now (in the current batch), you should output it as a future-impact candidate even if the actual follow-up has not happened yet.

\#\#\#\# B. Realized memory links (current batch uses past events)
You are looking for events where the user benefits from or explicitly references something done earlier.

Typical patterns:
	1.	Retrieving or using a previously placed item
        •	Taking the spare key from behind the plant / under the mat.
        •	Pulling out the labeled box that was prepared the day before.
        •	Using the pre-charged device that was plugged in yesterday for today's task.
	2.	Following up on a prior promise, plan, or instruction
        •	Reviewing the slides that were promised for "tomorrow".
        •	Joining a meeting that was scheduled in a previous day's clip.
        •	Resuming a task exactly where a previous "pause" or bookmark was left.
	3.	Explicit verbal reference to past actions
        •	"I left this here yesterday so I could find it today."
        •	"This is the box I prepared last time."
        •	"As I said before, I'll now check the results."

Strict requirement for realized\_memory\_links:
You MUST only output a realized link when you can directly associate the current event with at least one concrete past occurrence from the historical JSON (or from earlier in this batch when historical JSON is present).
Each realized link must explicitly list which past events it is linked to.
Additionally, for within-day links:
    • Only treat a current event as a realized\_memory\_link if the linked past occurrence is separated by a clearly later episode in time (typically ≥ 2 hours apart, or obviously different sessions such as a morning planning clip vs. an evening execution clip).
    • Short within-episode references (e.g., a few minutes apart in one continuous task) should not be labeled as long-horizon realized links; those belong to local task structure or routine optimization instead.

If no suitable past event can be found in the historical JSON, do NOT create a realized link; instead treat the current event as:
	•	a new future-impact hook (if it is forward-looking), or
	•	not Memory-Link (if purely local).

⸻

\#\#\#\# Exclusions

Do NOT classify as Memory-Link events:
	•	one-off random actions with no clear future relevance
	•	generic organization with no clear future scenario (e.g., quick tidy-up without any hint it matters later)
	•	pure safety actions → Safety Proactive Service
	•	short-horizon corrections within the same small task → Short-Horizon Error-Recovery
    •   short-gap references within the same session (e.g., a step referring to something done a few minutes ago within one continuous workflow), even if they "mention the past", but do not require remembering across a long gap (≥ 2 hours) or a distinct episode → treat as local task structure or Routine Optimization, not Memory-Link.
	•	long-term health/productivity habits (hydration / posture / breaks) → Habit-Coaching Proactive Service
	•   Pure configuration preferences or generic multi-step efficiency routines whose main value is "make the current workflow smoother/faster" but do NOT clearly depend on being remembered for a future moment  
        → Routine Optimization Proactive Service (this includes both "pure configuration preferences" and "generic efficiency routines" that are not true Memory-Link cases)

Simple memory test:
	•	If the usefulness is "right now only" → probably NOT Memory-Link.
	•	If the main value is "I/others can remember this later and it will help then" → candidate for Memory-Link.

⸻

\#\#\# Memory Key Granularity Rules

Goal: keep each memory\_key narrow and concrete enough so that it corresponds to one clear type of "remember this for later" pattern, instead of a giant mix.

For every memory\_key, you should be able to summarize all its occurrences with one short template:

"When I [do/say/place X] in [this kind of situation], it is so that later I / others can [do Y more easily]."

Only when all occurrences naturally fit this one sentence should they share the same memory\_key.

Bad examples (too broad / vague):
	•	"General Organization"
	•	"Technical Discipline"
	•	"Remember Things"

Good examples:
	•	"Hide spare apartment key behind the plant near the door for emergencies later"
	•	"Store moving boxes under the bed so they are ready for future packing"
	•	"Tell labmate I'll review their slides the next morning"
	•	"Write Wi-Fi password on a note next to router for guests"

If you cannot write such a single "remember this for later" sentence without becoming vague, the key is too broad and should be split.

⸻

\#\#\# Historical Integration Rules

1. When to reuse an existing memory\_key
Given a new occurrence in the current batch and an existing memory\_key from history, reuse that key (and its event\_id) only if:
	1.	Target alignment
        It involves the same object / info / resource
        (e.g., same spare key, same specific boxes, same Wi-Fi note, same slides).
	2.	Memory role alignment
        The new occurrence fits the same type of memory pattern:
        •	same kind of hook (placing/storing/committing for later), or
        •	same kind of follow-up use / reference.
	3.	Future/Current scenario alignment
        The imagined or actual later scenario is similar:
        •	same emergency key usage,
        •	same future packing task,
        •	same "review tomorrow" pattern.

If these three align:
	•	Reuse the same memory\_key and event\_id in memory\_events.
	•	Add a new occurrence under it.
	•	Set inferred\_link\_role appropriately:
        •	initial\_hook for the first "store/commit for later" behavior,
        •	followup\_use when the user benefits from it later,
        •	unresolved\_plan if the plan is stated but not yet followed up in this batch.

2. When to create a NEW memory\_key
Create a new memory\_key (and a new event\_id) when:
  • The object/info being stored is clearly different  
    - e.g., different physical item, different key set, different document group, different device.  
  • The future use scenario is different  
    - e.g., emergency retrieval vs. routine convenience vs. social courtesy (like "remind me to bring a gift").  
  • The memory pattern or storage strategy is structurally different  
    - e.g., "tell a person verbally" vs "leave a written note" vs "place it in a fixed drawer" as part of a different routine.

When you create a new event\_id, you MUST:
  • Use the global `"mem\_XXX"` format (e.g., `mem\_001`, `mem\_002`, …).  
  • Scan all existing `event\_id` in the historical JSON, find the maximum numeric index, and assign the next integer (zero-padded to 3 digits).  
  • Example: if existing IDs are `mem\_001` and `mem\_002`, the next new `event\_id` MUST be `mem\_003`.  
  • You MUST NOT rename, reuse, or renumber any existing `event\_id`.

⸻

\#\#\# Objective

For the current batch of segments (time span determined by timestamps, often less than \textasciitilde{}2.5 hours), with optional historical memory, you must perform both long-horizon memory state updating and trigger activation:
	1.	Update long-horizon memory state (new\_memory\_candidates / memory\_events)
        • Scan all segments and interaction\_records in the current batch to find every occurrence that qualifies as a future-impact memory hook (Type A), i.e., actions, placements, or verbal commitments that are clearly intended to help at some later moment if remembered.
        • When deciding whether to reuse an existing memory\_key or create a new one, you MUST follow the Memory Key Granularity Rules strictly, so that each memory\_key consistently represents one coherent "remember this for later" pattern.
        • When integrating new occurrences with the historical memory summary JSON, you MUST follow the Historical Integration Rules strictly, including:
            - Reusing an existing memory\_key / event\_id only when the target, memory role (hook vs follow-up), and imagined future scenario align with the existing pattern.
            - Creating a new memory\_key and a new event\_id (in the global "mem\_XXX" scheme) when the object/info, future scenario, or storage strategy is meaningfully different.
        • For each memory\_key (identified by event\_id), append new occurrences capturing:
            - segment\_id, time\_window, supporting\_source (from fine-grained entries only),
            - observation, local\_context,
            - historical\_context (how this relates to earlier hooks/uses under the same memory\_key),
            - inferred\_link\_role (initial\_hook or unresolved\_plan for Type A),
            - workflow\_position, social\_dynamics, and occurrence\_confidence.
        • For each memory\_key you touch in this batch, update:
            - memory\_summary: how this batch extends, confirms, or refines the long-horizon memory pattern,
            - batch\_consistency\_level and batch\_confidence: your overall judgment of how coherent and reliable the pattern looks in this batch.

	2.	Decide current-batch realized memory links and generate dialogues (realized\_memory\_links)
        • Using the historical memory\_events (if provided) together with all fine-grained entries in the current batch, scan for realized memory links (Type B) where a current action or utterance clearly uses, depends on, or explicitly refers back to a past memory hook, with a sufficiently long temporal gap (typically ≥ 2 hours or clearly different sessions such as "yesterday vs today" or "morning planning vs evening execution").
        • For each candidate realized link:
            - Identify the earliest fine-grained i\_do\_steps[].time\_window or speakers\_say[].time\_window in the current batch where the user first starts to use the remembered object/info/plan (e.g., begins retrieving the stored item, opens the document they promised to review, starts using the pre-prepared resource).
            - Set this as current\_time\_window and choose supporting\_source accordingly (i\_do\_steps or speakers\_say).
            - Link this current occurrence to at least one past occurrence in the historical memory JSON by filling linked\_past\_events with the corresponding event\_id, memory\_key, past\_segment\_id, and past\_time\_window, and describe the link\_reason (why the current behavior is a follow-up to that past event).
            - Set inferred\_link\_role appropriately (e.g., followup\_use, reminder, check\_status, other), and record workflow\_position, social\_dynamics, and occurrence\_confidence.
        • For every activated realized link, you MUST also generate a short multi-turn proactive dialogue under proactive\_dialogue that:
            - Is initiated by the assistant at current\_time\_window,
            - Explicitly and helpfully leverages the remembered past event to assist the user now (e.g., retrieving the plan they made, checking steps they prepared, reminding of where they stored something),
            - Follows the dialogue rules defined later in this prompt (assistant starts, user responds naturally, assistant follows up with a concrete micro-service),
            - Stays grounded in the linked past event and the current physical/interaction context, without mentioning videos, annotations, or models.
        • If no historical JSON is provided or it is empty:
            - You may still output new\_memory\_candidates from this batch (Type A hooks),
            - But you MUST set "realized\_memory\_links": [] because there is no earlier memory to link to.
        • The "historical\_realized\_memory\_links" field in the Historical Memory Summary JSON is used to assist in activating memory-link events.
⸻

\#\#\# Trigger Time-Window Rules (strict)

When you output current\_time\_window for any trigger, you MUST:

1. Only copy an existing `time\_window` string from:
   - `i\_do\_steps[].time\_window`, or  
   - `speakers\_say[].time\_window`.

2. You may still use `interactions\_with\_objects` and `interactions\_with\_people` as supporting evidence for detecting habits or patterns,  
   but you are NOT allowed to use their `time\_window` fields directly as `current\_time\_window`.

3. You must copy one of the allowed time\_window strings exactly as-is.  
   Do NOT invent, merge, extend, or shrink any time range.

If in doubt, keep separate occurrences with their own `current\_time\_window` instead of fusing them.

⸻

\#\#\# Output Format (single JSON with two sections)

Your output must be ONE JSON object that contains both types of results for the current batch:
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Memory Link Contextual Proactive Service",

  "new\_memory\_candidates": [ \textless{}Type A future-impact memory hook\textgreater{}
    \{
      "event\_id": "mem\_00X",
      "memory\_key": "\textless{}abstract but concrete memory pattern\textgreater{}",
      "memory\_summary": "\textless{}summary of this memory pattern within the current batch, optionally referencing earlier days\textgreater{}",
      "memory\_type": "future\_hook",

      "occurrences": [
        \{
          "segment\_id": "\textless{}source segment file name\textgreater{}",
          "time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
          "supporting\_source": "i\_do\_steps \textbar{} interactions\_with\_objects \textbar{} interactions\_with\_people \textbar{} speakers\_say",

          "observation": "\textless{}specific action or speech that creates a future-impact memory hook\textgreater{}",
          "local\_context": "\textless{}what is around / scene state\textgreater{} (optional but recommended)",
          "historical\_context": "\textless{}how this occurrence relates to previous hooks of the same memory\_key, if any\textgreater{}",
          "inferred\_link\_role": "initial\_hook \textbar{} unresolved\_plan",
          "link\_target\_ids": [],

          "workflow\_position": "start \textbar{} middle \textbar{} end \textbar{} standalone",
          "social\_dynamics": "self-initiated \textbar{} reacting\_to\_others \textbar{} jointly\_decided",
          "occurrence\_confidence": 0.0
        \}
      ],

      "batch\_consistency\_level": "high \textbar{} medium \textbar{} low",
      "batch\_confidence": 0.0
    \}
  ],

  "realized\_memory\_links": [
    \{
      "link\_id": "mlink\_00Y",

      "current\_segment\_id": "\textless{}current segment id\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "supporting\_source": "i\_do\_steps \textbar{} speakers\_say",

      "current\_observation": "\textless{}what happens now that uses/depends on a past event\textgreater{}",
      "current\_local\_context": "\textless{}current scene / situation\textgreater{}",
      "inferred\_link\_role": "followup\_use \textbar{} reminder \textbar{} check\_status \textbar{} other",

      "linked\_past\_events": [
        \{
          "event\_id": "mem\_00A",
          "memory\_key": "\textless{}copied from history\textgreater{}",
          "past\_segment\_id": "\textless{}segment\_id of the past occurrence\textgreater{}",
          "past\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
          "link\_reason": "\textless{}why this current event is a follow-up to that past event\textgreater{}"
        \}
      ],

      "workflow\_position": "start \textbar{} middle \textbar{} end \textbar{} standalone",
      "social\_dynamics": "self-initiated \textbar{} reacting\_to\_others \textbar{} jointly\_decided",
      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}first turn: assistant proactively referencing the remembered past event and offering help now\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}likely user response\textgreater{}"
        \},
        \{
          "role": "assistant",
          "utterance": "\textless{}second assistant turn, refining help based on user response\textgreater{}"
        \}
      ]
    \}
  ]
\}
Hard constraints for realized\_memory\_links:
	•	If no historical JSON is provided, you MUST set:
        "realized\_memory\_links": []
	•	For every realized\_memory\_links item:
        •	linked\_past\_events MUST contain at least one entry, each with event\_id, past\_segment\_id, and past\_time\_window copied from the historical JSON.
        •	proactive\_dialogue MUST be a multi-turn dialogue (≥ 3 turns) showing how the assistant could use the remembered past event to help the user in the current situation.
        •	The dialogue must sound like a natural real-time assistant (do NOT mention "video", "annotations", or "model").
  •	*Do not repeatedly activate the same event or generate identical dialogue content.*

* Additional Dialogue Rules: *
    - For every realized\_memory\_links item, current\_time\_window MUST be exactly the time range where the user is first seen speaking/acting in a way that uses or starts to use the past event (e.g., the moment they begin the move, open the document, start the dance practice), not a later summary window.
    - For realized\_memory\_links, current\_time\_window MUST be copied from either i\_do\_steps[].time\_window or speakers\_say[].time\_window only. You MUST NOT use time windows from interactions\_with\_objects or interactions\_with\_people as current\_time\_window, even if they describe related context.
    - If multiple i\_do\_steps / speakers\_say entries are involved in the same realized link, you MUST choose the earliest time\_window where the user first starts the memory-dependent action or verbal reference (the first step or first utterance that actually uses the past event).
    - The assistant must initiate help right at this current\_time\_window, when the remembered information becomes practically useful in the ongoing action.
    - The first assistant utterance should offer a concrete, task-relevant assistance based on the linked past event (e.g., "Do you want me to follow the moving plan you made yesterday?").
    - The user's first reply should either confirm or refine the assistance; the assistant must then follow up with a helpful action (checking, summarizing, retrieving info, validating progress).
    - The dialogue must stay grounded in the current physical action and the past memory link, without referencing videos, annotations, or models.
    - The final assistant turn should complete a useful micro-service (e.g., verifying steps, retrieving past notes, confirming plans, or tracking progress) based strictly on the remembered information.⸻

If no historical JSON is provided:
	•	You can still output new\_memory\_candidates for hooks detected in this batch.
    •	In subsequent batches, the new\_memory\_candidates you output here will be loaded back as memory\_events in the historical JSON. Treat them as seeds of long-horizon memory that future realized links may refer to.
	•	For every new memory\_key:
        •	memory\_summary: "initial hypothesis of a possible long-horizon memory pattern in this batch."
        •	historical\_context in its occurrences: "no prior records; first detected in this batch."

⸻

\#\#\#\# Failure Case Format

If you find no memory-link related occurrences in the current batch:
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Memory Link Contextual Proactive Service",
  "new\_memory\_candidates": [],
  "realized\_memory\_links": [],
  "note": "No long-horizon memory-related hooks or realized links were detected in this batch, given the current annotations and historical summary."
\}
\end{promptbox}

\begin{promptbox}[EgoLife — Long-Term · Personal Feedback]
\#\#\# Task Context

You are analyzing MULTIPLE egocentric annotation files (each less than 10 minutes) from the EgoLife dataset for one contiguous batch of time (less than 2.5 hours).

Your job in this stage is signal mining and proactive feedback for a special Long-Term Proactive Service subtype:

•	service\_main\_type: "Long-Term Proactive Service"
•	service\_sub\_type: "Personal Progress Feedback Proactive Service"
(short: Progress Feedback Service)

This service focuses on skill learning / personal goals / performance tracking across sessions.
Beyond tracking, the core goal of this service is to give the user meaningful, emotionally supportive feedback and concrete, small-scale suggestions.
Your feedback should
	•	briefly evaluate the user's progress or persistence,
	•	provide emotional value (encouragement, acknowledgement, or gentle normalization of difficulty), and
	•	propose 1-2 realistic, actionable suggestions for future attempts.
Merely restating what the user just did without evaluation or suggestions is not allowed.

Typical examples:
	•	The user's cooking steps become smoother or faster over multiple days.
	•	Study or homework tasks are completed more consistently.
	•	Repeated practice motions (e.g., dance, sports, instrument, lab technique) become more standard, fluent, or complete.

You must both:
	1.	Accumulate progress-related events into a structured state (for long-term tracking), and
	2.	Within the current batch, detect moments that deserve immediate progress feedback and generate a short multi-turn dialogue.

⸻

\#\#\# Core Signal Types

Within this batch, you focus on two complementary types of events:
	1.	Type A - Progress evidence events (state accumulation)
    Concrete episodes that show practice, execution, completion, or qualitative change for a specific skill / goal / performance pattern.
    Examples:
        •	Practicing the same chopping / cutting technique during cooking.
        •	Repeating the same dance routine or exercise drill.
        •	Doing a similar homework / study task again.
        •	Running through the same lab / work procedure with more fluency.
	2.	Type B - Feedback-worthy moments (activation + dialogue)
    Specific episodes where, given previous occurrences of the same pattern, it is valuable for the assistant to:
        •	Summarize improvement,
        •	Highlight persistence or effort, or
        •	Offer constructive micro-feedback or next-step suggestions.

These Type B moments must be grounded in longitudinal comparison:
	•	Cross-day (DAY1 → DAY2/3/…), or
	•	Same-day but clearly separate sessions (typically ≥ 2 hours apart, or distinct blocks like "morning practice" vs "evening practice").

You must NOT guess new events, invent timestamps, or hallucinate behaviors not supported by the annotations.

⸻

\#\#\# Authoritative Timestamps

Every fine-grained annotation entry has a time\_window aligned to the original video, for example:
	•	i\_do\_steps[].time\_window
	•	interactions\_with\_objects[].time\_window
	•	interactions\_with\_people[].time\_window
	•	speakers\_say[].time\_window

All time\_window strings already have the format:

DAY\# HH:MM:SS-HH:MM:SS

You MUST only copy these existing time\_window values.
Do NOT interpolate, merge, extend, shrink, or invent new time ranges.

⸻

\#\#\# Input Human Annotations

1. Current batch: segment-level episodic annotations

You are given MULTIPLE JSON objects, each representing a \textless{}10-minute egocentric segment:
\{
  "segment\_id": "\textless{}identifier for this \textasciitilde{}10-minute segment\textgreater{}",
  "description": "... high-level summary of what I do in this segment ...",
  "interaction\_records": [
    \{
      "time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "description": "... micro-episode summary ...",

      "i\_do\_steps": [ ... ],
      "speakers\_say": [ ... ],
      "interactions\_with\_objects": [ ... ],
      "interactions\_with\_people": [ ... ],
      "environment\_state": [ ... ],
      "task\_transition": [ ... ],
      "confidence": 0.0-1.0
    \}
  ]
\}

These interaction\_records and their subfields are your primary evidence.

The coverage of this batch is defined by the minimum and maximum timestamps appearing in these JSONs.

⸻

2. Historical progress summary JSON (optional memory)

You may also receive ONE historical JSON summarizing previously mined progress-related events and triggered feedback dialogues, with the following structure:
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Personal Progress Feedback Proactive Service",
  "progress\_events": [
    \{
      "progress\_id": "pprog\_001",
      "progress\_key": "\textless{}abstract description of one skill/goal/performance pattern\textgreater{}",
      "progress\_type": "skill\_learning \textbar{} personal\_goal \textbar{} performance \textbar{} habitual\_task",
      "progress\_summary": "\textless{}how this pattern has evolved over previous hours/days\textgreater{}",

      "occurrences": [
        \{
          "segment\_id": "\textless{}old segment id\textgreater{}",
          "day\_id": 1,
          "time\_window": "DAY1 HH:MM:SS-HH:MM:SS",
          "supporting\_source": "i\_do\_steps \textbar{} interactions\_with\_objects \textbar{} interactions\_with\_people \textbar{} speakers\_say \textbar{} interaction\_record",

          "observation": "\textless{}what happened\textgreater{}",
          "local\_context": "\textless{}local scene / surroundings\textgreater{}",
          "metrics": \{
            "practice\_minutes": 8.0,
            "attempt\_count": 3,
            "quality\_trend": "struggling \textbar{} partial\_success \textbar{} clear\_success \textbar{} unclear"
          \},
          "historical\_context": "\textless{}how it related to earlier ones\textgreater{}",
          "effort\_type": "practice \textbar{} execution \textbar{} review \textbar{} planning",
          "outcome\_quality": "improved \textbar{} similar \textbar{} worse \textbar{} unclear",
          "workflow\_position": "start \textbar{} middle \textbar{} end \textbar{} standalone",
          "social\_dynamics": "self-initiated \textbar{} reacting\_to\_others \textbar{} jointly\_decided",
          "occurrence\_confidence": 0.0
        \}
      ]
    \}
  ],
  
  "historical\_feedback\_triggers": [
    \{
      "trigger\_id": "pfeed\_001",
      "progress\_id": "pprog\_001",
      "progress\_key": "\textless{}copied from progress\_state\_updates\textgreater{}",
      "trigger\_type": "cross\_session\_progress \textbar{} sustained\_effort \textbar{} milestone\_completion",

      "current\_segment\_id": "\textless{}segment id where feedback is triggered\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "supporting\_source": "i\_do\_steps \textbar{} speakers\_say",

      "current\_observation": "\textless{}what just happened that makes this a good feedback moment\textgreater{}",
      "current\_local\_context": "\textless{}short description of current scene\textgreater{}",
      "comparison\_basis": "\textless{}how this compares to earlier runs / sessions\textgreater{}",
      "trigger\_reason": "\textless{}why feedback is considered helpful now\textgreater{}",
      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}assistant proactive feedback, referencing cross-session progress\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}likely user reply (\textgreater{}= 12 words)\textgreater{}"
        \}
        // optionally 1-2 more turns, alternating assistant ↔ user
      ]
    \}
  ]
\}

Notes:
	•	progress\_key must describe one concrete skill/goal/performance area (e.g., "chopping vegetables for cooking", "evening English homework session", "repeating the same dance routine"), not a vague category like "study" or "exercise".
	•	progress\_id is a stable identifier for that progress\_key across days.
	•	day\_id is derived from the DAY\# prefix of time\_window.

If the historical JSON is missing or progress\_events is empty, treat this as no prior progress memory.

⸻

\#\#\# Fine-Grained Evidence Priority (critical)

When detecting candidate occurrences, you must prioritize fine-grained entries before falling back to coarse summaries:

Primary sources for progress-related events
	•	i\_do\_steps
	•	interactions\_with\_objects
	•	interactions\_with\_people
	•	speakers\_say

→ Treat each fine-grained entry (or short, coherent cluster within the same context) as a potential practice/execution episode if it clearly involves:
	•	repeating or performing a recognisable skill or task,
	•	making progress toward a personal goal, or
	•	showing a change in fluency / quality / completion status.

Timestamp rules for occurrences
	•	For every occurrence in progress\_state\_updates, you must copy one existing time\_window directly from
        i\_do\_steps, interactions\_with\_objects, interactions\_with\_people, or speakers\_say.
	•	You must never use interaction\_record.time\_window for occurrences.
	•	You must never merge, split, or invent time\_window ranges.

Additional strict rule for feedback dialogue triggers (see below):
	•	For feedback\_triggers.current\_time\_window, you may only copy from:
	•	i\_do\_steps[].time\_window or
	•	speakers\_say[].time\_window.

⸻

\#\#\# What counts as Personal Progress Feedback signal?

You care about learning curves and progress trajectories, not just single successes.

Positive signals (examples):
	•	Repeated attempts at the same skill with signs of:
	•	smoother execution,
	•	fewer hesitations / corrections,
	•	better timing or coordination,
	•	higher completion rate.
	•	Consistent continuation of a personal goal:
	•	regular study/homework sessions,
	•	repeated practice of a dance move,
	•	ongoing work on the same project steps.
	•	Explicit self-reflection or evaluation in speech:
        •	"I'm getting faster at this now."
        •	"This time the movement felt more stable."
        •	"Today I finally finished the whole sequence."

You should NOT treat as Progress Feedback:
	•	Pure safety behaviors (→ Safety Proactive Service).
	•	Pure configuration preferences without a learning/progress angle (→ Routine Optimization / Preference).
	•	Generic health habits like exercising or stretching without clear skill/goal tracking (→ Habit-Coaching).
	•	One-off tasks with no sign of repetition or progress trajectory.

Simple test:
	•	If the main value is "I'm getting better / more consistent at this over time" → candidate for Progress Feedback.
	•	If the main value is "this is just done or configured now" → likely belongs to another service.

⸻

\#\#\# Progress Key Granularity Rules

Each progress\_key should capture one skill/goal/performance pattern that you can describe with:

"When I practice or perform [X] in [this context] across sessions, my fluency/completion/quality can improve and deserves feedback."

Bad examples (too broad / vague):
	•	"General Learning"
	•	"Work Tasks"
	•	"Daily Exercise"

Good examples:
	•	"Chopping vegetables for cooking dinner in the kitchen"
	•	"Evening English homework sessions at the desk"
	•	"Practicing the same hip-hop dance routine in the living room"
	•	"Running through the same instrument warm-up sequence before practice"

If you cannot write such a single sentence without becoming vague, the key is too broad and should be split.

⸻

\#\#\# Historical Integration Rules

1. When to reuse an existing progress\_key
Given a new occurrence in the current batch and an existing progress\_key from history, reuse that key (and its progress\_id) only if:
	1.	Skill/goal alignment
	    •	It is clearly the same skill / goal / task (e.g., same dance routine, same type of homework, same cooking procedure).
	2.	Context alignment
	    •	Similar physical or situational context (same room / location type / device, same "before dinner" study block, etc.).
	3.	Role alignment
        •	The occurrence plays a compatible role:
        •	practice vs full execution vs review,
        •	similar place in the workflow (full run, partial drill, cool-down review, etc.).

If these align:
	•	Reuse the same progress\_id and progress\_key.
	•	Add a new occurrence under it with updated historical\_context, metrics, and outcome\_quality.

2. When to create a NEW progress\_key
Create a new progress\_id / progress\_key when:
	•	The skill/goal is fundamentally different.
	•	The context is clearly different (e.g., completely different activity).
	•	Mixing them would make the key too broad or confusing.

⸻

\#\#\# Objective

For the current batch of segments, with optional historical progress memory, you must:

1. Update progress state (progress\_state\_updates)

   - Scan all segments and interaction\_records to find every time window that reflects:
     - practice or execution for a specific skill/goal, and/or
     - visible changes in fluency, completeness, or quality.
   - When defining or updating any progress\_key / progress\_id, you MUST strictly follow the rules in:
     - "Progress Key Granularity Rules" (to decide how fine-grained each progress\_key should be), and
     - "Historical Integration Rules" (to decide when to reuse an existing progress\_id vs. when to create a new one).
   - Integrate with `progress\_events` from history by:
     - reusing `progress\_key` and `progress\_id` when allowed by those rules, or
     - creating a new `progress\_id` / `progress\_key` when the rules say a new thread is needed.
   - For each `progress\_id`, append new occurrences capturing:
     - `segment\_id`, `day\_id`, `time\_window`, `supporting\_source`,
     - `observation`, `local\_context`,
     - `metrics` (approximate is fine),
     - `historical\_context`,
     - `effort\_type`, `outcome\_quality`,
     - `workflow\_position`, `social\_dynamics`,
     - `occurrence\_confidence`.

2. Decide current-batch feedback triggers (feedback\_triggers) and generate dialogues

   - For each `progress\_key`, use its historical + current occurrences to determine whether this batch contains a moment where:
     - there is enough longitudinal evidence (cross-day or cross-session) to justify feedback, and
     - the current occurrence sits at a natural reflection point (end of a run/session, or clear improvement/struggle).
   - When deciding whether to activate a feedback trigger, and how to phrase the feedback, you MUST strictly follow:
     - "Activation Logic for Feedback Triggers" (to decide *whether* to trigger and at *which* occurrence), and
     - "Dialogue Generation Objective (per activated trigger)" (to structure and style the multi-turn dialogue).
   - For each qualifying occurrence, activate one feedback trigger and generate a short multi-turn dialogue, grounded in the linked progress history.

⸻

\#\#\# Activation Logic for Feedback Triggers

A. Cross-session requirement (longitudinal comparison)
Before any activation:
	1.	For each progress\_key, collect all its occurrences (historical + current batch).
	2.	Parse day\_id from the DAY\# prefix of each time\_window.
	3.	Determine whether there are at least two distinct sessions, defined as:
      •	Occurrences on different days, or
      •	Occurrences on the same day but clearly separated (timestamps differ by ≥ 2 hours or obviously "morning vs evening" etc.).

A progress\_key is eligible for proactive feedback only if:
	•	It has occurrences in ≥ 2 sessions as defined above.

If it appears only within one short session:
	•	You may still record it in progress\_state\_updates,
	•	But do NOT create any feedback\_triggers for it in this batch.

B. Per-session uniqueness ("once per progress\_key per session")
For each eligible progress\_key:
	•	For every distinct session (DAY\# or separated block) in the current batch, do:
        1.	Collect all occurrences of this progress\_key in that session.
        2.	Sort them by the start time of their time\_window ascending.
        3.	Choose exactly one occurrence as the candidate feedback point using this rule:
          •	Prefer an occurrence with workflow\_position = "end" (end of a practice run / session).
          •	If none, prefer the latest occurrence in that session.
        4.	That occurrence is the per-session candidate; others in that session are not activated.

C. Per-occurrence activation criteria
Mark a candidate occurrence as activated (i.e., create a feedback\_triggers item) only if:
	1.	There exists at least one earlier session of the same progress\_key to compare with (baseline / prior attempts).
	2.	The current occurrence is the per-session unique candidate under rule B.
	3.	local\_context, observation, metrics, or outcome\_quality give some evidence of:
        •	improvement (faster, smoother, more complete, more standard), or
        •	meaningful persistence (continuing efforts on the same challenging task), or
        •	a clear completion milestone (e.g., finishing a sequence that was previously partial).
	4.	A helpful feedback message can:
        •	summarize progress so far, and/or
        •	give constructive micro-feedback or next-step suggestions
    that would make sense to the user.

If the episode is:
	•	purely a failure with no visible learning, or
	•	too ambiguous to judge, or
	•	mainly about safety / configuration / generic routine rather than progress,

then activated = false (no feedback dialogue), even though the occurrence is still recorded for progress tracking.

D. Intra-day cooldown for the same progress\_key
For each progress\_key on the same DAY\#:
	•	If a feedback\_trigger has already been activated at time T for this progress\_key,
	•	 then you MUST NOT activate another feedback\_trigger for the same progress\_key within the next 2 hours on that day. 
	•	Any candidate occurrence whose time\_window starts \textless{} 2 hours after the last activated trigger on that DAY\# must be skipped (activated = false), even if it satisfies A-C.

*The "historical\_feedback\_triggers" field in the Historical Progress Summary JSON is used as evidence for determining whether a progress event of the same type should be activated for the current batch. (the gap between triggers \textgreater{}= 2 hours each type)*

⸻

\#\#\# Timestamp Rules for Feedback Triggers (strict)

For every item in feedback\_triggers:
	•	current\_time\_window MUST be copied exactly from:
    •	i\_do\_steps[].time\_window or
    •	speakers\_say[].time\_window.
You MUST NOT use interactions\_with\_objects or interactions\_with\_people as the source of current\_time\_window, even if they provide context.
If multiple i\_do\_steps / speakers\_say entries are involved in the same progress episode, choose the earliest time\_window where the current practice/execution begins (e.g., starting the run, starting the explained reflection).

The assistant's first proactive utterance is interpreted as happening immediately after this current\_time\_window.

⸻

\#\#\# Dialogue Generation Objective (per activated trigger)

For each activated occurrence in feedback\_triggers:
	1.	Grounding
        •	Use progress\_key, progress\_summary, and this occurrence's:
        •	current\_observation, current\_local\_context,
        •	historical\_context, metrics, outcome\_quality,
        •	plus earlier sessions for comparison.

  2.	Feedback content
    You MUST go beyond describing what the user just did. Each proactive message must contain all three layers:
        •	Progress evaluation - briefly state what has changed or remained stable across sessions
        e.g., smoother / more fluent / more complete / more consistent, or "still struggling but making steady attempts".
        •	Emotional support - acknowledge the user's effort, difficulty, or persistence in a supportive way
        e.g., recognizing that they kept practicing, normalizing that improvement takes time.
        •	Concrete next-step suggestion - give 1-2 small, realistic suggestions for future attempts
        e.g., focusing on o ne sub-step next time, slowing down a tricky part, scheduling a short practice slot.

    It is not allowed to only paraphrase the user's actions without (1) progress evaluation, (2) emotional value, and (3) at least one actionable suggestion.

	3.	Tone
        •	Supportive, encouraging, realistic.
        •	Do not sound like grading or harsh evaluation.
        •	Do NOT mention videos, annotations, or models.
        •   Avoid replies that only repeat what the user just did; always add your own evaluation and forward-looking guidance.
	
 4.	  Dialogue structure
	  •	At least 2-3 turns:
        1.	Assistant (Turn 1)
        •	Proactive feedback + brief suggestion, grounded in longitudinal comparison.
        2.	User (Turn 2)
        •	Natural reply (≥ 12 English words).
        •	May accept, adjust, or downplay the feedback.
        3.	Assistant (optional Turn 3)
        •	Acknowledge the user's stance and refine or tone down the suggestion.
        4.	User (optional Turn 4)
        •	Short acknowledgement or final decision.
  
  5.	Diversity
    •	Vary phrasing: sometimes emphasize "you've been practicing this several times now…", sometimes "compared to earlier sessions, this looked more stable…", etc.
    •	Not every user must enthusiastically accept the feedback; some may say "I'm tired today, maybe later", etc.

⸻

\#\#\# Output Format (single JSON with two sections)

Your output MUST be ONE JSON object:
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Personal Progress Feedback Proactive Service",

  "progress\_state\_updates": [
    \{
      "progress\_id": "pprog\_001",
      "progress\_key": "\textless{}one skill/goal/performance pattern\textgreater{}",
      "progress\_type": "skill\_learning \textbar{} personal\_goal \textbar{} performance \textbar{} habitual\_task",
      "progress\_summary": "\textless{}how this pattern looks so far including this batch\textgreater{}",
      "batch\_consistency\_level": "high \textbar{} medium \textbar{} low",
      "batch\_confidence": 0.0,

      "occurrences": [
        \{
          "segment\_id": "\textless{}source segment id\textgreater{}",
          "day\_id": 2,
          "time\_window": "DAY2 HH:MM:SS-HH:MM:SS",
          "supporting\_source": "i\_do\_steps \textbar{} interactions\_with\_objects \textbar{} interactions\_with\_people \textbar{} speakers\_say",

          "observation": "\textless{}specific evidence of practice/execution in this batch\textgreater{}",
          "local\_context": "\textless{}what the user is doing / environment\textgreater{}",
          "metrics": \{
            "practice\_minutes": 10.0,
            "attempt\_count": 2,
            "quality\_trend": "struggling \textbar{} partial\_success \textbar{} clear\_success \textbar{} unclear"
          \},
          "historical\_context": "\textless{}how this relates to earlier occurrences under this progress\_id\textgreater{}",
          "effort\_type": "practice \textbar{} execution \textbar{} review \textbar{} planning",
          "outcome\_quality": "improved \textbar{} similar \textbar{} worse \textbar{} unclear",
          "workflow\_position": "start \textbar{} middle \textbar{} end \textbar{} standalone",
          "social\_dynamics": "self-initiated \textbar{} reacting\_to\_others \textbar{} jointly\_decided",
          "occurrence\_confidence": 0.0
        \}
      ]
    \}
  ],

  "feedback\_triggers": [
    \{
      "trigger\_id": "pfeed\_001",
      "progress\_id": "pprog\_001",
      "progress\_key": "\textless{}copied from progress\_state\_updates\textgreater{}",
      "trigger\_type": "cross\_session\_progress \textbar{} sustained\_effort \textbar{} milestone\_completion",

      "current\_segment\_id": "\textless{}segment id where feedback is triggered\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "supporting\_source": "i\_do\_steps \textbar{} speakers\_say",

      "current\_observation": "\textless{}what just happened that makes this a good feedback moment\textgreater{}",
      "current\_local\_context": "\textless{}short description of current scene\textgreater{}",
      "comparison\_basis": "\textless{}how this compares to earlier runs / sessions\textgreater{}",
      "trigger\_reason": "\textless{}why feedback is considered helpful now\textgreater{}",
      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}assistant proactive feedback, referencing cross-session progress\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}likely user reply (\textgreater{}= 12 words)\textgreater{}"
        \}
        // optionally 1-2 more turns, alternating assistant ↔ user
      ]
    \}
  ]
\}

Notes:
	•	progress\_state\_updates only needs to include new or updated progress patterns from this batch (not all history).
	•	For the very first batch with no history:
    •	progress\_summary: "initial hypothesis of a progress-related pattern in this batch."
    •	historical\_context in each occurrence: "no prior records; first detected in this batch."
  •	*Do not repeatedly activate the same event or generate identical dialogue content.*

⸻

Failure Case Format

If you find no progress-related occurrences in this batch, or no occurrence meets the activation rules for feedback:
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Personal Progress Feedback Proactive Service",
  "progress\_state\_updates": [],
  "feedback\_triggers": [],
  "note": "No personal-progress patterns or feedback-worthy cross-session moments were detected in this batch, given the current annotations and historical summary."
\}
\end{promptbox}

\begin{promptbox}[EgoLife — Long-Term · Routine Optimization]
\#\#\# Task Context

You are analyzing MULTIPLE egocentric annotation files (each less than 10 minutes) from the EgoLife dataset for one contiguous batch of time (less than 2.5 hours).

Your job in this stage is signal mining for a special Long-Term Proactive Service subtype:

	•	service\_main\_type: "Long-Term Proactive Service"
	•	service\_sub\_type: "Routine Optimization Proactive Service"

You handle both:
	1.	Multi-step routines (time-structured or task-structured):
		•	e.g., afternoon cleaning routine, pre-meeting preparation, after-dinner cleanup, post-recording wrap-up.
	2.	Configuration-only patterns (repeated "usual setup"):
		•	e.g., typical AC temperature before sleep, usual lamp brightness, preferred phone mode in meetings, typical work-desk layout.
	3.	Expected-but-missing routines within a usual time window:
		•	e.g., the user cleaned the room around 3-4 PM on several days, but today at similar time they have not done it yet.

as long as they are recurring across sessions/days and suitable for long-term optimization (defaults, shortcuts, bundled flows, or timely reminders).

⸻

\#\#\# Core Pattern Types

Within this batch, you focus on two complementary dimensions:
	1.	Pattern State (routine\_state\_updates)
	Concrete episodes that show the user:
		•	Running through a similar multi-step routine in a recognizable context, and/or
		•	Applying a stable configuration in a recurring situation.
	Examples:
		•	Afternoon cleaning routine with similar sequence of steps.
		•	Pre-meeting prep in a similar order (open slides → check link → test mic).
		•	Before sleep, setting AC, lights, and phone in a similar combination.
		•	Before online calls, always putting phone on vibrate and adjusting laptop volume.
	2.	Optimization Triggers (optimization\_triggers + dialogues)
	Specific episodes in the current batch where, given previous occurrences of the same pattern, it is valuable for the assistant to:
		•	Bundle or streamline multiple repeated steps (routine-level optimization), or
		•	Save / reuse a configuration as a default / shortcut, or
		•	Prepare tools/environment/settings in advance for future runs, or
		•	Gently remind the user about a usually stable routine that has not yet occurred in its typical time window, and offer to:
			•	run through a quick checklist,
			•	reschedule or skip intentionally,
			•	or set a different reminder rule.

These Type B moments must be grounded in longitudinal evidence:
	•	Cross-day (DAY1 → DAY2/3/…), or
	•	Same-day but clearly separate sessions (≥ 2 hours apart or obviously distinct blocks, like "morning prep" vs "evening prep").

You must NOT guess new events, invent timestamps, or hallucinate behaviors not supported by the annotations.

⸻

\#\#\# Authoritative Timestamps \& Fine-Grained Evidence Priority

Every fine-grained annotation entry has a time\_window aligned to the original video, for example:
	•	i\_do\_steps[].time\_window
	•	interactions\_with\_objects[].time\_window
	•	interactions\_with\_people[].time\_window
	•	speakers\_say[].time\_window

All time\_window strings already have the format:

DAY\# HH:MM:SS-HH:MM:SS

You MUST only copy these existing time\_window values.
Do NOT interpolate, merge, extend, shrink, or invent new time ranges.

Fine-Grained priority for pattern occurrences
When detecting candidate occurrences (for routine\_state\_updates):
•	Primary sources:
	•	i\_do\_steps
	•	interactions\_with\_objects
	•	interactions\_with\_people
	•	speakers\_say

Treat each fine-grained entry (or a small, coherent cluster in the same context) as a potential routine or configuration episode if it clearly involves:
	•	A recognizable recurring sequence of steps, and/or
	•	A repeated configuration being applied in a familiar situation.

Timestamp rules for occurrences:
	•	For every occurrence in routine\_state\_updates, you must copy one existing time\_window directly from:
	•	i\_do\_steps, or
	•	speakers\_say.
	•	You must never use interaction\_record.time\_window for occurrences.
	•	You must never merge, split, or invent time\_window ranges.

Additional strict rule for dialogue triggers
For optimization\_triggers.current\_time\_window, you may only copy time\_window from:
	•	i\_do\_steps[].time\_window or
	•	speakers\_say[].time\_window.

You MUST NOT use time windows from interactions\_with\_objects or interactions\_with\_people as the source for current\_time\_window, even if they describe related context.

For missed routine reminders, you still must anchor current\_time\_window to some actual i\_do\_steps or speakers\_say entry in the current batch that occurs in the relevant time-of-day window, representing the moment when the assistant decides to proactively check in (e.g., when the user is doing something else during the usual cleaning time).

⸻

\#\#\# Input Human Annotations

1. Current batch: segment-level episodic annotations
\{
  "segment\_id": "\textless{}identifier for this \textasciitilde{}10-minute segment\textgreater{}",
  "description": "... high-level summary of what I do in this segment ...",
  "interaction\_records": [
    \{
      "time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "description": "... micro-episode summary ...",

      "i\_do\_steps": [ ... ],
      "speakers\_say": [ ... ],
      "interactions\_with\_objects": [ ... ],
      "interactions\_with\_people": [ ... ],
      "environment\_state": [ ... ],
      "task\_transition": [ ... ],
      "confidence": 0.0-1.0
    \}
  ]
\}

These interaction\_records and their subfields are your primary evidence.

The coverage of this batch is defined by the minimum and maximum timestamps appearing in these JSONs.

2. Historical routine summary JSON (optional memory)
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Routine Optimization Proactive Service",
  "routine\_events": [
    \{
      "routine\_id": "rtopt\_001",
      "routine\_key": "\textless{}abstract description of one pattern\textgreater{}",
      "routine\_type": "configuration\_preference \textbar{} time\_structured\_routine \textbar{} task\_structured\_routine",
      "routine\_summary": "\textless{}how this pattern has unfolded over previous hours/days\textgreater{}",
      "batch\_consistency\_level": "high \textbar{} medium \textbar{} low",
      "batch\_confidence": 0.0,

      "occurrences": [
        \{
          "segment\_id": "\textless{}old segment id\textgreater{}",
          "day\_id": 1,
          "time\_window": "DAY1 HH:MM:SS-HH:MM:SS",
          "supporting\_source": "i\_do\_steps \textbar{} speakers\_say",

          "observation": "\textless{}what happened\textgreater{}",
          "local\_context": "\textless{}local scene / surroundings\textgreater{}",
          "historical\_context": "\textless{}how it related to earlier ones\textgreater{}",
          "inferred\_motivation": "\textless{}behavior-grounded explanation\textgreater{}",
          "workflow\_position": "start \textbar{} middle \textbar{} end \textbar{} standalone",
          "social\_dynamics": "self-initiated \textbar{} reacting\_to\_others \textbar{} jointly\_decided",
          "implicit\_avoidance": "\textless{}optional\textgreater{}",
          "routine\_evolution": "\textless{}optional\textgreater{}",
          "occurrence\_confidence": 0.0
        \}
      ]
    \}
  ],
  "historical\_optimization\_triggers": [
    \{
      "trigger\_id": "ropt\_001",
      "routine\_id": "rtopt\_001",
      "routine\_key": "\textless{}copied from routine\_state\_updates\textgreater{}",
      "routine\_type": "configuration\_preference \textbar{} time\_structured\_routine \textbar{} task\_structured\_routine",
      "trigger\_type": "routine\_block\_optimization \textbar{} configuration\_default\_suggestion \textbar{} missed\_routine\_reminder",

      "current\_segment\_id": "\textless{}segment id where optimization/reminder is triggered\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "supporting\_source": "i\_do\_steps \textbar{} speakers\_say",

      "current\_observation": "\textless{}what just happened that makes this a good optimization or reminder moment\textgreater{}",
      "current\_local\_context": "\textless{}short description of current scene\textgreater{}",
      "activation\_type": "cross\_day\_pattern \textbar{} expected\_pattern\_missing",
      "comparison\_basis": "\textless{}how this day's pattern compares to earlier days / sessions\textgreater{}",
      "activation\_reason": "\textless{}why optimization or reminder is considered helpful now\textgreater{}",
      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}assistant proactive pattern-level optimization or gentle reminder suggestion\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}likely user reply (\textgreater{}= 12 words)\textgreater{}"
        \}
        // optionally 1-2 more turns, alternating assistant ↔ user
      ]
    \}
  ]
\}

⸻

\#\#\# *What counts as a Routine Optimization signal?*

You care about recurring convenience patterns, not one-off tasks.

Positive signals (examples):
	1.	Multi-step routines (time\_structured\_routine / task\_structured\_routine)
		•	Similar sequence of steps in similar context:
		•	Afternoon cleaning: tidy room → collect trash → wipe surfaces → put tools back.
		•	Pre-meeting: open slides → check link → test mic → adjust seating.
		•	After cooking: clear table → rinse dishes → load dishwasher → wipe counters.
	2.	Configuration preferences (configuration\_preference)
		•	Repeatedly setting the same or very similar configuration in a recurring context:
		•	Before sleep: AC around 26°C + bedside lamp dim + phone to silent.
		•	During meetings: phone on vibrate + laptop volume low.
	3.	Expected-but-missing routines (reminder candidates)
		•	From historical data, a routine\_key appears on multiple days in a similar time-of-day window (e.g., 15:00-16:00 cleaning).
		•	In the current batch, time has progressed into or beyond this typical window, but:
		•	No occurrence of this routine\_key has been observed so far today, and
		•	The user is engaged in other activities (with i\_do\_steps / speakers\_say entries) that indicate the routine may have been forgotten or postponed.

In such cases, a soft reminder is a valid Routine Optimization trigger, because it helps maintain or intentionally reschedule a stable routine.

You should NOT treat as Routine Optimization:
	•	Pure safety behavior (→ Safety Proactive Service).
	•	Pure "getting better at a skill" without a configuration/routine optimization angle (→ Personal Progress Feedback).
	•	One-off or rare tasks with no sign of recurrence.

Simple test:
	•	If the main value is "this pattern happens again and again, and could be streamlined / auto-configured / gently remembered when missing" → candidate for Routine Optimization.
	•	If the main value is "I'm getting better at this skill" → likely belongs to Personal Progress.

⸻

\#\#\# Routine Key Granularity Rules

Each routine\_key should capture one pattern that you can describe with:
	•	For configuration\_preference:
"When I am in [this situation/time], I tend to set/use [object] with [this configuration/mode/place]."
	•	For time\_structured\_routine / task\_structured\_routine:
"When I am in [this time/situation], I tend to do [step A → step B → step C] as one routine block."

Bad examples (too broad / vague):
	•	"General productivity routine"
	•	"Daily cleaning"
	•	"Charging everything"

Good examples:
	•	"Before sleep: set bedroom AC to \textasciitilde{}26°C and dim bedside lamp to low warm light."
	•	"Before group meetings: open slides, check online link, and test microphone."
	•	"After cooking dinner: wipe counters, wash dishes, and take trash out."
	•	"During meetings: keep phone on vibrate and laptop volume low."

If you cannot write such a sentence without being vague, the key is too broad and should be split.

⸻

\#\#\# Historical Integration Rules

1. When to reuse an existing routine\_key
Given a new occurrence in the current batch and an existing routine\_key:

Reuse that key (and its routine\_id) only if:
	1.	Type alignment
		•	Same routine\_type (configuration\_preference vs time\_structured\_routine vs task\_structured\_routine).
	2.	Context alignment
		•	Similar time/situation trigger (e.g., "before sleep", "before meetings", "after cooking").
	3.	Configuration / task-cluster alignment
		•	For configuration\_preference: similar object/setting and value/mode/place.
		•	For routines: similar set of tasks in similar order/structure.
	4.	Role alignment
		•	Plays the same role (prep / wrap-up / typical configuration).

If these align:
	•	Reuse the same routine\_id and routine\_key.
	•	Append a new occurrence with updated historical\_context and routine\_evolution.

2. When to create a NEW routine\_key
Create a new routine\_id / routine\_key when:
	•	The trigger/context is fundamentally different.
	•	The core object/setting is different (for configuration preferences).
	•	The task cluster is different (for routines).
	•	Mixing them would make the key too broad, ambiguous, or internally inconsistent.

⸻

\#\#\# Objective

For the current batch, with optional historical routine memory, you must:
	1.	Update pattern state (routine\_state\_updates)
		1.	Scan all segments and all interaction\_records to find every time\_window that reflects a possible:
			•	configuration-level preference, and/or
			•	time-structured routine, and/or
			•	task-structured routine,
		applying:
			•	Fine-Grained Evidence Priority, and
			•	Routine Key Granularity Rules.
		Prefer high recall; uncertain cases can be kept with lower occurrence\_confidence.
		2.	Compare with routine\_events in the Historical Routine Summary JSON (if provided):
			•	Each routine\_key is one pattern (configuration or routine).
			•	The occurrences are concrete events.
			•	When scanning the current batch, if you detect a new event that matches an existing pattern (according to type + trigger/context + configuration/task cluster + role), you must:
			•	reuse that routine\_key and its event\_id in your output, and
			•	only add new occurrences from the current batch.
			•	If you detect a new pattern type not covered by any existing routine\_key, you must:
				•	create a new candidate\_events entry with:
				•	a new routine\_key, and
				•	a newly assigned event\_id that continues the numbering.
			•	For this new pattern, occurrences should contain only events from the current batch, and historical\_context / routine\_evolution should clearly state that this is a newly proposed pattern.
		3.	For each occurrence, record:
			•	observation, time\_window, segment\_id, supporting\_source
			•	Contextual fields:
			•	local\_context, historical\_context, workflow\_position, social\_dynamics, routine\_evolution, implicit\_avoidance (optional), occurrence\_confidence.
		4.	For each routine\_key, summarize:
			•	how this batch extends or refines the pattern (routine\_summary, routine\_evolution), and
			•	overall batch\_consistency\_level and batch\_confidence for this batch, taking historical memory into account when applicable.

	2.	Decide current-batch optimization triggers (optimization\_triggers) and generate dialogues
		•	For each routine\_key, use historical + current occurrences to determine whether this batch contains a moment where:
		•	There is enough longitudinal evidence (cross-day / cross-session) to justify optimization or reminder.
		•	The current occurrence is at a natural decision point:
			•	Pattern is being executed now, or
			•	Pattern is conspicuously missing/late in its usual time window, and the user is doing something else.
		•	For each such situation, activate one optimization trigger and generate a short multi-turn dialogue.

⸻

\#\#\# Activation Logic for Optimization Triggers

A. Cross-day requirement (for stable pattern detection)
Before any activation:
	1.	For each routine\_key, collect all its occurrences (historical + current batch).
	2.	Parse day\_id from the DAY\# prefix of each time\_window.
	3.	Determine whether there are at least two distinct days where this routine\_key appears.

A routine\_key is eligible for proactive optimization only if:
	•	It appears on ≥ 2 different days (e.g., DAY1 and DAY2).

If it appears only on a single day:
	•	You may still record it in routine\_state\_updates,
	•	But DO NOT create any optimization\_triggers for it in this batch.

⸻

B. Per-session uniqueness when pattern is present ("at most once per 2 hours per routine\_key")
For present pattern optimization triggers (i.e.,
	•	multi-step-routines,
	•	configuration-only patterns),

we allow multiple activations on the same day, but enforce a 2-hour cooldown for each routine\_key.

For each eligible routine\_key, and for each day where it appears in the current batch:
	1.	Collect all occurrences of this routine\_key on that day.
	2.	Sort them by the start time of their time\_window ascending.
	3.	Partition them into session blocks on that day, where:
		•	Two consecutive occurrences belong to the same session block if the time gap between their start times is \textless{} 2 hours.
		•	If the gap is ≥ 2 hours, start a new session block.
	4.	For each session block, choose exactly one occurrence as the candidate optimization point, using this rule:
		1.	If any occurrence has workflow\_position = "start", choose the earliest such occurrence in this block.
		2.	Else, if any occurrence has workflow\_position = "end", choose the earliest such occurrence in this block.
		3.	Else, choose the earliest occurrence in this block.
	5.	That occurrence is the per-session candidate for this routine\_key; other occurrences in the same 2-hour block are not activated.

This means:
	•	For multi-step-routines and configuration-only patterns,
	•	The same routine\_key can be activated at most once every 2 hours on a given day.

⸻

C. Expected-but-missing routines (reminder candidates, strictly once per day)
For expected-but-missing routine reminders (missed\_routine\_reminder), we keep a once-per-day rule.

For each eligible routine\_key, you must also check whether:
	1.	There are occurrences on ≥ 2 earlier days in similar time-of-day windows
(e.g., multiple days with occurrences between 15:00-16:00).
	2.	On the current day (DAY\#) covered by this batch:
		•	Time (based on i\_do\_steps / speakers\_say time\_windows) has advanced into or clearly beyond the typical window, and
		•	No occurrence of this routine\_key has been detected so far on this day.

	In this case, you may create a missed routine reminder trigger, with:
		•	trigger\_type = "missed\_routine\_reminder"
		•	activation\_type = "expected\_pattern\_missing"

	You must still choose a current\_time\_window from:
		•	The earliest i\_do\_steps[].time\_window or speakers\_say[].time\_window that:
		•	Occurs after the typical start of the usual routine window on this day, and
		•	Represents a reasonable moment for a gentle check-in (the user is engaged in something else and the routine has likely been forgotten or delayed).

	Additional constraint for C-type triggers:
		•	For each routine\_key, you may activate at most one missed\_routine\_reminder per day,
	regardless of how long the batch covers that day.

If such a moment cannot be clearly identified (e.g., the batch does not extend far enough into the usual time window), you should not trigger a reminder.

⸻

D. Per-occurrence activation criteria
For any candidate optimization/reminder point (present pattern or expected-but-missing):

Mark it as activated (i.e., create an optimization\_triggers item) only if:
	1.	There exists at least one earlier day of the same routine\_key to compare with.
	2.	It fits one of the following:
		•	Present pattern optimization (multi-step-routines / configuration-only):
			•	The current occurrence is the unique per-session candidate for its 2-hour block under rule B, and
			•	No other optimization trigger for the same routine\_key has been activated in the preceding 2 hours of clock time on that day, and
			•	local\_context, observation, and routine\_type show a clear routine or configuration being executed now, and
			•	A meaningful optimization (bundling steps, saving defaults, pre-setup, reordering) can help future runs.
		•	Expected-but-missing reminder (missed\_routine\_reminder):
			•	Conditions in rule C hold
			•	stable pattern in similar time windows on earlier days, missing so far today, and a reasonable anchor activity exists), and
			•	No other missed\_routine\_reminder for the same routine\_key has been activated yet on this day, and
			•	A gentle reminder or rescheduling suggestion would be helpful and not intrusive.
	3.	The situation is not primarily about safety or another proactive service type.

*The "historical\_optimization\_triggers" field in the Historical Routine Summary JSON is used to provide decision-making evidence for determining the Optimization Triggers in the current batch. (the gap between triggers \textgreater{}= 2 hours each type)*

⸻

\#\#\#\# Timestamp Rules for Optimization Triggers (strict)

For every item in optimization\_triggers:
	•	current\_time\_window MUST be copied exactly from:
	•	i\_do\_steps[].time\_window or
	•	speakers\_say[].time\_window.

Even for missed routine reminders, you must anchor to a real i\_do\_steps or speakers\_say entry in the current batch (the activity during which the assistant decides to check in).

The assistant's first proactive utterance is interpreted as happening immediately after this current\_time\_window.

⸻

\#\#\# Dialogue Generation Objective (per activated trigger)

For each activated occurrence in optimization\_triggers:
	1.	Grounding
	Use:
		•	routine\_key, routine\_summary, and this trigger's:
		•	current\_observation, current\_local\_context,
		•	historical\_context, inferred\_motivation,
		•	workflow\_position, routine\_evolution,
		•	comparison\_basis, activation\_type, trigger\_type,
		•	plus earlier days' occurrences as evidence.

	2.	Optimization / Reminder content

	Regardless of trigger type, the proactive message must:
		1.	Recognize the pattern
			•	For present routines: acknowledge the recurring routine or configuration.
			•	For missed routines: gently note that the user usually handles X around this time without sounding like strict monitoring.
		2.	Provide convenience framing \& emotional support
			•	Emphasize reduced friction, mental load, or remembering burden.
			•	For missed routines, validate that it's okay to change plans, and position the assistant as helpful, not scolding.
		3.	Offer concrete, realistic options
			•	For present routines:
			•	Bundle steps into a reminder/shortcut/checklist,
			•	Save / reuse as default configuration,
			•	Suggest pre-setup for tools / environment next time.
			•	For missed routines:
			•	Ask if the user wants to:
			•	still do it now with a quick checklist,
			•	move it to later today,
			•	skip it this time, or
			•	adjust the future reminder rule (e.g., weekdays only).

	Avoid replies that only paraphrase what the user did or usually does; always add:
		•	Pattern-level framing, and
		•	Future-facing, actionable optimization or reminder options.

	3.	Tone
		•	Practical, supportive, and non-judgmental.
		•	Especially for missed routines: avoid guilt; offer choices.
		•	Do NOT mention videos, annotations, or models.
		•	Do NOT talk explicitly about "cross-day analysis" or internal logs.

	4.	Dialogue structure

	For each optimization\_triggers item:
		•	At least 2-3 turns:
		1.	Assistant (Turn 1)
			•	Proactive optimization / reminder suggestion, grounded in cross-day pattern.
		2.	User (Turn 2)
			•	Natural reply (≥ 12 English words).
			•	May accept, partially accept, postpone, decline, or adjust rules.
		3.	Assistant (optional Turn 3)
			•	Acknowledge the user's choice and either:
			•	confirm the new shortcut / checklist / default, or
			•	confirm the rescheduling / skipping rule, or
			•	back off politely.
		4.	User (optional Turn 4)
			•	Short acknowledgement or final confirmation.

	5.	Diversity
	Across all dialogues in one output:
		•	Vary phrasing:
		•	"you usually follow this routine…"
		•	"you often handle this situation in a similar way…"
		•	"you tend to set things up like this when…"
		•	Vary structure:
		•	Sometimes start from the pattern ("Since you often…")
		•	Sometimes from the offer ("If you'd like, I can…").
		•	Not every suggestion must be accepted; some users may say "not today", "only on weekdays", etc. Adapt accordingly.

⸻

\#\#\# Output Format (single JSON with two sections)

Your output MUST be ONE JSON object:
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Routine Optimization Proactive Service",

  "routine\_state\_updates": [
    \{
      "routine\_id": "rtopt\_001",
      "routine\_key": "\textless{}one routine/configuration pattern\textgreater{}",
      "routine\_type": "configuration\_preference \textbar{} time\_structured\_routine \textbar{} task\_structured\_routine",
      "routine\_summary": "\textless{}how this pattern looks so far including this batch\textgreater{}",
      "batch\_consistency\_level": "high \textbar{} medium \textbar{} low",
      "batch\_confidence": 0.0,

      "occurrences": [
        \{
          "segment\_id": "\textless{}source segment id\textgreater{}",
          "day\_id": 2,
          "time\_window": "DAY2 HH:MM:SS-HH:MM:SS",
          "supporting\_source": "i\_do\_steps \textbar{} interactions\_with\_objects \textbar{} interactions\_with\_people \textbar{} speakers\_say \textbar{} interaction\_record",

          "observation": "\textless{}specific evidence of this pattern in this batch\textgreater{}",
          "local\_context": "\textless{}what the user is doing / environment\textgreater{}",
          "historical\_context": "\textless{}how this relates to earlier occurrences under this routine\_id\textgreater{}",
          "inferred\_motivation": "\textless{}behavior-grounded guess\textgreater{}",
          "workflow\_position": "start \textbar{} middle \textbar{} end \textbar{} standalone",
          "social\_dynamics": "self-initiated \textbar{} reacting\_to\_others \textbar{} jointly\_decided",
          "implicit\_avoidance": "\textless{}optional\textgreater{}",
          "routine\_evolution": "\textless{}optional\textgreater{}",
          "occurrence\_confidence": 0.0
        \}
      ]
    \}
  ],

  "optimization\_triggers": [
    \{
      "trigger\_id": "ropt\_001",
      "routine\_id": "rtopt\_001",
      "routine\_key": "\textless{}copied from routine\_state\_updates\textgreater{}",
      "routine\_type": "configuration\_preference \textbar{} time\_structured\_routine \textbar{} task\_structured\_routine",
      "trigger\_type": "routine\_block\_optimization \textbar{} configuration\_default\_suggestion \textbar{} missed\_routine\_reminder",

      "current\_segment\_id": "\textless{}segment id where optimization/reminder is triggered\textgreater{}",
      "current\_time\_window": "DAY\# HH:MM:SS-HH:MM:SS",
      "supporting\_source": "i\_do\_steps \textbar{} speakers\_say",

      "current\_observation": "\textless{}what just happened that makes this a good optimization or reminder moment\textgreater{}",
      "current\_local\_context": "\textless{}short description of current scene\textgreater{}",
      "activation\_type": "cross\_day\_pattern \textbar{} expected\_pattern\_missing",
      "comparison\_basis": "\textless{}how this day's pattern compares to earlier days / sessions\textgreater{}",
      "activation\_reason": "\textless{}why optimization or reminder is considered helpful now\textgreater{}",
      "occurrence\_confidence": 0.0,

      "proactive\_dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}assistant proactive pattern-level optimization or gentle reminder suggestion\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}likely user reply (\textgreater{}= 12 words)\textgreater{}"
        \}
        // optionally 1-2 more turns, alternating assistant ↔ user
      ]
    \}
  ]
\}

Notes:
	•	routine\_state\_updates only needs to include new or updated patterns from this batch (not the whole historical store).
	•	For the very first batch with no history:
		•	routine\_summary: "initial hypothesis of a routine/configuration pattern in this batch."
		•	historical\_context in each occurrence: "no prior records; first detected in this batch."
	•	*Do not repeatedly activate the same event or generate identical dialogue content.*

\#\#\#\# Failure Case Format
\{
  "service\_main\_type": "Long-Term Proactive Service",
  "service\_sub\_type": "Routine Optimization Proactive Service",
  "routine\_state\_updates": [],
  "optimization\_triggers": [],
  "note": "No stable routine/configuration patterns or optimization-worthy cross-day moments were detected in this batch, given the current annotations and historical summary."
\}
\end{promptbox}

% \subsection{HoloAssist Annotation Prompts}
% \label{sec:supp_holoassist_annotation}

% The HoloAssist subset covers hands-on procedural tasks (assembly, repair, lab work) in short single-task episodes. Only Instant and Short-Term service categories apply (5 out of 11 sub-types). Each prompt is sent to Gemini along with manual annotations for a single video clip. The model extracts service events matching the target category and generates 2--4 turn dialogues.

% \begin{promptbox}[HoloAssist — User Prompt Template (Input Format)]
% \#\#\# Manual Annotations of Clip ID \{clip\_id\}
% \{annotation\_data\}
% \end{promptbox}

\begin{promptbox}[HoloAssist — Instant · Safety]
\#\#\# Role

You are an Instant Proactive Service (Instant PS) annotation and dialogue-generation assistant for the HoloAssist dataset.
In laboratory, hands-on operation, or mobility scenarios, you analyze manual annotations to extract time-windows of "Safety" risks / immediate physical hazards, and for each extracted event, you generate a 2-4 turn "assistant ↔ user" dialogue.

You must rely only on the time-windows provided by the manual annotations.
You must NOT extend, shorten, merge, or fabricate any time segments that do not exist in the manual labels.

⸻

\#\#\# All Defined Proactive Services
	•	Instant (second-level, grounded in the current moment)
        •	Safety: immediate bodily/accident danger (flame, blade, electric shock, slip, rotating parts, vehicle proximity) → stop first, then handle.
        •	Tool Use: improper tool operation/configuration (grip, not powered off, orientation, loose chuck, missing guard, unsafe posture).
	•	Short-Horizon (tens of seconds to a few minutes, within a single session)
        •	Next-Step Guidance: workflow is already underway; provide suggestions for the next step based on what has been done.
        •	Error-Recovery: the user has just made a workflow mistake (wrong step, wrong object, wrong target, wrong configuration for this task) and must rollback to fix it.
        •	Resource Reminder: end-of-task state is not handled (fire/power left on, door/cap open, unsaved work, leftover items, missing refill) → remind to close/save/take/refill.

⸻

\#\#\# Input Manual Annotations (the only authoritative time source)

Provides fine-grained temporal information for all dialogue and user actions in the video.

⸻

\#\#\# Objective
	1.	Read each manual annotation labeled as "Safety", and output its time\_window exactly as annotated (start\_time-end\_time, verbatim).
    You must traverse every user-error segment in the manual annotations and process them one by one without omission.
	2.	For each Safety event, output:
        • risk\_type (standardized from the Safety label)
        • objective observation (from comment and/or video JSON; must be directly verifiable)
        • confidence
	3.	If multiple Safety labels exist in the same time-window → output multiple separate events.
If repeated identical labels appear → deduplicate and record merged sources.
	4.	Output ONLY Safety events (not Tool Use, not Privacy, not other types).
	5.	Dialogue generation: for every event, generate a 2-4 turn dialogue:
        • Assistant speaks first, calmly but with appropriately urgent tone;
        • Must clearly state the specific physical hazard (no timestamps);
        • Must provide immediate precaution (e.g., "Please step back," "Keep your hand away from the blade," "Turn off the burner now").
        • User reply must be ≥12 English words and express acceptance/hesitation/justification.
        • Assistant final turn gives short actionable instruction or one-step mitigation, and concludes calmly.
        • Dialogue text must not contain timestamps, but structured output must include aligned clip\_id and time\_window.

⸻

\#\#\# Task Definition / Nature (Instant · Safety)
- Nature: Triggered by immediate physical hazards that can cause injury or damage within a few seconds.  
  (Examples: sharp blade near hand, boiling liquid splashing, exposed electric wire, unstable object overhead, slippery spill underfoot, open flame near clothing, rotating part with no guard.)

- Temporal scope (critical):
  - Each Instant Safety event corresponds to a very short window:
    - typically 0-5 seconds from the onset of the hazardous configuration to the moment a warning should be issued,
    - with a hard upper bound of ≤10 seconds.
  - If the hazardous situation persists or develops over \textgreater{}10 seconds, or requires monitoring over a longer period,
    it should be handled by Short-Horizon proactive services, not Instant Safety.

- Event granularity:
  - Each manual annotation segment labeled with a Safety category and fitting the above temporal scope is counted as one Safety event.
  - Do not merge multiple separated hazard segments into a single long event; keep each labeled hazard window as an independent instant event.

- Common labels include:
  `sharp\_blade\_near\_hand`, `spill\_slip\_risk`, `electric\_shock\_risk`,
  `open\_flame\_near\_cloth`, `hot\_surface\_burn\_risk`,
  `unguarded\_rotating\_part`, `falling\_object\_risk`, `vehicle\_close\_pass`, etc.

- Trigger strategy:
  - Trigger instantly per annotation segment, with no cross-segment aggregation and no modification of time windows  
    (no stretching, shortening, smoothing, or merging).

- Priority over other services:
  - If a tool-use mistake or a workflow / process error creates an acute physical danger (e.g., high risk of cut, burn, electric shock, collision) that could harm the user or others within seconds,  
    it must be classified as Instant · Safety rather than Tool Use, Error-Recovery, or other service types.

⸻

\#\#\# Output Format and Rules

Two parallel arrays must be produced: safety\_instant\_events and dialogs.
Each Safety event must correspond to exactly one dialogue.

\#\#\#\# Mandatory constraints
  • Exact Match: time\_window must match the manual annotation exactly.
  • Annotation Only: You may not invent new windows or extend/shorten segments.
  • Objective observation: Use verifiable details; no speculation.
  • Multi-label: separate event entries; identical ones deduplicated.
  • Order: sort by clip\_id ascending, then by start\_time ascending.

\#\#\#\# Dialogue constraints
  • 2-4 turns
  • Assistant speaks first
  • First turn must include:
    •	explicit mention of the safety hazard
    •	immediate risk-mitigation instruction (Stop / Move / Step back / Avoid contact / Turn off / Pull hand away)
  • User reply:
    •	≥12 English words
    •	shows realistic reasoning (agreement, hesitation, justification)
  • Assistant final turn:
    •	concise safety correction / SOP mini-card / confirmation
  • No timestamps in dialogue
  • No Tool-Use/Privacy content
  • No hallucinated facts

⸻

\#\#\# Unified Output Schema
\{
  "safety\_instant\_events": [
    \{
      "clip\_id": "\textless{}from annotations.clip\_id\textgreater{}",
      "segment\_id": "\textless{}from annotations.segment\_id or 'unknown'\textgreater{}",
      "time\_window": "HH:MM:SS.mmm-HH:MM:SS.mmm",
      "risk\_type": "sharp\_blade\_near\_hand \textbar{} spill\_slip\_risk \textbar{} electric\_shock\_risk \textbar{} open\_flame\_near\_cloth \textbar{} hot\_surface\_burn\_risk \textbar{} unguarded\_rotating\_part \textbar{} falling\_object\_risk \textbar{} vehicle\_close\_pass \textbar{} other",
      "observation": "\textless{}concise, objective evidence (no speculation)\textgreater{}",
      "source": "manual\_annotation",
      "confidence": 0.0
    \}
  ],
  "dialogs": [
    \{
      "clip\_id": "\textless{}same as paired event\textgreater{}",
      "segment\_id": "\textless{}same as paired event\textgreater{}",
      "time\_window": "HH:MM:SS.mmm-HH:MM:SS.mmm",
      "risk\_type": "\textless{}same as paired event\textgreater{}",
      "dialogue": [
        \{"role": "assistant", "utterance": ""\},
        \{"role": "user", "utterance": "\textless{}non-trivial response (\textgreater{}=12 words)\textgreater{}"\},
        \{"role": "assistant", "utterance": "\textless{}short immediate mitigation + confirmation\textgreater{}"\},
        \{"role": "user", "utterance": ""\}   // optional
      ]
    \}
  ]
\}

\#\#\#\# Failure Case (If there are no valid Safety events in current video clip)
\{
  "clip\_id": "",
  "safety\_instant\_events": [],
  "dialogs": [],
  "note": "No Safety risk segments were present in the provided manual annotations."
\}
\end{promptbox}

\begin{promptbox}[HoloAssist — Instant · Tool Use]
\#\#\# Role

You are an Instant Proactive Service (Instant PS) annotation and dialogue-generation assistant for the HoloAssist dataset.
In laboratory / hands-on operation settings, you analyze manual annotations to extract time-windows of "Tool Use" risks / improper operations, and for each extracted event, you generate a 2-4 turn "assistant ↔ user" dialogue.

You must rely only on the time-windows provided by the manual annotations.
You must not extend, shorten, merge, or fabricate any time segments that do not exist in the manual labels.

⸻

\#\#\# All Defined Proactive Services
	•	Instant (second-level, grounded in the current moment)
        •	Safety: immediate bodily/accident danger (flame, blade, electric shock, slip, rotating parts, vehicle proximity) → stop first, then handle.
        •	Tool Use: improper tool operation/configuration (grip, not powered off, orientation, loose chuck, missing guard, unsafe posture).
	•	Short-Horizon (tens of seconds to a few minutes, within a single session)
        •	Next-Step Guidance: workflow is already underway; provide suggestions for the next step based on what has been done.
        •	Error-Recovery: the user has just made a workflow mistake (wrong step, wrong object, wrong target, wrong configuration for this task) and must rollback to fix it.
        •	Resource Reminder: end-of-task state is not handled (fire/power left on, door/cap open, unsaved work, leftover items, missing refill) → remind to close/save/take/refill.

⸻

\#\#\# Input Manual Annotations (authoritative time source)

Provides fine-grained temporal information for all dialogue and user actions in the video.

⸻

\#\#\# OBJECTIVE
	1.	Read each manual annotation labeled as "Tool Use", and output its time\_window exactly as annotated (start\_time-end\_time, verbatim).
    You must traverse every user-error segment in the manual annotations and process them one by one without omission.
	2.	For each event, output:
        •	risk\_type (standardized from the label)
        •	an objective observation (from comment and/or video JSON; must be verifiable)
        •	confidence
	3.	If multiple labels exist in the same time-window → output multiple separate events.
        If repeated identical labels appear → deduplicate and conceptually merge their sources.
	4.	Output only Tool Use events (not Safety, not Privacy, not Error-Recovery, not Resource Reminder).
	5.	Dialogue generation: for every event, generate a 2-4 turn dialogue:
        •	Assistant speaks first, calmly, politely, low-intrusion.
        •	Clearly state the specific tool-use risk (no timestamps), and provide 1-2 actionable corrections
    (e.g., "power off first, then…", "adjust your grip below the guard ring").
        •	User must not reply vaguely; produce ≥12 English words with meaningful content (accept/modify/decline and give reasons).
        •	Assistant closes with confirmation / optional SOP snippet / short reminder.
        •	Dialogue text must not include timestamps, but the structured output must include aligned clip\_id and time\_window.

⸻

\#\#\# Task Definition / Nature (Instant · Tool Use)

Core Focus
	•	This category is restricted to problems that arise purely from how a tool is being used: grip, posture, contact, orientation, clamp/guard state, power state / configuration of the tool itself.
	•	By definition, Instant · Tool Use never requires rolling back or redoing previously completed workflow steps. The current step (object, target, step choice) is logically correct; only the usage technique is problematic.
	•	It does not cover mistakes about which object / part / slot / step / goal is chosen in the workflow (those belong to Short-Horizon · Error-Recovery).

Nature
	•	Triggered when an immediate tool-related operational risk appears.
	•	Focus on technique / configuration issues (grip, contact area, hand placement, body posture, orientation, clamp/guard state, power-off timing) that can become unsafe or damaging within a few seconds if not corrected.
	•	If the same mis-use is already causing an acute bodily hazard (e.g., clear cut / burn / electric-shock risk), it should be classified as Instant · Safety, not Tool Use.

Temporal scope (critical)
	•	Each Instant Tool Use event corresponds to a very short snippet of ongoing execution:
	•	typically 0-5 seconds between the risky configuration and when intervention should happen;
	•	with a hard upper bound of ≤10 seconds.
	•	If understanding or fixing the problem requires:
	•	looking back over ≥10 seconds of prior workflow, or
	•	undoing earlier completed steps and then redoing them,
then it should conceptually be handled by Short-Horizon services (especially Error-Recovery), not by Instant · Tool Use.

Event granularity
	•	Each manual annotation segment that satisfies the temporal scope and nature above is counted as one Tool Use event.
	•	You must not merge multiple distant segments into a longer window to "simulate" an instant event.

Common labels (examples)

improper\_grip, unstable\_handle, device\_not\_off, unsafe\_posture,
wrong\_orientation, missing\_guard, loose\_attachment, unstable\_support, etc.

Example 1 (Tool Use, not Error-Recovery)
The user is drilling into a workpiece with the correct drill bit and position, but their hand is very close to the rotating bit and the drill is tilted, making the operation unstable.
If they simply reposition their hand further away, adjust the tilt, and stabilize the drill, the task remains valid. No previous step needs to be undone.
This is an Instant · Tool Use event (technique correction), not Error-Recovery.

⸻

\#\#\# Mutual Exclusion \& Priority vs. Error-Recovery (and Safety)

When deciding between Instant · Tool Use, Short-Horizon · Error-Recovery, and Instant · Safety, use the following rules.

1. Completion vs. ongoing execution (primary test: Tool Use vs. Error-Recovery)
Use this completion test first:

"If the user immediately switches to the correct technique from now on, without undoing anything already done, does the mistake disappear?"

	•	If YES → this is Tool Use (ongoing execution / technique correction).
	•	If NO, because the current state is already wrong and must be undone and redone, then it belongs to Short-Horizon · Error-Recovery, not Tool Use.

In other words:
	•	Tool Use
        •	The step itself is logically correct (right object, right target, right step for this task).
        •	The problem lies in how the tool is being operated (grip, angle, stability, power-off timing, missing clamp/guard, etc.).
        •	Fix = adjust how the tool is being handled / configured right now, without rolling back earlier workflow states.
	•	Error-Recovery
        •	The workflow state itself is wrong (wrong part installed, wrong sample loaded, wrong slot used, wrong target selected, steps swapped, required step skipped, etc.).
        •	Fix = stop, undo what was done, and redo the step correctly.
        •	These should not be labeled as Tool Use in this task.

2. Technique vs. workflow (rephrased decision rule)
	•	If the main problem is how the tool is being handled or configured in this short 0-10 second window
(grip, posture, orientation, clamp/guard, power-off timing), and correcting it means adjusting the current action, classify it as Instant · Tool Use.
	•	If the main problem is what has already been done in the workflow
(wrong object, wrong slot/target, wrong order, wrong configuration for this task, skipped required step), and the user must undo and redo a step, classify it as Short-Horizon · Error-Recovery.

3. Safety override
	•	If the current tool use creates an immediate, high-risk safety hazard (e.g., hand directly in front of an active blade, imminent burn from an exposed hot surface, clear electric-shock risk),
the primary label should be Instant · Safety, even if there is also a technique issue.
	•	In such cases, prioritize Safety over Tool Use.

4. Time scale
	•	Tool Use: typically 0-10 seconds, focused on a currently ongoing motion or micro configuration with no rollback.
	•	Error-Recovery: can span ≈10 seconds to a few minutes, requiring short-term memory of earlier completed actions and explicit rollback.

5. Example 2 (Error-Recovery, not Tool Use)
The user is assembling a device that requires inserting Part A first and then Part B.
Instead, they insert Part B directly, tighten it, and skip Part A.
Simply improving their hand technique or tightening style cannot fix this — the assembly sequence itself is wrong.
The assistant should ask them to stop, remove Part B (undo), insert Part A, then re-insert Part B in the correct order (redo).
This is Error-Recovery because it is a workflow-level mistake that requires rollback + redo, not just a Tool Use adjustment.

In this task, you are only asked to output Tool Use events.
Segments that match the Error-Recovery definition above should not be labeled as Tool Use.

⸻

\#\#\# Output Format and Rules

You must produce two parallel arrays: tool\_use\_instant\_events and dialogs.
Each event must correspond to exactly one dialogue.

\#\#\# Mandatory constraints
	•	Exact Match
        •	time\_window must match the annotated start\_time-end\_time exactly.
        •	No stretching, shortening, smoothing, or merging.
	•	Annotation Only
	    •	You may not introduce new or extended time windows.
	•	Objective observation
	    •	Must be verifiable; no speculation or hidden-mental-state guesses.
	•	Multi-label
	    •	Separate output entries for each label; exact duplicates merged.
	•	Ordering
	    •	Sort by clip\_id ascending, then by start\_time ascending.

\#\#\# Dialogue constraints
	•	2-4 turns.
	•	Assistant speaks first.
	•	First assistant turn must include:
	•	explicit mention of the specific tool-use risk, and
	•	1-2 concrete corrective steps.
	•	User reply:
	•	≥12 words, non-trivial, expresses acceptance, modification, or refusal with explanation.
	•	Assistant final turn:
	•	step-by-step guidance / confirmation / optional mini SOP card.
	•	No timestamps in dialogue.
	•	No Safety / Privacy content.
	•	No hallucinated facts.

⸻

\#\#\# Unified Output Schema
\{
  "tool\_use\_instant\_events": [
    \{
      "clip\_id": "\textless{}from annotations.clip\_id\textgreater{}",
      "segment\_id": "\textless{}from annotations.segment\_id or 'unknown'\textgreater{}",
      "time\_window": "HH:MM:SS.mmm-HH:MM:SS.mmm",
      "risk\_type": "improper\_grip \textbar{} unstable\_handle \textbar{} device\_not\_off \textbar{} unsafe\_posture \textbar{} wrong\_orientation \textbar{} missing\_guard \textbar{} loose\_attachment \textbar{} other",
      "observation": "\textless{}concise, objective evidence (no speculation)\textgreater{}",
      "source": "manual\_annotation",
      "confidence": 0.0
    \}
  ],
  "dialogs": [
    \{
      "clip\_id": "\textless{}same as paired event\textgreater{}",
      "segment\_id": "\textless{}same as paired event\textgreater{}",
      "time\_window": "HH:MM:SS.mmm-HH:MM:SS.mmm",
      "risk\_type": "\textless{}same as paired event\textgreater{}",
      "dialogue": [
        \{ "role": "assistant", "utterance": "" \},
        \{ "role": "user", "utterance": "\textless{}non-trivial response (\textgreater{}=12 words)\textgreater{}" \},
        \{ "role": "assistant", "utterance": "\textless{}two-step corrective action + confirmation\textgreater{}" \},
        \{ "role": "user", "utterance": "" \}
      ]
    \}
  ]
\}

\#\#\#\# Failure Case (If there are no valid Tool Use events in current video clip)
\{
  "tool\_use\_instant\_events": [],
  "dialogs": [],
\}
\end{promptbox}

\begin{promptbox}[HoloAssist — Short-Horizon · Error-Recovery]
\#\#\# Role

You are a Short-Horizon Error-Recovery annotation and dialogue-generation assistant for the HoloAssist dataset.
Based on manual annotations, you extract time-windows where the user has just completed, or is about to complete, a wrong workflow step, and for each event you generate a 2-4 turn "assistant ↔ user" dialogue.

You must rely only on the time-windows provided by the manual annotations.
You must not extend, shorten, merge, or fabricate any time segments that do not exist in the manual labels.

⸻

\#\#\# All Defined Proactive Services
	•	Instant (second-level, grounded in the current moment)
        •	Safety: immediate bodily/accident danger (flame, blade, electric shock, slip, rotating parts, vehicle proximity) → stop first, then handle.
        •	Tool Use: improper tool operation/configuration (grip, not powered off, orientation, loose chuck, missing guard, unsafe posture).
	•	Short-Horizon (tens of seconds to a few minutes, within a single session)
        •	Next-Step Guidance: workflow is already underway; provide suggestions for the next step based on what has been done.
        •	Error-Recovery: the user has just made a workflow mistake (wrong step, wrong object, wrong target, wrong configuration for this task) and must rollback to fix it.
        •	Resource Reminder: end-of-task state is not handled (fire/power left on, door/cap open, unsaved work, leftover items, missing refill) → remind to close/save/take/refill.

⸻

\#\#\# INPUT Manual Annotations (authoritative time source)

Provides fine-grained temporal information for all dialogues and user actions in the video.

⸻

\#\#\# OBJECTIVE
	1.	For each manual annotation segment labeled as Error-Recovery (or equivalent label), output the time\_window exactly as annotated: time\_window = start\_time-end\_time (verbatim).
    You must traverse every user-error segment in the manual annotations and process them one by one without omission.
	2.	For each event, output:
        •	error\_type (standardized from the label)
        •	an objective observation (grounded in the annotation JSON, no speculation)
        •	confidence
	3.	If multiple different Error-Recovery labels exist in the same time window → output multiple separate events.
        If there are repeated identical labels for the same window → deduplicate and merge their sources conceptually.
	4.	Output only Error-Recovery events (do not output Tool Use / Safety / Resource Reminder / etc.).
	5.	For each event, generate a 2-4 turn dialogue:
        •	The assistant speaks first, gently pointing out the error or impending error.
        •	The assistant proposes 1-2 concrete repair paths (rollback / replace / retune / redo).
        •	The user's reply must be non-trivial (≥12 English words) and express acceptance, adjustment, or refusal with some reasoning.
        •	The assistant then guides the rollback / fix and confirms that the workflow is back on track.
        •	Dialogue text must not show any timestamps, but structured fields must keep clip\_id and time\_window aligned with the event.

⸻

\#\#\# Task Definition / Nature (Short-Horizon · Error-Recovery)

Core Focus
- This category is restricted to workflow-level mistakes where the task has already entered an incorrect completed state, such that the user must rollback + redo one or more steps to return to a valid workflow path.
- By definition, Error-Recovery always requires undoing something.
    If no rollback is needed, the issue is *not* Error-Recovery.

Nature
- Triggered when the user has already performed a wrong choice, wrong object, wrong target, wrong step, or wrong configuration that invalidates the current workflow.
- If left uncorrected, the run will fail, produce incorrect results, or deviate significantly from the intended sequence.
- Fixing the issue requires:
    1. Stop the current action
    2. Undo / rollback the wrong state
    3. Redo the step correctly

Temporal Scope (critical)
- Short-horizon within the same session.
- Typically spans:
    - ≈10 seconds to a few minutes,
    - and at most within the last \textasciitilde{}10 minutes of actions.
- You follow only long enough to return to the last correct state — not across long breaks or activity changes.

Event Granularity
- Each manual annotation segment that reflects a workflow-state error requiring rollback is one Error-Recovery event.
- Do not merge separate segments.
- Do not shorten or extend annotated windows.

Common Labels (examples)
These labels all imply a wrong workflow state that cannot be fixed by adjusting technique alone:
- wrong\_order
- missing\_component
- wrong\_part\_type
- wrong\_dose
- misconfiguration\_param *(only when it invalidates the run and requires redo)*
- forgot\_step\_required
- wrong\_target
- wrong\_container

Example 1 (Error-Recovery, not Tool Use)
The user must insert Part A first and then Part B.
They instead insert Part B, tighten it, and skip Part A.
Adjusting technique cannot fix the wrong sequence.
Fix = remove Part B → insert A → redo B.
This is Error-Recovery (rollback + redo).

Example 2 (Tool Use, not Error-Recovery)
The user drills with the correct bit and correct target, but their hand is too close and the drill is tilted.
The workflow state is correct; only technique is wrong.
Fix = adjust grip/angle. No rollback.
Therefore, this is Tool Use, not Error-Recovery.

⸻

\#\#\# Mutual Exclusion \& Priority vs. Tool Use (and Safety)

1. Completion vs. Ongoing Execution (Primary Test)
Use the core discriminative question:
\textgreater{} *"If the user immediately switches to the correct technique from now on, without undoing anything already done, does the mistake disappear?"*
\textgreater{} 
- YES → Tool Use (technique correction during a valid step).
- NO → Error-Recovery (workflow is already in a wrong completed state; rollback required).

2. Workflow vs. Technique (What is actually wrong?)
Error-Recovery
- The workflow state itself is invalid:
    - wrong part / wrong sample
    - wrong slot / wrong container
    - wrong target
    - skipped required step
    - wrong sequence / swapped order
    - misconfiguration that makes the run invalid
- Fix = undo + redo.

Tool Use
- The workflow choice (object, target, step) is correct, but:
    - grip, posture, orientation, angle
    - speed, force, tool contact
    - clamp/guard not secured
    - device not powered off yet
- Fix = adjust technique, with no rollback.

3. Safety Override
- If the misuse creates an acute physical hazard (cut/burn/shock/collision) that threatens safety within seconds,
    → classify as Instant · Safety, not Error-Recovery or Tool Use.

4. Time Scale
- Tool Use: 0-10 seconds; micro-operations; no rollback.
- Error-Recovery: 10 seconds to a few minutes; requires remembering and fixing previous steps.

5. Example Revisited (Error-Recovery vs. Tool Use)
Same as Example 1 \& 2 above:
If the step itself is wrong → Error-Recovery.
If the technique is wrong → Tool Use.

In this task, you are only asked to output Error-Recovery events.
For segments that fit the Tool Use definition above, do not create Error-Recovery events (they belong to Instant · Tool Use instead).

⸻

\#\#\# OUTPUT FORMAT AND RULES
	•	You must output two parallel arrays:
	•	error\_recovery\_events
	•	dialogs
Each event in error\_recovery\_events must correspond to exactly one dialogue in dialogs.
	•	Exact Match (time window)
	•	time\_window must equal the annotated start\_time-end\_time.
	•	No stretching, shortening, merging, or smoothing of time windows.
	•	Annotation-only scope
	•	You may not create new time windows not present in the manual annotations.
	•	You may not extend or split existing windows.
	•	Objective observation
	•	observation must use verifiable cues from annotation JSON.
	•	Avoid psychological interpretation or hidden intent.
	•	Ordering
	•	Sort outputs by clip\_id ascending, then by start\_time ascending.
	•	Dialogue style
	•	Review / repair style:
	•	Point out the deviation gently.
	•	Offer 1-2 concrete repair paths (rollback / redo / change parameter, etc.).
	•	Confirm that the workflow is now back on the correct track.
	•	Avoid blame or harsh language; the tone should be supportive and practical.

⸻

\#\#\# Unified Output Schema (single-line JSON skeleton)
\{
  "error\_recovery\_events": [
    \{
      "clip\_id": "",
      "segment\_id": "\textless{}seg or 'unknown'\textgreater{}",
      "time\_window": "HH:MM:SS.mmm-HH:MM:SS.mmm",
      "error\_type": "wrong\_order \textbar{} missing\_component \textbar{} wrong\_part\_type \textbar{} wrong\_dose \textbar{} misconfiguration\_param \textbar{} forgot\_step\_required \textbar{} other",
      "observation": "",
      "source": "manual\_annotation",
      "confidence": 0.0
    \}
  ],
  "dialogs": [
    \{
      "clip\_id": "",
      "segment\_id": "",
      "time\_window": "HH:MM:SS.mmm-HH:MM:SS.mmm",
      "error\_type": "",
      "dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}gentle pinpoint of the error + propose rollback/fix\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}non-trivial reply (\textgreater{}=12 words)\textgreater{}"
        \},
        \{
          "role": "assistant",
          "utterance": "\textless{}guide through rollback/replace/retune + confirm back-on-track\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": ""
        \}
      ]
    \}
  ]
\}

\#\#\#\# Failure Case
If no valid Error-Recovery segments are present in the provided manual annotations:
\{
  "error\_recovery\_events": [],
  "dialogs": [],
\}
\end{promptbox}

\begin{promptbox}[HoloAssist — Short-Horizon · Next-Step Guidance]
\#\#\# ROLE

You are a Short-Horizon Task Continuity (Next-Step Guidance) annotation and dialogue-generation assistant for the HoloAssist dataset.
Using manual annotations, you extract time-windows related to Next-Step Guidance, and generate a 2-4 turn "assistant ↔ user" dialogue for each event.

You must rely only on the time-windows provided in the manual annotations.
You must NOT extend, shorten, modify, merge, or create any new time-windows.

⸻

\#\#\# INPUT

Manual Annotations (the only authoritative time source)

Provides fine-grained temporal information describing all dialogues and user actions in the video.

⸻

\#\#\# All Defined Proactive Services
	•	Instant (second-level, grounded in the current moment)
        •	Safety: immediate bodily/accident danger (flame, blade, electric shock, slip, rotating parts, vehicle proximity) → stop first, then handle.
        •	Tool Use: improper tool operation/configuration (grip, not powered off, orientation, loose chuck, missing guard, unsafe posture).
	•	Short-Horizon (tens of seconds to a few minutes, within a single session)
        •	Next-Step Guidance: workflow is already underway; provide suggestions for the next step based on what has been done.
        •	Error-Recovery: the user has just made a workflow mistake (wrong step, wrong object, wrong target, wrong configuration for this task) and must rollback to fix it.
        •	Resource Reminder: end-of-task state is not handled (fire/power left on, door/cap open, unsaved work, leftover items, missing refill) → remind to close/save/take/refill.
        
⸻

\#\#\# OBJECTIVE
	1.	Read each manual annotation labeled as Next-Step, and output the exact time\_window (start\_time-end\_time).
	2.	Output guidance\_type (standardized from the label), objective observation, and confidence.
	3.	If multiple labels exist in the same time-window → output multiple entries; repeated identical labels → deduplicate and merge sources.
	4.	Output only Next-Step Guidance events (not Tool Use / Safety / Resource / Error-Recovery).
	5.	For each event, generate a 2-4 turn dialogue:
        •	Assistant speaks first: acknowledge completed step(s) and offer 1-2 possible next-step paths (or parameter/tool options).
        •	User response must be non-trivial (≥12 English words).
        •	Assistant confirms the chosen path and provides a mini step-card / timer / material checklist.
        •	Dialogue text must not show timestamps, but structured fields must retain alignment.

⸻

\#\#\# TASK DEFINITION / NATURE (Short-Horizon · Next-Step)
    •	Nature: Triggered after the user completes a correct step, to provide the next logical action in a multi-step workflow
(e.g., cooking, assembly, lab work, device operation, software procedures).
    •	Activation Conditions (critical)
    A segment qualifies as Next-Step Guidance only if all of the following hold:
        •	The user has just completed a correct step
    (e.g., prepping ingredients, opening/closing a lid, tightening, switching a mode, finishing a measurement).
        •	The current task is clearly a multi-step workflow
    with a next step that has obvious logical continuity.
        •	The user is in a state of waiting / pausing / hesitating,
    or otherwise appears ready for the next actionable instruction.
    •	Temporal Scope (short-horizon)
        •	Operates within the same ongoing task session.
        •	Uses ≈10 seconds to a few minutes, up to \textasciitilde{}10 minutes of recent context.
        •	Focuses on the structure: completed A/B → pending C.
    •	Event Granularity
        •	Each manual annotation segment labeled as Next-Step is counted as one event.
        •	Do not merge separated segments.
        •	No inferred, new, or extended time windows.
    •	Common Labels: next\_step\_mixing, next\_step\_install, next\_step\_measure, next\_step\_cleanup, next\_step\_save\_export, etc.
    •	Not Included (Routing Rules)
        •	If the user performed an incorrect step → classify as Short-Horizon · Error-Recovery.
        •	If the user's technique of using a tool is unsafe or improper → classify as Instant · Tool Use.
        •	If an acute physical hazard appears (cut/burn/shock/impact within seconds) → classify as Instant · Safety.
    •	Intuition Example
        •	After finishing chopping ingredients → "You can heat the pan next."
        •	After securing a component → "Next, attach the connector."

⸻

\#\#\# OUTPUT FORMAT AND RULES
Produce two parallel dictionaries: next\_step\_events and dialogs, with one-to-one correspondence. Each event in next\_step\_events must have exactly one matching dialog in dialogs.

\#\#\#\# Mandatory Constraints
1. Exact Match of Time Window
	•	time\_window must exactly match the annotation
(verbatim start\_time-end\_time).
2. Annotation Only
	•	You may not create new time windows.
	•	You may not extend, shorten, merge, or infer new segments.
3. Objective Observation
	•	Grounded in the manual annotation. 
	•	No speculation, emotion, or psychological interpretation.
4. Ordering
	•	Sort by clip\_id ascending, then by start\_time ascending.
5. Multi-label
	•	Multiple Next-Step labels in the same time-window → produce separate events.
	•	Identical duplicates → deduplicate but merge sources conceptually.
6. Redundancy Avoidance
	•	When two adjacent Next-Step Guidance timestamps occur within a short interval (≤10 seconds) and correspond to the same ongoing process or workflow, only the earlier timestamp should trigger a Next-Step Guidance event.
	•	The later timestamp should be ignored to avoid redundant or overly frequent next-step prompts.

\#\#\#\# Dialogue Constraints

Each dialogue must be 2-4 turns, road-map style.

The structure:
Turn 1 — Assistant
	•	Acknowledge what the user has just correctly completed.
	•	Provide 1-2 next-step options or a clear next action.
	•	No evaluative or corrective tone.
Turn 2 — User
	•	≥ 12 English words
	•	Must show a meaningful response:
acceptance, choosing among options, modifying the plan, or asking for clarity.
Turn 3 — Assistant
	•	Confirm the user's chosen path.
	•	Provide a brief next-step guide card / checklist / parameter reminder.
(Optional) Turn 4 — User
	•	Brief acknowledgment.

No timestamps in dialogue.
No Safety / Tool-Use / Error-Recovery language.

⸻

\#\#\# Unified Output Schema (single-line JSON)
\{
  "next\_step\_events": [
    \{
      "clip\_id": "",
      "segment\_id": "\textless{}seg or 'unknown'\textgreater{}",
      "time\_window": "HH:MM:SS.mmm-HH:MM:SS.mmm",
      "guidance\_type": "next\_step\_mixing \textbar{} next\_step\_install \textbar{} next\_step\_measure \textbar{} next\_step\_cleanup \textbar{} next\_step\_save\_export \textbar{} other",
      "observation": "\textless{}objective cue of what's completed and what's next\textgreater{}",
      "source": "manual\_annotation",
      "confidence": 0.0
    \}
  ],
  "dialogs": [
    \{
      "clip\_id": "",
      "segment\_id": "",
      "time\_window": "HH:MM:SS.mmm-HH:MM:SS.mmm",
      "guidance\_type": "",
      "dialogue": [
        \{"role": "assistant", "utterance": "\textless{}acknowledge completed step(s) + offer 1-2 next options\textgreater{}"\},
        \{"role": "user", "utterance": "\textless{}non-trivial reply (\textgreater{}=12 words), choose/ask/modify\textgreater{}"\},
        \{"role": "assistant", "utterance": "\textless{}confirm choice + mini step card / timer / checklist\textgreater{}"\},
        \{"role": "user", "utterance": ""\}
      ]
    \}
  ]
\}

\#\#\#\# Failure Case (If there are no valid Next-Step Guidance events in current video clip)
\{
  "next\_step\_events": [],
  "dialogs": [],
\}
\end{promptbox}

\begin{promptbox}[HoloAssist — Short-Horizon · Resource Reminder]
\#\#\# Role

You are a Short-Horizon Resource Reminder annotation and dialogue-generation assistant for the HoloAssist dataset.  
In short-term task episodes, you analyze manual annotations to extract time-windows where a state or resource has not been properly closed, shut off, saved, secured, or taken, and for each event you generate a 2-4 turn "assistant ↔ user" dialogue.

You must rely only on the time-windows provided in the manual annotations.  
You must not extend, shorten, merge, or fabricate any new time-windows.

⸻

\#\#\# All Defined Proactive Services
	•	Instant (second-level, grounded in the current moment)
        •	Safety: immediate bodily/accident danger (flame, blade, electric shock, slip, rotating parts, vehicle proximity) → stop first, then handle.
        •	Tool Use: improper tool operation/configuration (grip, not powered off, orientation, loose chuck, missing guard, unsafe posture).
	•	Short-Horizon (tens of seconds to a few minutes, within a single session)
        •	Next-Step Guidance: workflow is already underway; provide suggestions for the next step based on what has been done.
        •	Error-Recovery: the user has just made a workflow mistake (wrong step, wrong object, wrong target, wrong configuration for this task) and must rollback to fix it.
        •	Resource Reminder: end-of-task state is not handled (fire/power left on, door/cap open, unsaved work, leftover items, missing refill) → remind to close/save/take/refill.

⸻

\#\#\# INPUT Manual Annotations (authoritative time source)
Provides fine-grained temporal information describing all dialogues and user actions in the video.

⸻

\#\#\# Objective
1. Traverse all manual annotations labeled as Resource Reminder (or equivalent label) and output `time\_window = start\_time-end\_time` exactly as annotated.
   You must traverse every user-error segment in the manual annotations and process them one by one without omission.
2. For each event, output:
   - `reminder\_type` (standardized from the label),
   - an objective `observation` (verifiable from annotation / video JSON, no speculation),
   - `confidence`.
3. If multiple different Resource Reminder labels exist in the same time-window → output multiple separate events.  
   If repeated identical labels appear → deduplicate and conceptually merge sources.
4. Output only Short-Horizon · Resource Reminder events (do not output Safety / Tool Use / Error-Recovery / etc.).
5. For each event, generate a 2-4 turn dialogue:
   - Assistant speaks first, politely highlighting the unclosed / unhandled state  
     (e.g., power left on, unsaved file, cap loose, door unlocked, item left behind, low supply).
   - Assistant offers 1-2 concrete options (close / save / lock / bring item / refill / set a later reminder).
   - User reply must be non-trivial (≥12 English words) and show some reasoning or preference.
   - Assistant confirms the chosen action or records a short-term reminder / "ignore once".
   - Dialogue text must not include timestamps (the structured fields keep `clip\_id` and `time\_window`).

⸻

\#\#\# Task Definition / Nature (Short-Horizon · Resource Reminder)

- Nature (what it is):  
  A lightweight end-state closure reminder, focusing on turning devices/resources from  
  "on / open / unsaved / left-behind / low-supply" → safe and stable state in the current episode.

  Typical examples:
  - forgetting to turn off a stove or power source,
  - forgetting to close water/gas valves,
  - leaving a door unlocked or a bottle cap loose,
  - leaving work unsaved in an application,
  - walking away while items or tools are left behind,
  - noticing that supplies are nearly empty and should be refilled soon.

- Activation conditions (critical):
  - The unclosed / unmanaged state is related to the current short workflow  
    (same room / same task context, not a distant past event).
  - The user is about to leave or shift context, such that forgetting this state may cause  
    loss, waste, mild damage, or inconvenience (but not acute bodily harm).
  - The risk is non-acute: it does not yet reach the level of immediate physical danger  
    (if it clearly threatens bodily safety within seconds, it belongs to Instant · Safety instead).

- Temporal scope (short-horizon):
  - Operates within tens of seconds to a few minutes, up to roughly one short session (\textasciitilde{}10 minutes).
  - The reminder remains relevant only until the state is handled (closed/saved/locked/taken/refilled)  
    or the user explicitly ignores it *this time*.

- Event granularity:
  - Each manual annotation segment labeled as Resource Reminder and fitting the above is counted as one event.
  - Do not merge separated reminder segments into one long event.
  - If the user repeats the same unclosed state continuously over a short window,  
    you only need to trigger at the first moment when the oversight becomes clear.

- Common labels include:
  - `stove\_left\_on`, `unsaved\_data`, `cap\_loose`,  
    `door\_unlocked`, `valve\_open`, `power\_not\_off`,  
    `forgot\_item\_left`, `low\_supply\_needs\_refill`, etc.

- Relationship to other services (routing rules):
  - Not Safety:  
    If forgetting a resource or state has already created an acute physical hazard
    (e.g., strong fire hazard, high risk of burn/shock/explosion within seconds),  
    classify it as Instant · Safety, not Resource Reminder.
  - Not Tool Use:  
    If the core issue is how a tool is being held or operated right now  
    (grip, posture, orientation, guard/clamp, power-off timing) and does not involve a leftover state,  
    classify it as Instant · Tool Use, not Resource Reminder.
  - Not Error-Recovery:  
    If the main problem is that a workflow step or decision is wrong and must be rolled back + redone  
    (wrong object/slot/parameter/order), classify it as Short-Horizon · Error-Recovery, not Resource Reminder.
  - Resource Reminder is only for "state/closure not finished yet",  
    when previous steps are basically correct but cleanup / shutdown / save / take / refill is missing.

⸻

\#\#\# Output Format and Rules

Two parallel arrays must be produced: `resource\_reminder\_events` and `dialogs`.  
Each event must correspond to exactly one dialogue.

\#\#\#\# Mandatory constraints

- Exact Match (time window):  
  `time\_window` must match the annotated `start\_time-end\_time` verbatim.  
  No stretching, shortening, smoothing, or merging.

- Annotation Only:  
  You may not introduce new time windows, nor split or extend existing ones.

- Objective observation:  
  - Use only verifiable cues from the annotation / video JSON.  
  - Avoid guessing user intentions or emotions.

- Multi-label handling:  
  - If multiple different Resource Reminder labels share the same window → output separate events.  
  - If labels are completely identical → output one event and treat others as duplicates.

- Ordering:  
  Sort outputs by `clip\_id` ascending, then by `start\_time` ascending.

\#\#\#\# Dialogue constraints

- Length: 2-4 turns per dialogue, assistant speaks first.
- Assistant first turn:
  - Politely points out the specific unclosed / unmanaged state.
  - Offers 1-2 concrete options, such as:
    - "turn off / close / lock now",
    - "save the file now",
    - "take this item with you",
    - "set a short reminder instead."
- User turn:
  - Must contain ≥12 English words,
  - Expresses acceptance, modification (e.g., "remind me later"), or polite refusal with some reasoning.
- Assistant final turn:
  - Confirms the chosen action,
  - Optionally describes the effect (e.g., "stove turned off", "reminder set for 10 minutes"),
  - Keeps tone calm, low-intrusion, and helpful.
- No timestamps inside dialogue text.
- No hallucinated facts; all references to devices/items/states must be plausible given the observation.

⸻

\#\#\# Unified Output Schema (single-line JSON skeleton)
\{
  "resource\_reminder\_events": [
    \{
      "clip\_id": "",
      "segment\_id": "\textless{}seg or 'unknown'\textgreater{}",
      "time\_window": "HH:MM:SS.mmm-HH:MM:SS.mmm",
      "reminder\_type": "stove\_left\_on \textbar{} unsaved\_data \textbar{} cap\_loose \textbar{} door\_unlocked \textbar{} valve\_open \textbar{} power\_not\_off \textbar{} forgot\_item\_left \textbar{} low\_supply\_needs\_refill \textbar{} other",
      "observation": "",
      "source": "manual\_annotation",
      "confidence": 0.0
    \}
  ],
  "dialogs": [
    \{
      "clip\_id": "",
      "segment\_id": "",
      "time\_window": "HH:MM:SS.mmm-HH:MM:SS.mmm",
      "reminder\_type": "",
      "dialogue": [
        \{
          "role": "assistant",
          "utterance": "\textless{}polite cue of the unclosed/unhandled state + quick options\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": "\textless{}non-trivial reply (\textgreater{}=12 words)\textgreater{}"
        \},
        \{
          "role": "assistant",
          "utterance": "\textless{}apply close/save/lock/take/refill or set reminder + confirm\textgreater{}"
        \},
        \{
          "role": "user",
          "utterance": ""
        \}
      ]
    \}
  ]
\}

\#\#\#\# Failure Case (If there are no valid Resource Reminder events in current video clip)
\{
  "resource\_reminder\_events": [],
  "dialogs": [],
\}
\end{promptbox}

% \subsection{CaptainCook4D Annotation Prompt}
% \label{sec:supp_cc4d_annotation}

% CaptainCook4D provides step-level annotations with pre-identified human errors in instructional cooking and assembly tasks. Unlike EgoLife and HoloAssist where each service category has a separate prompt, CaptainCook4D uses a single unified prompt that classifies each annotated error into the appropriate service type and generates the corresponding dialogue. The applicable categories span Instant, Short-Term, and Episodic horizons (7 out of 11 sub-types; Long-Term services are excluded as they require multi-day context).

\begin{promptbox}[CaptainCook4D — Unified Error-to-Service Annotation Prompt]
You are a proactive service annotation assistant for egocentric instructional videos.

You will be given structured step annotations from a task video.
Each step may include:
- a step description,
- start and end times,
- and one or more annotated errors (already identified by humans).

IMPORTANT:
You MUST NOT discover new errors.
You MUST ONLY generate proactive services for the errors that are explicitly annotated.

Your task is to:
For EACH annotated error,
(1) determine the correct proactive service type,
(2) generate a short proactive dialogue (1-2 turns),
based strictly on the provided annotations.

The dialogue should be:
- natural and respectful,
- supportive rather than commanding,
- concise and task-focused,
- appropriate for an instructional / hands-on scenario
  (e.g., cooking, assembling furniture, laboratory experiments).

------------------------------------------------------------
Proactive Service Types (MUST choose exactly ONE per error)
------------------------------------------------------------

\#\#\# Instant Proactive Services (second-level, immediate, less than 10 seconds)

1. Safety
Use ONLY if the annotated error could plausibly cause bodily harm
or an immediate accident.

Examples:
- risk of burns, cuts, electric shock,
- unsafe proximity to moving parts,
- unstable heavy objects,
- hazardous spills or heat.

RULE:
If an error could endanger the user's body,
it MUST be classified as Safety,
even if it also involves a tool or technique.

2. Tool Use
Use when the error reflects:
- improper tool operation,
- unstable or unfamiliar handling,
- incorrect technique that does NOT yet require rollback.

Examples:
- incorrect pouring technique,
- unstable grip,
- poor control,
- lack of precision or consistency.

------------------------------------------------------------

\#\#\# Short-Horizon Proactive Services (10 seconds to 10 minutes)

3. Error-Recovery
Use ONLY if:
- the user has already completed a wrong step,
- the task must be corrected or redone,
- the error typically spans more than \textasciitilde{}10 seconds
  and affects task correctness.

Examples:
- wrong measurement already added,
- wrong component assembled,
- incorrect configuration applied.

4. Next-Step Guidance
Use if:
- the step itself is completed correctly,
- the user is transitioning to the next stage,
- guidance helps move the workflow forward.

5. Resource Reminder
Use if:
- something is left unfinished or unresolved
  while transitioning to another step.

Examples:
- leftover material,
- missing cleanup,
- container not closed,
- power or heat not turned off.

------------------------------------------------------------
\#\#\# Episodic Proactive Services (short-horizon memory within the same day + more than 10 minutes + less than 2.5 hours)

6. Episodic Task Reminder
Use if:
- the current error is best explained by an earlier unfinished commitment or step,
- the user previously started or committed to something earlier in the same session,
- there is no evidence of completion in the provided annotations,
- and the user is now moving on without resolving it.

Examples:
- earlier calibration/setup step was started but not finished,
- a required part-prep step was deferred and is now causing trouble,
- a previously mentioned prerequisite remains incomplete.

7. Episodic Memory Recall
Use if:
- the current error can be corrected by recalling something from earlier in the same session,
- such as where an item was placed, a prior measurement/setting, or an earlier instruction,
- and the annotation/context explicitly contains that earlier information.

Examples:
- recall where a tool/part was placed earlier,
- recall a previously stated measurement/setting,
- recall an earlier instruction that resolves the current confusion.

NOTE:
Use Episodic services ONLY when the provided annotations/context explicitly support
a same-session dependency. Do NOT speculate or invent prior events.

------------------------------------------------------------
STRICT Classification Rules
------------------------------------------------------------

- Any error that may cause bodily injury → Safety.
- Unstable or unskilled operation → Tool Use.
- Errors that require rollback or correction → Error-Recovery.
- Do NOT downgrade Safety to Tool Use.
- Do NOT use Error-Recovery unless correction is necessary.

------------------------------------------------------------
Dialogue Generation Rules
------------------------------------------------------------

For EACH error:
- Generate a short proactive dialogue of 1-2 turns.
- The assistant speaks first.
- The tone must be polite, calm, and respectful.
- Do NOT scold, command, or sound judgmental.
- Do NOT mention "error", "mistake", or "annotation".
- The dialogue should naturally fit into the task flow.

------------------------------------------------------------
Output Format (STRICT JSON)
------------------------------------------------------------

For each error, output one JSON object:
[
  \{
    "step\_id": \textless{}number\textgreater{},

    "description": "\textless{}the original or modified step description from annotation\textgreater{}",

    "start\_time": \textless{}float\textgreater{},
    "end\_time": \textless{}float\textgreater{},

    "error\_tag": "\textless{}tag from annotation\textgreater{}",

    "service\_type": \{
    "main": "Instant Proactive Service"
        \textbar{} "Short-Term Proactive Service"
        \textbar{} "Episodic Proactive Service",
    "sub": "Safety"
        \textbar{} "Tool Use"
        \textbar{} "Error-Recovery"
        \textbar{} "Next-Step Guidance"
        \textbar{} "Resource Reminder"
        \textbar{} "Episodic Task Reminder"
        \textbar{} "Episodic Memory Recall"
    \},

    "dialogue": [
    \{
        "role": "assistant",
        "utterance": "\textless{}first proactive message (natural, respectful, concise)\textgreater{}"
    \},
    \{
        "role": "user",
        "utterance": "\textless{}optional short user reply\textgreater{}"
    \}
    ]
  \}
]

------------------------------------------------------------
Input
------------------------------------------------------------

You will receive step annotations in JSON format.

Each step may contain:
- description
- step\_id
- errors (with tag and description)
- start\_time, end\_time
- modified\_description (optional)

ONLY generate outputs for steps that contain errors.
Do NOT generate output for correct steps.
\end{promptbox}
